A Conceptual Framework for Ethical Evaluation of Machine Learning Systems

Research in Responsible AI has developed a range of principles and practices to ensure that machine learning systems are used in a manner that is ethical and aligned with human values. However, a critical yet often neglected aspect of ethical ML is the ethical implications that appear when designing evaluations of ML systems. For instance, teams may have to balance a trade-off between highly informative tests to ensure downstream product safety, with potential fairness harms inherent to the implemented testing procedures. We conceptualize ethics-related concerns in standard ML evaluation techniques. Specifically, we present a utility framework, characterizing the key trade-off in ethical evaluation as balancing information gain against potential ethical harms. The framework is then a tool for characterizing challenges teams face, and systematically disentangling competing considerations that teams seek to balance. Differentiating between different types of issues encountered in evaluation allows us to highlight best practices from analogous domains, such as clinical trials and automotive crash testing, which navigate these issues in ways that can offer inspiration to improve evaluation processes in ML. Our analysis underscores the critical need for development teams to deliberately assess and manage ethical complexities that arise during the evaluation of ML systems, and for the industry to move towards designing institutional policies to support ethical evaluations.

==> old/iteration3_03.tex <==
\section{Considering Ethics in Selecting Evaluation Frameworks}

We show how ethical values, and other practical needs of practitioners, are considered when selecting best evaluation practices for ML systems. In illustrating the discussion teams have, we introduce a novel utility based framework that shows the interaction and tradeoffs between ethics and information gained in performing evaluations. 
% state how we came up with this and the fact that this is novel.  

\subsection{Sketch of Utility Framing of Best Evaluation Practice} \hari{Desiderata for ethical/optimal/responsible? evaluation practice}

We step \hari{formulate?} through six illustrative properties of a team's decision\hari{unless we know this from literature, I wouldnt frame it as team's decisions, keep it at a high level, we identified.. } making when selecting an evaluation practice for ML systems, building to a single utility model that captures the advantages and disadvantages of a best evaluation practice. For each of the six properties, we discuss its necessity, the underlying assumptions, and its implications. We close by discussing how the properties interlink to create a model of the best \hari{do we have a definition of "best" in related work, or are we defining what best means?} evaluation practice. In representing the multilayered behaviors of teams in these steps, we are able to  clearly define their choices, tradeoffs, and constraints. These steps also will allow us to discuss cases in Section 4, and frame advice for mitigation strategies for the ethical AI industry in Section 5. 

\textbf{Property 1: Selecting a best evaluation out of several alternatives.}
ML development teams have several considerations and options for evaluation practices, including both online and offline testing methods.  Some questions teams might ask themselves in formulating evaluation methods include which desired properties tests should target, or what specific components of a large system need to be tested. The fundamental purpose of an evaluation is to detect differences between desired and actual model behavior, so defining what desired model behavior is is critical \cite{zhang2020machine}. Prior works describe the innumerable evaluation decisions (is d a specific evaluation method, or is it more low level and relates to decisions that needs to be made when planning evaluation?) as leading to a ``paradox of choice" for practitioners deciding how to perform an evaluation \cite{goel2021robustness}. So, the starting point for our utility model of decision making is generating options for evaluation frameworks $D$ and our goal will be:

$$\textit{choose best } d \in D$$

\textbf{Property 2: Evaluations are cost constrained.}
Across the development lifecycle, workers are often ``incentivized by metrics associated with financial gain" \cite{ali2023walking}. For ML testing specifically, one of the fundamental challenges is cost constraints, with teams often considering options for reducing costs of tests via methods such as test prioritisation, in which inputs generated for tests are limited to inputs that are most indicative of problematic behavior \cite{zhang2020machine}. Thus, our decision function is restricted by resources available. We represent this as:

$$\textit{choose best } d \in D \textit{ such that cost(d)}\leq \textit{resources}$$

\textbf{Property 3: The best evaluation method has the highest utility.}
An evaluation practice can be good or bad depending on its consequences, and the best evaluation practice can be chosen based on the utility of the evaluation practice. This is in following of the consequentialism philosophy - that actions are good or bad depending on its consequences - which is used to argue that the goal of a ML model evaluation is to understand how a model will interact with society, and establish that this ``understanding" can be represented as utility \cite{hutchinson2022evaluation}. The fair ML literature has established the representation of ML models as providing a utility, to consider decision making regarding model choice as a function of costs and benefits \cite{corbett2017algorithmic, corbett2018measure, chohlas2021learning}. Here, rather than utility maximization representing the decision of a team in selecting a model, the utility maximization problem represents the decisions made by a team in developing and deploying a large-scale ML system \hari{should this just be evaluation, a step in developing and deploying...}.

We represent the best decision of evaluation practice for the team as the decision with the highest utility. The utility function maps each decision option the team is considering to a single numeric value (with unit ``utils"), and selecting the best decision equates to selecting the decision with the highest utility. An evaluation framework $d^*$ is the optimal decision if it is the utility maximizing decision, indicated as:

$$u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$$


\textbf{Property 4: Utility is composed of gain and loss, in the form of of information and ethical harms.}
The goal of machine learning testing is to learn about system performance in order to detect differences between desired and actual model behavior \cite{zhang2020machine}. We characterize the information we learned from a test as the \emph{gain} from the evaluation process. On the other hand, concerns about ethics of machine learning systems include concerns about the ethics of evaluation practices, because operationalizing the evaluation process may lead practitioners to make sacrifices across ethical values. This will be further exemplified in a series of cases in Section 4. We break the utility function into a cost-benefit function, with the information gain representing the utility benefit, and potential ethical harm representing the utility cost. Thus, our decision of the optimal evaluation framework would solve:

$$\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{such that cost}(d) \leq \textit{resources}$$

\textbf{Property 5: Information gain and ethical harm are in expectation}. 
Thus far, we have chosen to represent the decision of the best evaluation framework as choosing an evaluation with the highest numeric value of utility, and we now need to acknowledge that in doing so, costs and benefits in the utility function need to be represented as average expected values. This expectation allows us to illustrate three things: (1) In several instances, ethical values are difficult to prove or quantify \cite{ali2023walking}, as is information gain. (2) There are several instances of models that differ in social impact across groups, notably underrepresented groups. The estimate of expected ``ethical harm" can be considered an average of harm across several individuals who experience disparate impact from the models \cite{hutchinson2022evaluation}. (3) We account for likelihood of risks over time. In following the consequentialism argument, utility corresponds with impact \cite{hutchinson2022evaluation}. Ethical harm of an evaluation may not be guaranteed but may have some likelihood of occurring (for example, an evaluation that may carry risk of potential privacy leaks at some point in the future, but is not guaranteed to today). For these reasons, we adjust our notation and use the function $\mathit{IG}(d)$ for information gain, the function $\mathit{EH}(d)$ for ethical harm of the evaluation, and now our optimal decision of evaluation framework would solve:

$$\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$$


\textbf{Property 6: Ethical harm is composed of weighted ethical values.}
Ethical values need to be accounted for independently of one another in the utility function, for two reasons. (1) It is obvious that not all ethical values are applicable in all settings -- for example, there may be applications where privacy is not a concern because only public data is used, or cultural sensitivity is not a concern because individual data is not used. (2) There is an established tradeoff between some ethical concerns themselves. For example, existing literature has established gains in fairness of a model yield loss of privacy ~\todocite{ashwin?}. By parameterizing ethical values in our utility function, we acknowledge the need for model practitioners to weigh ethical concerns against each other in selecting the best evaluation practice. With these values parameterized, we add a weighting to each value, to represent differing ethical priorities of teams, or regulatory requirements on particular ethical values.

Thus, parameterizing values by $j$, with weights $w_j$, the best evaluation practice for a team would solve:
\begin{equation}
\text{max}_{d\in \mathcal{D}}\mathbb{E}(\mathit{IG}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))
\end{equation}

\subsection{Discussion and Implications}
\hari{I would keep the two tables and fold it into the previous sub-section, I dont think we need to have discussion and implications here}
\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.45\linewidth}|p{0.35\linewidth}|p{0.2\linewidth}|}
        \hline
        \textbf{Utility Framing} & \textbf{Properties} & \textbf{Motivating questions and considerations} \\
        \hline
         $\textit{choose best } d \in D$ & Selecting the best evaluation & \emph{What is our testing goal, what options do we have for evaluation frameworks, and what would they look like?} \\
        \hline
        $\textit{choose best } d \in D \textit{ s.t. } \textit{cost} (d)\leq \textit{resources}$& Evaluations are cost constrained & \emph{What are our resource limitations for evaluating our system?} \\
        \hline
        $u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$
& The best evaluation has the highest utility & \emph{How can I define the best evaluation framework and compare between options?}\\
        \hline
        $\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{such that cost}(d) \leq \textit{resources}$
& Information gain and ethical harm & \emph{What information do I hope to gain and what ethical harms could I cause?} \\
        \hline
         $\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$& Expectation of information gain and ethical harm & \emph{Have I accounted for potential ethical harm or information gain in the future? Have I accounted for disparate impact by population?} \\
        \hline
        $\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$& Ethical harm composed of ethical values & \emph{Which ethical values am I prioritizing, or what regulatory requirements for ethics do I need to satisfy?} \\
        \hline
    \end{tabular}
    \caption{Summary of properties of deciding to use an ethical evaluation that, when taken together, lead to a single utility model framing the costs, benefits, and resource constraints for a team's decision making. Although the order in which these are listed increase in detail, this is for the purpose of describing the setting, and do not need to be considered in this order. }
    \label{tab:tab1}
\end{table}


\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.2\linewidth}|p{0.35\linewidth}|p{0.45\linewidth}|}
        \hline
        \textbf{Notation} & \textbf{Definition} & \textbf{Meaning} \\
        \hline
         ${d \in D}$ & Evaluation choices & The set of possible evaluation methods is D and we are aiming to choose the d that yields maximium utility \\
        \hline
        $\mathbb{E}(\textit{IG}(d))$& Expected benefit in utility & Expected information gain from evaluation practice d. \\
        \hline
        $\mathbb{E}(\textit{EH}_j(d))$& Expected cost in utility & Expected ethical harm of decision d across value j \\
        \hline
        $j$ & Specific ethical value & Parameterizes ethical value concerns \\
        \hline
         $\textit{cost}(d) \leq \textit{resources}$& Resource constraints to testing & Limits to evaluation processes that fit budget \\
        \hline
        $w_j$ & value importance & weight of particular value concern, imposed by priority or regulation \\
        \hline

    \end{tabular}
    \caption{Notation guide to Equation 1, which serves to illustrate the components and tradeoffs of a team's decision to select an ethical evaluation practice.}
    \label{tab:tab2}
\end{table}


We have described, in the section above, the key properties of practitioners' decision making when selecting an ethical evaluation practice. Combining these properties into a single equation, Equation 1 (with notation guide in Table 2), we see that a best evaluation practice is chosen after considering the information gained from the practice, potential ethical harms, and is limited by the resources available. In Table 1, we combine these properties with suggested questions a team might ask itself in the process of formulating this decision making process.

In the next section, we will discuss cases of teams that have utilized this cost-benefit framework, and, in discussing analagous domains, we will cover the potential mitigations that strengthen ethical value considerations in machine learning. 

% Defend why this is a good model, why we care about max utility, how can we think about info gain and evaluation, why did we decide not to consider time. Walk through formulation and get them to buy in. Make sure a person who is new will be able to understand. Self contained. Come up with list of cases for section 4, flesh out the model some more. define what tradeoff is, why we need it, elaborate on formulation. Convince them it is useful. 


%\textbf{Model Implications to improve ethical ML}
% Continuing the framing described, we now discuss implications this analogy has for ways to improve the ethicality of machine learning systems. \textbf{Mitigation 1: Better tests eliminate uncertainty} IRB checks on expectation of ethical harm.  \textbf{Mitigation 2: Add constraints} Increase costs to ethical harm by creating regulation driving up weight on ethical harm.  In the next section, we will discuss ways in which these weights, if enforced by regulation, can be used to ensure ethical evaluation practices. The optimization is also subject to the cost constraints of the evaluation, as teams are bind by infeasibility of doing every possible evaluation on a system.  \textbf{Mitigation 3: Create incentives for earnings to vary with values} Information gain or resources can vary with ethical harm. 


==> old/jan_01_intro.tex <==
\section{Introduction}


\hari{Notes from Jessica:}
Typical model evaluation focuses on estimating generalization error, loss on a new sample from same distribution. The ML workflow - specifically separate train test and validation data and use of procedures like cross validation set the standard for getting high internal validity in estimates. Getting good estimates of generalization error is important for several reasons: so that developers can ensure that the error is reasonable for their intended use/deployment, and so that developers have a metric to try to further refine the model in light of. However, the laser focus on minimizing error has been criticized leading to lots of alternative metrics and methods for evaluation focused on various ethical concerns, as well as threats to external validity like distribution shift, where the estimated generalization error on iid data is a poor estimate for the action error experienced when the model is deployed due to various forms of dataset shift.

We observe that even when evaluation does involve considering ethical factors like fairness, privacy loss, etc., harms induced by the evaluation itself may still be overlooked. [examples].

To conceptualize evaluation itself as ethically implicated, we distinguish between the evaluation population consisting of indivdiuals affected by the evaluation procedure and the deployment population consisting of individuals who experience the model in production. The evaluation population is typically instrumental in helping developers ensure that the deployment population experiences a maximally performant model, whether in terms of accuracy or other properties (fairness, privacy, etc). [now briefly frame it as balancing the utility of the information gained from evaluation (which can be instrumental for improving the model further) with the utility lost in the process of evaluation itself]







\textbf{****1. Scope of evaluation has expanded to include range of qualitative and quantitative metrics requiring complex evaluations.}

Traditionally, in developing machine learning  models, the focus has been on optimizing models for accuracy or other performance metrics. In building machine learning models that are both useful and ethical, we evaluate models across various criteria. The suitability of a machine learning model is governed by more than just accuracy, necessitating evaluation frameworks of models with regard to characteristics such as robustness, privacy, fairness, and interpretability. Regardless of the particular evaluation practice via a quantified metric or using a non-quantifiable argument, the higher level goal is to make evaluation more effective by enabling practitioners to identify model shortcomings before deployment.
Quantifiable metrics, like xxx or xxx.... Other research highlights the necessity of non-technical, harder to quantify lines of inquiry, encouraging practitioners to consider the downstream harms of models, and whether performance disparities align with historic or engrained power imbalances. These approaches advocate that practitioners identify and engage with different stakeholders, and understand the extent to which they are impacted by the deployment.


As systems grow in scope and size, so do testing needs. 


% Traditional evaluation methods for machine learning models rely on quantified metrics that have been established for one or multiple of these characteristics, i.e., in evaluating fairness of a model, we may look to counterfactual fairness of individual outcomes, and in evaluating privacy, we may look to differential private mechanisms. \jessica{differential privacy is a mathematical guarantee that we can use mechanisms to achieve, so I wouldn't say its used to evaluate,  more to parameterize noising algs. do you have an example in mind?}

\jessica{Personally I prefer a more third person account, eg rather than saying people should, say These approaches advocate that... so its clearer who is issuing directive}

Metrics for evaluation are usually quantified aspects of a model’s performance that can be measured and reported by practitioners. For instance, beyond simply accuracy, developers may seek to measure a model's fairness, robustness, interpretability, or capacity for misuse. In service of these goals, related work has developed, and studied the tradeoffs, of different metrics. There is a continuous evolution of research in this field as machine learning paradigms also evolve; For instance, a growing literature covers the need for quantifying generative models in terms of their toxicity, bias, and factual correctness.

In support of the pursuit of these goals, a growing body of work creates more comprehensive methods with which to evaluate models, rather than providing a singular empirical metric or set of metrics. 

These provide practitioners a standardized worksheet approach with which to evaluate models, with many focused on a single concrete goal (eg privacy), and others taking a more holistic view, seeking to provide practitioners with a means of balancing multiple forms of evaluation. 

These provide valuable transparency for practitioners by establishing a common setting and add ease to communication. A number of evaluation methods are pre-deployment like benchmarking. Other mechanisms, to aid evaluation ex-post deployment, such as bug bounty challenges, \jessica{not familiar with what this is} provide infrastructure to support stakeholder feedback.
A particular evaluation process may involve choosing one or many evaluation metrics to measure, as part of a decision of which metrics best serve values or ideals. Evaluation decisions are so pervasive that prior work has observed that practitioners can suffer from a ``paradox of choice'' when it comes to deciding how to perform evaluation~\cite{goel2021robustness}.

\textbf{Evaluating the Ethical Values of ML Systems}. More disparate than the other two relevant bodies of literature is a broad set of work that focuses on the ethicality of machine learning systems. \jessica{is it that easy to separate ethics? like isn't a choice to prioritize accuracy ethical in some sense, because you're minimizing bad outcomes as population level?} Existing work characterizes principles and values that machine learning systems should adhere to, and questions goals of deployed systems. Evaluation processes and metrics assess the performance of a model across specific \textit{values}, as values are aspects of a system which practitioners are interested in measuring. For instance, engineers may use metrics to measure achievement of values, such as fairness, robustness, or accuracy. \jessica{again im not sure there's a clear distinction between the values you mean here and the values that lead us to use more conventional metrics}





- \textbf{*****2. while these evaluation approaches are necessary for RAI, there are inherent harms in conducting evaluation. Real world examples}

 However, \sout{based on prior work/literature, we see that} when carrying these evaluations out, we make tradeoffs. \jessica{might use 'researchers' instead of 'we' for clarity} We have evaluation methods that assess viability of a particular model, aiming to provide engineers with greater information on a model's shortcomings. But, when operationalizing the evaluation process, we make sacrifices across other values, because the evaluation process itself may create ethical harms. The Tesla Autopilot systems are an example of a model where its evaluation practice  is considered by many to be unethical in the process of evaluation, but may be effective at preventing downstream harm once completed. The system is trained and tested on public roads with other drivers, but were involved in several fatal crashes \cite{siddiqui2022} \jessica{move this description earlier, when I read the previous sentence I wanted to know what I was supposed to already know about Tesla Autopilot}


- \textbf{****3. problem is underdefined. We characterize the problem and various trade-offs, and we propose ethical evaluation based on analogous domains.}

To close, this \jessica{what?} is a critical question for the machine learning community to discuss. In disaggregated evaluation, we ask ourselves whether the end result model is a good fit for what its being used for. When model is deployed, we have numerous methods for evaluating these methods based on values of the community. Although we care about the values of deployed models, less visible, but highly important ethical decisions are happening during building and testing. \jessica{seems like this should be said earlier/integrated above. I would just end intro with contributions}


Unfortunately, the literature offers little guidance on how practitioners should navigate ethical dilemmas while evaluating a model. This work seeks to fill the gap by documenting and discussing ethical criteria for evaluation practices of machine learning models. We assess how certain evaluation methods force us to prioritize certain values over others, and the value tradeoffs we make when choosing evaluation methods. We begin by identifying the values guiding models, \jessica{does this mean the AI/ML models, or some other models Is this saying these values are guiding model selection?} such as harm-avoidance, interpretability, or cost. Then, we discuss the value-based decisions and evaluation process \jessica{what does the prev phrase refer to?} within various evaluation methods, \jessica{what is an evaluation process within an evaluation method?} such as A/B testing or adversarial testing. \jessica{Our premise in highlighting the ethical dimension of evaluation decisions is that} advanced planning can help ensure an evaluation method is compliant with \jessica{researcher's} values.  

Questions around ethical evaluation practices is not a new problem in various scientific communities, and is occurring in machine learning following several other groups. \jessica{what does that latter phrase mean, following several other groups?} We close by observing where similar tradeoffs arise in the evaluation practices of analogous domains. \jessica{I'm not sure where this paragraph is going - seems like now we are saying ethics of eval is not new, but what else?} For example, A/B testing done in clinical trials requires IRB approval. We study analogous domains, such as drug development, to identify (1) how comparable practitioners balance achieving their goals subject to various constraints when building models, and (2) the mitigating procedures and institutions that have been developed in order to support their values. \jessica{I think I'm having trouble differentiating what contribution this paragraph is highlighting versus the paragraph above this one }

This is novel \jessica{what is novel?} in that this discussion of values is to be considered during the model development lifecycle and pre-deployment, and can also be discussed post-deployment, post-incident, or during regulatory compliance changes. \jessica{point of prev sentence is getting lost for me} As ethical practitioners, we need to care about \jessica{what?} during the lifecycle as well, whereas most existing frameworks provide post-deployment documentation. \jessica{not sure about previous claim}.
We provide examples around value discussions from other domains that also aim to avoid harmful practices, to generate discussion around options for emerging best practices for evaluation of values in machine learning




\hari{note to self, non-testable programs}



%Machine learning literature which focuses on quantifiable metrics for performing evaluation ignores ethical challenges that emerge in the evaluation process. In contrast, reporting toolkits that have become available aim to increase transparency of AI ethics by acknowledging model shortcomings across various ethical characteristics, and are often provided by teams that have built models as documentation with a deployed model. These allow teams considering using a model to accurately evaluate its ethical impacts and tradeoffs of deploying a provided model on a population of users (cite modelcards etc). Additionally, note that the values of the creators may be different than the values for the end users. 

==> old/jan_02_model.tex <==
\section{Conceptualizing the Ethics of Evaluation} \label{sec:framework}

ML software teams can benefit from a conceptual framework to characterize the ethical trade-offs in evaluating machine learning models. Ideally, such a framework should (1) account for different ethical \textit{values} at play, such as fairness, privacy, and social impact, (2) support the analysis of future \textit{benefits} from evaluation insights by accounting for present ethical \textit{harms} of evaluation choices, and (3) facilitate productive discourse around \textit{minimizing} ethical harms from the evaluation process. Here, we formulate a utility-based conceptual framework for ethics of evaluation by considering prior work on ethical values in ML and evaluation methods and objectives.  Specifically, we define six key properties that are integral to planning ML evaluation. For each property, we discuss its necessity, scope, underlying assumptions, and its implications. Collectively, these properties form a conceptual utility framework that captures the advantages and disadvantages of a chosen evaluation practice from an ethical standpoint.

We note that this conceptualization follows a common style in decision sciences or macroeconomics in illustrating a thought experiment by sketching a simplified world of decision-making \cite{sargent2000recursive}. By decomposing the ``best" model evaluation into only its key components, we can differentiate and categorize the variables that impact the model evaluation method, discuss the interaction between these variables (whether they are competing or complementary), and formulate strategies to prioritize ethics. This is not meant to be taken as a measurable series of linear steps a team will undertake.

\textbf{Property 1: Selecting an evaluation approach out of several alternatives.}
Evaluation is the process of assessing and measuring a model's performance against a set of defined criteria or benchmarks. ML development teams have several options and considerations when planning evaluations that involve complex decisions across evaluation scope, context, and effect~\cite{zhang2020machine, riccio2020testing, song2022exploring}. In fact, prior work has observed that practitioners can suffer from a ``paradox of choice'' when it comes to deciding how to perform evaluation~\cite{goel2021robustness}. Some questions teams might ask themselves include which desired properties tests should target, what specific components of a large system need to be tested, or what metrics best reflect the model's real-world performance. Therefore, a model for ethics of evaluation should inherently situated in the space of decisions in planning model evaluation. Let us represent this space of evaluation as $D = \{d_1,d_2,\ldots,d_m \}$ where d is an evaluation decision (e.g., choice of metrics, method of evaluation, sample selection, etc.). 
$$\textit{choose some d}\in D$$
\textbf{Property 2: Evaluations are cost constrained.}
\textit{Cost} measures the resources required to conduct an evaluation. One of the fundamental challenges for ML testing is cost constraints, in which teams are often considering options for reducing the costs of tests via methods such as test prioritization, in which inputs generated for tests are limited to inputs that are most indicative of problematic behavior~\cite{zhang2020machine}. For instance, monetary constraints may restrict the number of annotations developers may procure for validation data~\todocite{work on efficiently building validation sets}. Constraints on labor availability may restrict the number of engineers capable of focusing on evaluation, requiring more automation and less manual examination of errors~\todocite{work on automatically detecting errors}. Constraints on time may restrict the ability of engineers to run longer-range evaluations\todocite{}{add citation}. These resource constraints can challenge responsible model development~\cite{hopkins2021machine}. Thus, our decision function is restricted by the resources available. We represent this as:

$$\textit{choose } d \in D \textit{ such that cost(d)}\leq \textit{resources}$$


\textbf{Property 3: The best evaluation method has the highest utility.}
An evaluation practice can be good or bad, depending on its consequences. This perspective aligns with  \textit{consequentialism} philosophy, which posits that the morality of an action is judged based on its outcome~\cite{mill2016utilitarianism, bentham1996collected}. In the context of ML model evaluation, this principle suggests that the primary objective is to understand how a model will function within societal contexts and can be quantified as `utility'~\cite{hutchinson2022evaluation}. The fair ML literature has established the representation of ML models as providing a utility to consider decision-making regarding model choice as a function of costs and benefits \cite{corbett2017algorithmic, corbett2018measure, chohlas2021learning}. For example, in \cite{corbett2017algorithmic}, the authors provide a definition of `immediate utility', which reflects the costs and benefits of a fair decision by a policymaker, notably in the setting of pre-trail bail release decisions. Similarly, in \cite{corbett2018measure}, the utility function reflects a single decision made by a model, such as whether or not to screen an individual for diabetes. In \cite{chohlas2021learning}, a utility function determines the optimal decision-making, such as in the decision to provide funded transportation for court appearances. Our framework deviates from these in that we are not focused on the fair output and decisions made by an ML model. Rather, we are focused on the decisions made by a team when developing and evaluating an ML model or system.

We represent the best decision of evaluation practice for the team as the decision with the highest utility. The utility function maps each decision option the team is considering to a single numeric value (with unit ``utils"), and selecting the best decision equates to selecting the decision with the highest utility. An evaluation framework $d^*$ is the optimal decision if it is the utility-maximizing decision, indicated as:

$$u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$$


\textbf{Property 4: Utility is composed of gain and loss in the form of information and ethical harms.}
As mentioned earlier, the goal of testing is to learn about system performance in order to detect differences between desired and actual model behavior~\cite{zhang2020machine}. We characterize this information learned as the \emph{gain} from the evaluation process. Based on prior literature, the information gained can be about internal validity, external validity, and robustness of the model. In social science, \textbf{internal validity} measures the methodological correctness of an experimental study and the extent to which its findings reflect true phenomenon in the studied data~\cite{drost2011validity}. In ML evaluation, internal validity is concerned with ensuring the validity of a property within a specific learning problem~\cite{liao2021we}. This includes information verifying that the model's performance reflects its ability to learn and generalize from the data it was trained on and is not unduly influenced by external factors or biases. Threats to interval validity often arise from researcher-degrees-of-freedom in defining the learning problem in ways that artificially inflate performance estimates such that their intended meaning no longer holds \cite{hofman2023pre}. The engineers may have inadvertently used information from the test set during model training, causing train-test leakage~\cite{kapoor2023leakage}, or face issues with inaccurate labels during training and testing~\cite{northcutt2021pervasive, chen2022, gordon2021disagreement}, leading to misleading performance metrics. Additionally, internal validity can be compromised by software bugs affecting metric reporting or by continued optimization post-test set evaluation, both of which can skew the true performance of the model~\cite{allevitan2021,hosseini2020tried}.

Further information gain corresponds to \textbf{External validity} --- the extent to which findings on a studied context or population hold for different contexts or populations~\cite{drost2011validity}. In ML evaluation, the most pressing form of threat to external validity is that performance on evaluation tests will not be consistent with the performance on the deployment population due to distribution shifts. Other challenges to external validity may emerge from constraints in the benchmark dataset or discrepancies between the evaluation metrics used and those that are actually relevant to the broader task~\cite{liao2021we}. Third, external validity is also linked to information gained about the \textbf{robustness} of the model, i.e., the degree to which the model or system maintains its correctness and performance under varying conditions and inputs, including invalid or adversarial inputs~\cite{zhang2020machine}. Testing for robustness involves evaluating the model's accuracy and performance in the presence of noise or disturbances~\cite{tjeng2017evaluating}. Threats to the utility can arise from errors in creating adversarial examples, model complexity, limited understanding of underlying mechanics, and choosing appropriate metrics that accurately reflect robustness~\cite{zhang2020machine, goodfellow2014explaining}.  

In describing information gain, we recognized potential threats to information utility due to evaluation choices regarding internal validity, external validity, and robustness. However, a critical and often overlooked area of concern pertains to the ethical implications of evaluation practices. The process of operationalizing evaluation can sometimes lead practitioners into challenging situations where they may have to balance or even compromise on ethical values. When ethical considerations are not adequately addressed in evaluation decisions, it can potentially diminish the acceptability of the results and the overall value and utility of the information derived from the evaluation. Thus, we break the utility function into a cost-benefit function, with the information gain representing the utility benefit and potential ethical harm representing the utility cost. Thus, our decision on the optimal evaluation framework would solve the following:

$$\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{ such that cost}(d) \leq \textit{resources}$$

A growing body of literature discusses properties that ethical machine learning systems should inherently possess~\cite{jobin2019global,zhang2020machine, martinez2022software}. These properties may be discussed in the context of what machine learning systems are tested to accomplish for~\cite{zhang2020machine}, or these properties may be discussed in the context of what an ethical machine learning system embodies~\cite{jobin2019global}. These studies converge on the following ethical values: (1) \textbf{Harmfulness}, which measures the extent to which the evaluation workflows and outcomes inflict an injury on any individual or population~\cite{mehrabi2021survey}, (2) \textbf{Privacy} which as a value refers to the principle of protecting personal and sensitive information from unauthorized access, use, or exposure during the entire ML lifecycle~\cite{liu2021machine}, (3) \textbf{Fairness} in which the goal is to achieve equitable treatment and outcomes for all individuals, ensuring that the benefits and burdens of AI systems are distributed justly across diverse populations~\cite{mehrabi2021survey}, (4) \textbf{Cultural Sensitivity} which involves designing algorithms and models that are attuned to and respectful of cultural differences, ensuring that they do not perpetuate stereotypes, biases, or insensitivities~\cite{jo2020lessons}, (5) \textbf{Sustainability} which ensures that models are developed in a manner that is environmentally responsible, economically feasible, and socially equitable~\cite{eugoals,lacoste2019quantifying}, and (6) \textbf{Societal Impact} which refer to ensuring that the models contribute positively to societal wellbeing, addresses social issues, and does not harm individuals or communities~\cite{birhane2022values}. We emphasize that this is not a comprehensive listing of all ethical values that a machine learning system may seek to accomplish but is most common in existing ML literature. 

\textbf{Property 5: Information gain and ethical harm are in expectation}. 
Thus far, we have chosen to represent the decision of the best evaluation framework as choosing an evaluation with the highest numeric value of utility, and we now need to acknowledge that in doing so, costs and benefits in the utility function need to be represented as average expected values. This expectation allows us to illustrate three things: (1) In several instances, ethical values are difficult to prove or quantify \cite{ali2023walking}, as is information gain. (2) There are several instances of models that differ in social impact across groups, notably underrepresented groups. The estimate of expected ``ethical harm" can be considered an average of harm across several individuals who experience disparate impact from the models \cite{hutchinson2022evaluation}. (3) We account for the likelihood of risks over time. In following the consequentialism argument, utility corresponds with impact \cite{hutchinson2022evaluation}. Ethical harm of an evaluation may not be guaranteed but may have some likelihood of occurring (for example, an evaluation that may carry the risk of potential privacy leaks at some point in the future but is not guaranteed today). For these reasons, we adjust our notation and use the function $\mathit{IG}(d)$ for information gain, the function $\mathit{EH}(d)$ for ethical harm of the evaluation, and now our optimal decision of evaluation framework would solve:

$$\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{ such that cost}(d) \leq \textit{resources}$$


\textbf{Property 6: Ethical harm is composed of weighted ethical values.}
\neha{One option to consider is expanding this section out into saying 'ethical harm can be decomposed into several factors', including various values, the duration of the impact, who the impact is on....}
Ethical values need to be accounted for independently of one another in the utility function for two reasons: (1) It is obvious that not all ethical values are applicable in all settings -- for example, there may be applications where privacy is not a concern because only public data is used, or cultural sensitivity is not a concern because individual data is not used. (2) There is an established trade-off between some ethical concerns themselves. For example, some researchers have established privacy risks of in fairness in some models \cite{pujol2021equity}. By parameterizing ethical values in our utility function, we acknowledge the need for model practitioners to weigh ethical concerns against each other in selecting the best evaluation practice. With these values parameterized, we add a weighting to each value to represent differing ethical priorities of teams or regulatory requirements on particular ethical values.

Thus, parameterizing values by $j$, with weights $w_j$, the best evaluation practice for a team would solve:
\begin{equation}
\text{max}_{d\in \mathcal{D}}\mathbb{E}(\mathit{IG}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d)) \textit{ s.t. } \textit{costs}(d) \leq \textit{resources}
\end{equation}

To summarize, here we have described the key properties of practitioners' decision-making when selecting an ethical evaluation practice. Combining these properties into a single equation, Equation 1 (with notation guide in the appendix), we see that a best evaluation practice is chosen after considering the information gained from the practice, potential ethical harms, and is limited by the resources available. In the next section, we will discuss real-world cases of evaluations that violate ethical values through this cost-benefit framework. 



\begin{comment}
    




A particular evaluation process may involve choosing one or many evaluation metrics to measure, as part of a decision of which metrics best serve values or ideals. 


ML development teams have several considerations and options for evaluation practices, including both online and offline testing methods.  Some questions teams might ask themselves in formulating evaluation methods include which desired properties tests should target, or what specific components of a large system need to be tested. The fundamental purpose of an evaluation is to detect differences between desired and actual model behavior, so defining what desired model behavior is is critical \cite{zhang2020machine}. Prior works describe the innumerable evaluation decisions (is d a specific evaluation method, or is it more low level and relates to decisions that need to be made when planning evaluation?) as leading to a ``paradox of choice" for practitioners deciding how to perform an evaluation \cite{goel2021robustness}. So, the starting point for our utility model of decision-making is generating options for evaluation frameworks $D = {}$ and our goal will be:





\textbf{Machine learning evaluation metrics.} A large body of work focuses on defining and motivating metrics for evaluation. These are usually quantified aspects of a model’s performance that can be measured and reported by practitioners. For instance, beyond simply accuracy, developers may seek to measure a model's fairness, robustness, interpretability, or capacity for misuse. In service of these goals, related work has developed, and studied the tradeoffs, of different metrics. There is a continuous evolution of research in this field as machine learning paradigms also evolve; For instance, a growing literature covers the need for quantifying generative models in terms of their toxicity, bias, and factual correctness.

\textbf{Machine Learning Evaluations.} In support of the pursuit of these goals, a growing body of work creates more comprehensive methods with which to evaluate models, rather than providing a singular empirical metric or set of metrics. \jessica{seems like previous two sentences should go first in this section, like before metrics?}
%These provide practitioners a standardized worksheet approach with which to evaluate models, with many focused on a single concrete goal (eg privacy), and others taking a more holistic view, seeking to provide practitioners with a means of balancing multiple forms of evaluation. 
These provide valuable transparency for practitioners by establishing a common setting and add ease to communication. A number of evaluation methods pre-deployment, such as A/B testing or live testing, \jessica{isn't A/B testing usually done live?} are common practice across institutions and domains. Other mechanisms, to aid evaluation ex-post deployment, such as bug bounty challenges, \jessica{not familiar with what this is} provide infrastructure to support stakeholder feedback.








\section{Considering Ethics in Selecting Evaluation Frameworks}

We show how ethical values, and other practical needs of practitioners, are considered when selecting best evaluation practices for ML systems. In illustrating the discussion teams have, we introduce a novel utility based framework that shows the interaction and tradeoffs between ethics and information gained in performing evaluations. 
% state how we came up with this and the fact that this is novel.  

\subsection{Sketch of Utility Framing of Best Evaluation Practice} \hari{Desiderata for ethical/optimal/responsible? evaluation practice}

We step \hari{formulate?} through six illustrative properties of a team's decision\hari{unless we know this from literature, I wouldnt frame it as team's decisions, keep it at a high level, we identified.. } making when selecting an evaluation practice for ML systems, building to a single utility model that captures the advantages and disadvantages of a best evaluation practice. For each of the six properties, we discuss its necessity, the underlying assumptions, and its implications. We close by discussing how the properties interlink to create a model of the best \hari{do we have a definition of "best" in related work, or are we defining what best means?} evaluation practice. In representing the multilayered behaviors of teams in these steps, we are able to  clearly define their choices, tradeoffs, and constraints. These steps also will allow us to discuss cases in Section 4, and frame advice for mitigation strategies for the ethical AI industry in Section 5. 










\textbf{Property 5: Information gain and ethical harm are in expectation}. 
Thus far, we have chosen to represent the decision of the best evaluation framework as choosing an evaluation with the highest numeric value of utility, and we now need to acknowledge that in doing so, costs and benefits in the utility function need to be represented as average expected values. This expectation allows us to illustrate three things: (1) In several instances, ethical values are difficult to prove or quantify \cite{ali2023walking}, as is information gain. (2) There are several instances of models that differ in social impact across groups, notably underrepresented groups. The estimate of expected ``ethical harm" can be considered an average of harm across several individuals who experience disparate impact from the models \cite{hutchinson2022evaluation}. (3) We account for likelihood of risks over time. In following the consequentialism argument, utility corresponds with impact \cite{hutchinson2022evaluation}. Ethical harm of an evaluation may not be guaranteed but may have some likelihood of occurring (for example, an evaluation that may carry risk of potential privacy leaks at some point in the future, but is not guaranteed to today). For these reasons, we adjust our notation and use the function $\mathit{IG}(d)$ for information gain, the function $\mathit{EH}(d)$ for ethical harm of the evaluation, and now our optimal decision of evaluation framework would solve:

$$\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$$


\textbf{Property 6: Ethical harm is composed of weighted ethical values.}
Ethical values need to be accounted for independently of one another in the utility function, for two reasons. (1) It is obvious that not all ethical values are applicable in all settings -- for example, there may be applications where privacy is not a concern because only public data is used, or cultural sensitivity is not a concern because individual data is not used. (2) There is an established tradeoff between some ethical concerns themselves. For example, existing literature has established gains in fairness of a model yield loss of privacy ~\todocite{ashwin?}. By parameterizing ethical values in our utility function, we acknowledge the need for model practitioners to weigh ethical concerns against each other in selecting the best evaluation practice. With these values parameterized, we add a weighting to each value, to represent differing ethical priorities of teams, or regulatory requirements on particular ethical values.

Thus, parameterizing values by $j$, with weights $w_j$, the best evaluation practice for a team would solve:
\begin{equation}
\text{max}_{d\in \mathcal{D}}\mathbb{E}(\mathit{IG}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))
\end{equation}

\subsection{Discussion and Implications}
\hari{I would keep the two tables and fold it into the previous sub-section, I dont think we need to have discussion and implications here}
\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.45\linewidth}|p{0.35\linewidth}|p{0.2\linewidth}|}
        \hline
        \textbf{Utility Framing} & \textbf{Properties} & \textbf{Motivating questions and considerations} \\
        \hline
         $\textit{choose best } d \in D$ & Selecting the best evaluation & \emph{What is our testing goal, what options do we have for evaluation frameworks, and what would they look like?} \\
        \hline
        $\textit{choose best } d \in D \textit{ s.t. } \textit{cost} (d)\leq \textit{resources}$& Evaluations are cost constrained & \emph{What are our resource limitations for evaluating our system?} \\
        \hline
        $u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$
& The best evaluation has the highest utility & \emph{How can I define the best evaluation framework and compare between options?}\\
        \hline
        $\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{such that cost}(d) \leq \textit{resources}$
& Information gain and ethical harm & \emph{What information do I hope to gain and what ethical harms could I cause?} \\
        \hline
         $\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$& Expectation of information gain and ethical harm & \emph{Have I accounted for potential ethical harm or information gain in the future? Have I accounted for disparate impact by population?} \\
        \hline
        $\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$& Ethical harm composed of ethical values & \emph{Which ethical values am I prioritizing, or what regulatory requirements for ethics do I need to satisfy?} \\
        \hline
    \end{tabular}
    \caption{Summary of properties of deciding to use an ethical evaluation that, when taken together, lead to a single utility model framing the costs, benefits, and resource constraints for a team's decision making. Although the order in which these are listed increase in detail, this is for the purpose of describing the setting, and do not need to be considered in this order. }
    \label{tab:tab1}
\end{table}


\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.2\linewidth}|p{0.35\linewidth}|p{0.45\linewidth}|}
        \hline
        \textbf{Notation} & \textbf{Definition} & \textbf{Meaning} \\
        \hline
         ${d \in D}$ & Evaluation choices & The set of possible evaluation methods is D and we are aiming to choose the d that yields maximium utility \\
        \hline
        $\mathbb{E}(\textit{IG}(d))$& Expected benefit in utility & Expected information gain from evaluation practice d. \\
        \hline
        $\mathbb{E}(\textit{EH}_j(d))$& Expected cost in utility & Expected ethical harm of decision d across value j \\
        \hline
        $j$ & Specific ethical value & Parameterizes ethical value concerns \\
        \hline
         $\textit{cost}(d) \leq \textit{resources}$& Resource constraints to testing & Limits to evaluation processes that fit budget \\
        \hline
        $w_j$ & value importance & weight of particular value concern, imposed by priority or regulation \\
        \hline

    \end{tabular}
    \caption{Notation guide to Equation 1, which serves to illustrate the components and tradeoffs of a team's decision to select an ethical evaluation practice.}
    \label{tab:tab2}
\end{table}


We have described, in the section above, the key properties of practitioners' decision making when selecting an ethical evaluation practice. Combining these properties into a single equation, Equation 1 (with notation guide in Table 2), we see that a best evaluation practice is chosen after considering the information gained from the practice, potential ethical harms, and is limited by the resources available. In Table 1, we combine these properties with suggested questions a team might ask itself in the process of formulating this decision making process.

In the next section, we will discuss cases of teams that have utilized this cost-benefit framework, and, in discussing analagous domains, we will cover the potential mitigations that strengthen ethical value considerations in machine learning. 

% Defend why this is a good model, why we care about max utility, how can we think about info gain and evaluation, why did we decide not to consider time. Walk through formulation and get them to buy in. Make sure a person who is new will be able to understand. Self contained. Come up with list of cases for section 4, flesh out the model some more. define what tradeoff is, why we need it, elaborate on formulation. Convince them it is useful. 


%\textbf{Model Implications to improve ethical ML}
% Continuing the framing described, we now discuss implications this analogy has for ways to improve the ethicality of machine learning systems. \textbf{Mitigation 1: Better tests eliminate uncertainty} IRB checks on expectation of ethical harm.  \textbf{Mitigation 2: Add constraints} Increase costs to ethical harm by creating regulation driving up weight on ethical harm.  In the next section, we will discuss ways in which these weights, if enforced by regulation, can be used to ensure ethical evaluation practices. The optimization is also subject to the cost constraints of the evaluation, as teams are bind by infeasibility of doing every possible evaluation on a system.  \textbf{Mitigation 3: Create incentives for earnings to vary with values} Information gain or resources can vary with ethical harm. 







We show how ethical values, and other practical needs of practitioners, are considered when selecting best evaluation practices for ML systems. In illustrating the discussion teams have, we introduce a novel utility based framework that shows the interaction and tradeoffs between ethics and information gained in performing evaluations. 





Here, we draw a distinction between values, evaluations, and metrics, as defined in other literature, in order to use these terms in subsequent sections with clarity and guide further discussion. \jessica{this is more wordy than it needs to be - makes things harder to parse over more terse statements}


% Practitioners engage in evaluation by performing \textit{tests}. A test is any activity intended to detect the differences between the existing and required behaviors of an ML system~\cite{zhang2020machine}. A test executes and measures the performance of a machine learning model according to a particular evaluation metric \cite{hutchinson2022evaluation}. 

%Tests and metrics assesses the performance of a model across specific \textit{values}–the aspects of a system which practitioners are interested in measuring. For instance, engineers may assess for properties like fairness, robustness, or accuracy. 

% Second, an ML test is engineered via an evaluation \textit{workflow}–the method by which engineers execute the test. In many cases, a workflow may consist of building a validation dataset and evaluating the model on this validation set. However, a workflow could also consist of interviews with downstream users regarding their experience using the model. Finally, every ML test produces an \textit{outcome}–the product of the workflow. For most workflows, the outcome will be a metric which numerically captures the property.

% As proposed evaluation practices may be highly application specific and non-standardized, we formalize the notion of an \textit{evaluation decision}–any choice made by a practitioner in the decision or execution of an evaluation. Evaluation decisions can pertain to  properties–under a constrained budget, an engineer may have to choose which values to prioritize, such as whether to evaluate a model for fairness or robustness. Evaluation decisions also arise in the construction of workflows. In annotating labelled test sets for example, practitioners must decide on how many different annotations they would like for each sample. A particular evaluation process may involve choosing one or many evaluation metrics to measure, as part of a decision of which metrics best serve values or ideals. Evaluation decisions are so pervasive that prior work has observed that practitioners can suffer from a ``paradox of choice'' when it comes to deciding how to perform evaluation~\cite{goel2021robustness}.




\textbf{Evaluating the Ethical Values of ML Systems}. More disparate than the other two relevant bodies of literature is a broad set of work that focuses on the ethicality of machine learning systems. \jessica{is it that easy to separate ethics? like isn't a choice to prioritize accuracy ethical in some sense, because you're minimizing bad outcomes as population level?} Existing work characterizes principles and values that machine learning systems should adhere to, and questions goals of deployed systems. Evaluation processes and metrics assess the performance of a model across specific \textit{values}, as values are aspects of a system which practitioners are interested in measuring. For instance, engineers may use metrics to measure achievement of values, such as fairness, robustness, or accuracy. \jessica{again im not sure there's a clear distinction between the values you mean here and the values that lead us to use more conventional metrics}

As an example to illustrate the differences between these three types of research areas, the ethics literature would ask: `Why would we use facial recognition technology in surveillance?'. In contrast, the metrics literature would ask about the best metric for evaluating the bias vs the effectiveness of the model. Meanwhile, evaluation questions would ask what an effective test of the facial recognition technology would be.\jessica{aren't these all evaluation questions?} We proceed by discussing the importance of bridging these disparate fields, and prompt teams to think about ethics in their evaluation methods, rather than exclusively considering the ethical values of their end products.

\jessica{How we chose the categories in this section is hard for me to understand. Worth considering how exactly they set up the rest of the paper. It also feels like we're talking very broadly here, and the ML evaluations subsection is particularly generic/hard to separate from ethical values.}

\neha{
\subsection{Software Lifecycle}

\cite{ashmore2021assuring} surveys ways in which machine learning models are determined to be safe, referring to these as assurance methods, at various stages of the machine learning lifecycle. When they define the machine learning lifecycle, they discuss 3 initial stages: data management, model learning, and model verification, in which models are produced. The final stage they define is model deployment. Every model is spiraling through these stages over its lifecycle, as models can be updated after deployment or with new data samples gathered. The authors further describe key disederata for each of these stages of the lifecycle. For the data management stage, they are relvance, completeness, balance, and accuracy. For the model learning stage, desiderata include whether the assurance method is performant, robust, resuable, and interpretable. 

When \cite{zhang2020machine} discuss the role of testing in ML systems, they describe a circular model in which both online and offline testing happen, and the user cycles through: historical data, prototyping, offline testing, deployment, user interaction, predictions, online testing, adapted model, online data. The authors describe the testing properties as happening only in the online and offline testing phases of the cycle, and discuss questions such as \emph{why} we test models. The ethical \emph{why} question should go beyond what properties a model can be tested for, and should be posed at stages of the lifecycle beyond testing, such as the security and privacy of data management systems. 

In \cite{ashurst2022disentangling}, the authors discuss ethics in ML research. Research precedes deployment of live systems, and considerations they discuss, such as treatment of workers contributing to research that influences a deployed model, should be considered part of a deployed systems' lifecycle.
}

\subsection{Information Gained in Testing}

\subsubsection{Internal validity}
In social science, \textit{internal validity} measures the methodological correctness of an experimental study, and the extent to which its findings reflect true phenomenon in the studied data~\cite{drost2011validity}. In the context of evaluation, internal validity corresponds to the correctness of an evaluation output. For instance, suppose engineers test a model on ImageNet and report a test set accurate rate of 99\%. This test would be internally valid if the model was actually correct on 99\% of the test set images. \jessica{I don't think this is a very clear way to describe this. A better description to capture threats to internal validity is to talk about how we want the estimates we get on our particular sample to be good predictions of what we'd get on new test sets from the same distribution. I recommend seeing Liao et al. are we learning yet paper, where they define threats to internal and external validity in ML}

The internal validity of a test can be threatened in many different ways. The engineers may have accidentally \sout{trained the model on samples from the ImageNet} \jessica{used information from the} test set \jessica{in training their model}, resulting in train-test leakage~\cite{shankar2022}. \jessica{I would replace Shankar cite with Sayash Kapoor taxonomy of leakage paper} Alternatively, crowdworkers may have misunderstood the label schema, thereby assigning incorrect labels to the test samples~\cite{northcutt2021pervasive, chen2022, gordon2021disagreement}. \jessica{Prev sentence also seems too specific if we are talking about general issues. Would say 'If the measurements used in training and testing (i.e., labels) are themselves erroneous, reported expectations test performance will not capture what they are intended to. } Internal validity can be threatened by software bugs, which lead to incorrect reporting of metrics (e.g., ~\cite{allevitan2021}), \jessica{or researchers continuing to optimize their method after test set evaluation}~\cite{hosseini2020tried} 
\sout{Errors have already been identified in different aspects of popular machine learning libraries.} \jessica{Threats to interval validity often arise from researcher-degrees-of-freedom in defining the learning problem in ways that artificially inflate performance estimates such that their intended meaning no longer holds}~\cite{hofman2023}.

\subsubsection{External validity}
\textit{External validity} corresponds to the generalizability of observations: the extent to which findings on a studied context or population hold for different contexts or populations~\cite{drost2011validity}. In the context of \jessica{machine learning} evaluation,  \jessica{the most pressing form of threat to} external validity \sout{captures the extent to which} \jessica{is that} performance on evaluation tests \sout{are} \jessica{will not be} consistent with performance on actual domain data \jessica{due to distribution shift}. \jessica{what is actual domain data? I would say 'deployment population an} Since the samples a model predicts labels for during deployment will always be different then the samples used in evaluation tests, \jessica{what is "will always be different"? I think the language is too ambiguous; need to be precise when talking about these kinds of threats} there is a risk that conclusions drawn about performance from test data will be incorrectly applied to deployment data.

Prior work has extensively documented settings in which evaluation tests lack external validity. \jessica{if we mention prior work we should be adding cites; in general this section of paper might benefit from more references} This is common when task data involves long tails, temporally dependent data, or skewed data collection procedures. Problems with external validity can also arise in the choice of metrics. For instance, an evaluation test may rely on metrics that do not appropriately capture the cost of failures in deployment.

\subsubsection{Robustness}

\subsection{Formalizing Values for ML systems} \label{sec:evaluation_dimensions}

\st{We formalize and define a set of values that a team developing a machine learning software product can seek to uphold. We do not seek to provide a comprehensive listing or enumeration of all possible values, instead categorizing and identifying key values based on other literature.}
\jessica{I'm not sure I'd call these formalizations in the current version. They seem like loose verbal definitions. Also wondering how did this set of values get chosen? Are they comprehensive? Paper may need a method section to explain the selection here and for the following section. }

\neha{Hopefully this helps @JH:

A growing body of literature discusses properties that ethical machine learning systems embody, and are tested for embodying. These properties may be discussed in the context of what machine learning systems are tested to accomplish for (as in \cite{zhang2020machine}), or these properties may be discussed in the context of what an ethical machine learning system embodies (as in \cite{jobin2019global}). 

In \cite{zhang2020machine}, the authors propose the following properties as definining \emph{why} machine learning systems are tested: correctness, overfitting, robustness, security, privacy, efficiency, fairness, and interpretability. In \cite{martinez2022software}, the authors offer a metastudy of a decade of studies published and evaluating AI systems, finding that relevent system properties range over various studies, but commonly occuring ones include: safety, correctness, reliability, robustness, fairness, accuracy, safety, consistency, model relevance, security, data privacy, interpretability, ethics and regulation, software structure, testability, maintainbility, performance, risk and uncertainty, economic impact, adaptability, scalability, reusability, and more. Finally, in \cite{jobin2019global}, the authors also offer a global metastudy by geographic location including writing from private companies and governmental agencies, to map principles of ethical AI. They note convergence around transparency, justice and fairness, non-maleficence, responsibility, and privacy, but note broad disparities in the interpretation of these values. They also note some repetitively occurring values of beneficience, freedom and autonomy, and trust.

In the remainder of this section, we discuss many, but not all, of these properties. We emphasize that this is not a comprehensive listing of all properties that a machine learning system may seek to accomplish, and that any group may define these properties somewhat differently. 


}

%Assessing the ethicality of an evaluation requires defining a set of criteria upon which we can measure an evaluation decision. Existing literature on AI ethicality suggests that decisions, systems, and designs can often be evaluated with respect to distinct social, economic, or political values. We refer to these values as \textit{evaluation dimensions}. A single evaluation dimension offers an axis upon which to measure the ethicality of an evaluation decision. Independently, a dimension may weigh in favor of against a particular evaluation decision, depending on whether the decision aligns with the dimension's value. A collection of dimensions act in concert to define a cost/benefit balancing framework. For instance, a particular decision may prioritize certain dimensions over others. In this work, we identify seven evaluation dimensions.

\subsubsection{Harmfulness/Social Impact}
\textit{Harmfulness} measures the extent to which the evaluation workflows and outcomes inflicts an injury on any individual or population.\jessica{are we making this up, or taking from prior definitions? I personally would prefer more careful citation in this section} The law \jessica{what law?} provides a broad interpretation of injury. The most well-known form of injuries are physical, and involve losses of ``life or limb.'' However, injuries may also be dignitary, and considered to affect an individuals' well being or reputation. Such dignitary harms include defamation or the infliction or emotional distress. Finally, injuries may be economic, as they directly deprive individuals of monetary benefits, or deprive them of the opportunity to realize monetary benefits.

Consequently, harm can manifest in evaluation workflows in a variety of ways. Engineers commonly deploy experimental models over users in order to collect actual performance data. Erroneous predictions may result in physical~\cite{siddiqui2022teslas} or economic harms \cite{linkedin} to users. Collecting annotations for certain types of tasks–like content moderation–can result in harms to human labelers~\cite{bbc2020}.

\subsubsection{Interpretability}

\textit{Interpretability} measures the extent to which the outputs of an evaluation test can be understood by the stakeholders in a particular ML application. Interpretability encompasses two principles. First, evaluation tests derive value from providing actionable information to stakeholders. Tests which enable practitioners to better diagnose the source of model errors are preferable to those that don't. Second, evaluation tests derive value as a means by which practitioners can communicate information about performance to relevant stakeholders. When tests involve proprietary data or methods, the ability for stakeholders to understand or contest model performance is thus severely limited. \jessica{prev sentence seems like a very specific example in an otherwise general paragraph}  


Certain evaluation tests involve metrics which are difficult to understand or quantify in absolute terms \cite{xu2018empirical}. Other metrics–while understandable to developers–may be too complex for downstream users to engage with~\todocite{medical imaging metrics}. \yannis{\cite{kaychi2015} shows that even commonly used metrics, such as the F-measure, come with interpretability challenges.} Others have noted that certain evaluations are more likely to induce developer confirmation bias, or that the presentation of a test may significantly impact a developer's understanding of a model~\todocite{work on fairness presentation}. \jessica{so what is the implication of that?} For some applications, model developers have refused to reveal evaluation outputs or protocols due to concerns involving trade secrets~\cite{wexler2018life}. Privacy concerns with past dataset releases~\todocite{Netflix and AOL dataset releases} mean that developers are often hesitant to release internal evaluation datasets.\jessica{how is this interpretability rather than privacy?}

\subsubsection{Privacy}
Broadly, privacy as a value measures the extent to which engineering practices or processes avoid the unnecessary collection of an individual's data or information~\todocite{privacy by design and related literature}. \jessica{isnt it also often about sharing data, not just collection?} In the context of evaluation, privacy preserving tests or workflows are ones which avoid collecting additional information about a user. \jessica{or disclosing sensitive identifying information evaluation.}

Evaluation workflows implicate privacy in different ways. Prior work has noted, for instance, that measuring model fairness or performing disaggregated evaluations often requires collecting additional, sensitive, demographic metadata~\todocite{work on collecting demographic data}. Evaluating models on data from deployment requires collecting and storing user data. This can increase the likelihood for privacy violations, either by engineers, or in data breaches.  

\subsubsection{Fairness}
\jessica{need citations; otherwise reader may wonder how much we're making this up rather than grounding in existing literature. In general this section of paper would read much stronger if we it were about distilling key concerns from the literature, rather than just listing things people care about but not being specific about how we are coming up with this}
The traditional definition of fairness encompasses the extent to which individuals belonging to different subgroups are treated equivalently by a process. In the context of evaluation, fairness measures the extent to which evaluation tests and workflows induce varying outcomes that correlate with subgroup membership. Fairness in evaluation is not about the model's performance on different subgroups, but the extent to which a workflow privileges or harms certain subgroups over others. 

Concerns regarding fairness in evaluation thus usually accompany other dimensions of evaluations. For instance, evaluation harms--through practices like live testing–-may be disproportionately inflicted on certain demographic subgroups. Alternatively, the underrepresentation of subgroups may subject them to increased data collection, resulting in greater privacy violations. For tasks like toxic content detection–where annotations can depend on annotator democraphic characteristics–internal validity concerns can arise for simple-majority vote label aggregation strategies.

\subsubsection{Cultural Sensitivity}

todo: fill in with folder given by Hari. 

\subsubsection{Environmental Impact/Sustainability}

Many AI systems aim to be environmentally friendly, regardless of whether sustainability is a primary aim of the product. Sustainability can be achieved in the energy consumption and resources required at any point during the development lifecycle. Sustainability is a major goal of governments across the world, and their encouragement, as well as consumer sentiment, has made this a goal for many private industries developing ML models as well \cite{eugoals}. \yannis{This reads more like the environmental impact/sustainability of the final model and/or other parts of the development process rather than the environmental impact/sustainability of the model evaluation itself. When I first read the section title, I was thinking more of the environmental impact of setting up the infrastructure for testing, incl. running model inference, the impact of travel for testing that involves physical participation, etc.}

\jessica{is this list supposed to be comprehensive? how was it arrived at? Missing a sense of methodological rigor}

\jessica{thinking about this section after reading more of the paper - I think we are mixing definitions of properties of methods that have instrumental value (as a means to an end) with outcomes (eg harms, monetary costs). I think it would help to split the list into something like Desirable Properties and Outcomes. Things like interpretability and privacy are desirable properties that lead to outcomes like trust, better use of the system, etc in practice. avoiding harms and reducing resource expenditure on the other hand are better thought of as outcomes rather than properties of methods. I think preceding the values section shoudl be a section laying out the fundmantal formalization we are talking about (see my comments in next section)  
}


\subsection{Cost}
\textit{cost} measures the resources required to conduct an evaluation. Machine learning developers always operate under resource constraints, which affect the time, money, and labor that may be devoted towards evaluation. For instance, monetary constraints may restrict the amount of annotations developers may procure for validation data~\todocite{work on efficiently building validation sets}. Constraints on labor availability may restrict the number of engineers capable of focusing on evaluation, requiring more automation and less manual examination of errors~\todocite{work on automatically detecting errors}. Constraints on time may restrict the ability for engineers to run longer-range evaluations.

\subsection{Related works on utility framing in software}
This is not the first body of work framing ML models as providing utility to society, and emphasizing ethical considerations, but other works restrict to discussing a single model's output and social impact. For example, in \cite{corbett2017algorithmic}, the authors provide a definition of immediate utility, which reflects the costs and benefits of a fair decision by a policymaker, notably in the setting of pre-trail bail release decisions. Similarly, in \cite{corbett2018measure}, the utility function reflects a single decision made by a model, such as whether or not to screen an individual for diabetes. In \cite{chohlas2021learning}, a utility function determines the optimal decision making, such as in the decision of providing funded transportation for court appearances. Our framework deviates from these in that we are not focused on the fair output and decisions made by an ML model. Rather, we are focused on the decisions made by a team when developing and deploying a large-scale ML system.

This is also not the first body of work to discuss ML models and utility while emphasizing evaluations. \cite{hutchinson2022evaluation} use a utility function to simplify and discuss framing of an evaluation of a single model's appropriateness for a given application. The motivating philosophy of consequentalism - that actions are good or bad depending on its consequences - also applies here. However, our framing centers on an overall system rather than one model. In broadening the discussion to a teams' model development lifecycle, we are able to incorporate teams' value decisions at all stages of a development lifecycle - including creating, testing, and deploying - rather than just consequences of a single model's use for a particular application. 

\newpage


\end{comment}

==> old/jan_02_relatedwork.tex <==
\section{Background and related work}\label{sec:related_work}




Here, we draw a distinction between values, evaluations, and metrics, as defined in other literature, in order to use these terms in subsequent sections with clarity and guide further discussion. \jessica{this is more wordy than it needs to be - makes things harder to parse over more terse statements}


% Practitioners engage in evaluation by performing \textit{tests}. A test is any activity intended to detect the differences between the existing and required behaviors of an ML system~\cite{zhang2020machine}. A test executes and measures the performance of a machine learning model according to a particular evaluation metric \cite{hutchinson2022evaluation}. 

%Tests and metrics assesses the performance of a model across specific \textit{values}–the aspects of a system which practitioners are interested in measuring. For instance, engineers may assess for properties like fairness, robustness, or accuracy. 

% Second, an ML test is engineered via an evaluation \textit{workflow}–the method by which engineers execute the test. In many cases, a workflow may consist of building a validation dataset and evaluating the model on this validation set. However, a workflow could also consist of interviews with downstream users regarding their experience using the model. Finally, every ML test produces an \textit{outcome}–the product of the workflow. For most workflows, the outcome will be a metric which numerically captures the property.

% As proposed evaluation practices may be highly application specific and non-standardized, we formalize the notion of an \textit{evaluation decision}–any choice made by a practitioner in the decision or execution of an evaluation. Evaluation decisions can pertain to  properties–under a constrained budget, an engineer may have to choose which values to prioritize, such as whether to evaluate a model for fairness or robustness. Evaluation decisions also arise in the construction of workflows. In annotating labelled test sets for example, practitioners must decide on how many different annotations they would like for each sample. A particular evaluation process may involve choosing one or many evaluation metrics to measure, as part of a decision of which metrics best serve values or ideals. Evaluation decisions are so pervasive that prior work has observed that practitioners can suffer from a ``paradox of choice'' when it comes to deciding how to perform evaluation~\cite{goel2021robustness}.

\textbf{Machine learning evaluation metrics.} A large body of work focuses on defining and motivating metrics for evaluation. These are usually quantified aspects of a model’s performance that can be measured and reported by practitioners. For instance, beyond simply accuracy, developers may seek to measure a model's fairness, robustness, interpretability, or capacity for misuse. In service of these goals, related work has developed, and studied the tradeoffs, of different metrics. There is a continuous evolution of research in this field as machine learning paradigms also evolve; For instance, a growing literature covers the need for quantifying generative models in terms of their toxicity, bias, and factual correctness.

\textbf{Machine Learning Evaluations.} In support of the pursuit of these goals, a growing body of work creates more comprehensive methods with which to evaluate models, rather than providing a singular empirical metric or set of metrics. Evaluation is the process by which practitioners detect differences between desired and actual model behavior~\cite{zhang2020machine}. It is a process yielding an empirical assessment of model properties \cite{shevlane2023model}. \jessica{seems like previous two sentences should go first in this section, like before metrics?}
%These provide practitioners a standardized worksheet approach with which to evaluate models, with many focused on a single concrete goal (eg privacy), and others taking a more holistic view, seeking to provide practitioners with a means of balancing multiple forms of evaluation. 
These provide valuable transparency for practitioners by establishing a common setting and add ease to communication. A number of evaluation methods pre-deployment, such as A/B testing or live testing, \jessica{isn't A/B testing usually done live?} are common practice across institutions and domains. Other mechanisms, to aid evaluation ex-post deployment, such as bug bounty challenges, \jessica{not familiar with what this is} provide infrastructure to support stakeholder feedback.
A particular evaluation process may involve choosing one or many evaluation metrics to measure, as part of a decision of which metrics best serve values or ideals. Evaluation decisions are so pervasive that prior work has observed that practitioners can suffer from a ``paradox of choice'' when it comes to deciding how to perform evaluation~\cite{goel2021robustness}.


\textbf{Evaluating the Ethical Values of ML Systems}. More disparate than the other two relevant bodies of literature is a broad set of work that focuses on the ethicality of machine learning systems. \jessica{is it that easy to separate ethics? like isn't a choice to prioritize accuracy ethical in some sense, because you're minimizing bad outcomes as population level?} Existing work characterizes principles and values that machine learning systems should adhere to, and questions goals of deployed systems. Evaluation processes and metrics assess the performance of a model across specific \textit{values}, as values are aspects of a system which practitioners are interested in measuring. For instance, engineers may use metrics to measure achievement of values, such as fairness, robustness, or accuracy. \jessica{again im not sure there's a clear distinction between the values you mean here and the values that lead us to use more conventional metrics}

As an example to illustrate the differences between these three types of research areas, the ethics literature would ask: `Why would we use facial recognition technology in surveillance?'. In contrast, the metrics literature would ask about the best metric for evaluating the bias vs the effectiveness of the model. Meanwhile, evaluation questions would ask what an effective test of the facial recognition technology would be.\jessica{aren't these all evaluation questions?} We proceed by discussing the importance of bridging these disparate fields, and prompt teams to think about ethics in their evaluation methods, rather than exclusively considering the ethical values of their end products.

\jessica{How we chose the categories in this section is hard for me to understand. Worth considering how exactly they set up the rest of the paper. It also feels like we're talking very broadly here, and the ML evaluations subsection is particularly generic/hard to separate from ethical values.}

\neha{
\subsection{Software Lifecycle}

\cite{ashmore2021assuring} surveys ways in which machine learning models are determined to be safe, referring to these as assurance methods, at various stages of the machine learning lifecycle. When they define the machine learning lifecycle, they discuss 3 initial stages: data management, model learning, and model verification, in which models are produced. The final stage they define is model deployment. Every model is spiraling through these stages over its lifecycle, as models can be updated after deployment or with new data samples gathered. The authors further describe key disederata for each of these stages of the lifecycle. For the data management stage, they are relvance, completeness, balance, and accuracy. For the model learning stage, desiderata include whether the assurance method is performant, robust, resuable, and interpretable. 

When \cite{zhang2020machine} discuss the role of testing in ML systems, they describe a circular model in which both online and offline testing happen, and the user cycles through: historical data, prototyping, offline testing, deployment, user interaction, predictions, online testing, adapted model, online data. The authors describe the testing properties as happening only in the online and offline testing phases of the cycle, and discuss questions such as \emph{why} we test models. The ethical \emph{why} question should go beyond what properties a model can be tested for, and should be posed at stages of the lifecycle beyond testing, such as the security and privacy of data management systems. 

In \cite{ashurst2022disentangling}, the authors discuss ethics in ML research. Research precedes deployment of live systems, and considerations they discuss, such as treatment of workers contributing to research that influences a deployed model, should be considered part of a deployed systems' lifecycle.
}

\subsection{Information Gained in Testing}

\subsubsection{Internal validity}
In social science, \textit{internal validity} measures the methodological correctness of an experimental study, and the extent to which its findings reflect true phenomenon in the studied data~\cite{drost2011validity}. In the context of evaluation, internal validity corresponds to the correctness of an evaluation output. For instance, suppose engineers test a model on ImageNet and report a test set accurate rate of 99\%. This test would be internally valid if the model was actually correct on 99\% of the test set images. \jessica{I don't think this is a very clear way to describe this. A better description to capture threats to internal validity is to talk about how we want the estimates we get on our particular sample to be good predictions of what we'd get on new test sets from the same distribution. I recommend seeing Liao et al. are we learning yet paper, where they define threats to internal and external validity in ML}

The internal validity of a test can be threatened in many different ways. The engineers may have accidentally \sout{trained the model on samples from the ImageNet} \jessica{used information from the} test set \jessica{in training their model}, resulting in train-test leakage~\cite{shankar2022}. \jessica{I would replace Shankar cite with Sayash Kapoor taxonomy of leakage paper} Alternatively, crowdworkers may have misunderstood the label schema, thereby assigning incorrect labels to the test samples~\cite{northcutt2021pervasive, chen2022, gordon2021disagreement}. \jessica{Prev sentence also seems too specific if we are talking about general issues. Would say 'If the measurements used in training and testing (i.e., labels) are themselves erroneous, reported expectations test performance will not capture what they are intended to. } Internal validity can be threatened by software bugs, which lead to incorrect reporting of metrics (e.g., ~\cite{allevitan2021}), \jessica{or researchers continuing to optimize their method after test set evaluation}~\cite{hosseini2020tried} 
\sout{Errors have already been identified in different aspects of popular machine learning libraries.} \jessica{Threats to interval validity often arise from researcher-degrees-of-freedom in defining the learning problem in ways that artificially inflate performance estimates such that their intended meaning no longer holds}~\cite{hofman2023}.

\subsubsection{External validity}
\textit{External validity} corresponds to the generalizability of observations: the extent to which findings on a studied context or population hold for different contexts or populations~\cite{drost2011validity}. In the context of \jessica{machine learning} evaluation,  \jessica{the most pressing form of threat to} external validity \sout{captures the extent to which} \jessica{is that} performance on evaluation tests \sout{are} \jessica{will not be} consistent with performance on actual domain data \jessica{due to distribution shift}. \jessica{what is actual domain data? I would say 'deployment population an} Since the samples a model predicts labels for during deployment will always be different then the samples used in evaluation tests, \jessica{what is "will always be different"? I think the language is too ambiguous; need to be precise when talking about these kinds of threats} there is a risk that conclusions drawn about performance from test data will be incorrectly applied to deployment data.

Prior work has extensively documented settings in which evaluation tests lack external validity. \jessica{if we mention prior work we should be adding cites; in general this section of paper might benefit from more references} This is common when task data involves long tails, temporally dependent data, or skewed data collection procedures. Problems with external validity can also arise in the choice of metrics. For instance, an evaluation test may rely on metrics that do not appropriately capture the cost of failures in deployment.

\subsubsection{Robustness}

\subsection{Formalizing Values for ML systems} \label{sec:evaluation_dimensions}

\st{We formalize and define a set of values that a team developing a machine learning software product can seek to uphold. We do not seek to provide a comprehensive listing or enumeration of all possible values, instead categorizing and identifying key values based on other literature.}
\jessica{I'm not sure I'd call these formalizations in the current version. They seem like loose verbal definitions. Also wondering how did this set of values get chosen? Are they comprehensive? Paper may need a method section to explain the selection here and for the following section. }

\neha{Hopefully this helps @JH:

A growing body of literature discusses properties that ethical machine learning systems embody, and are tested for embodying. These properties may be discussed in the context of what machine learning systems are tested to accomplish for (as in \cite{zhang2020machine}), or these properties may be discussed in the context of what an ethical machine learning system embodies (as in \cite{jobin2019global}). 

In \cite{zhang2020machine}, the authors propose the following properties as definining \emph{why} machine learning systems are tested: correctness, overfitting, robustness, security, privacy, efficiency, fairness, and interpretability. In \cite{martinez2022software}, the authors offer a metastudy of a decade of studies published and evaluating AI systems, finding that relevent system properties range over various studies, but commonly occuring ones include: safety, correctness, reliability, robustness, fairness, accuracy, safety, consistency, model relevance, security, data privacy, interpretability, ethics and regulation, software structure, testability, maintainbility, performance, risk and uncertainty, economic impact, adaptability, scalability, reusability, and more. Finally, in \cite{jobin2019global}, the authors also offer a global metastudy by geographic location including writing from private companies and governmental agencies, to map principles of ethical AI. They note convergence around transparency, justice and fairness, non-maleficence, responsibility, and privacy, but note broad disparities in the interpretation of these values. They also note some repetitively occurring values of beneficience, freedom and autonomy, and trust.

In the remainder of this section, we discuss many, but not all, of these properties. We emphasize that this is not a comprehensive listing of all properties that a machine learning system may seek to accomplish, and that any group may define these properties somewhat differently. 


}

%Assessing the ethicality of an evaluation requires defining a set of criteria upon which we can measure an evaluation decision. Existing literature on AI ethicality suggests that decisions, systems, and designs can often be evaluated with respect to distinct social, economic, or political values. We refer to these values as \textit{evaluation dimensions}. A single evaluation dimension offers an axis upon which to measure the ethicality of an evaluation decision. Independently, a dimension may weigh in favor of against a particular evaluation decision, depending on whether the decision aligns with the dimension's value. A collection of dimensions act in concert to define a cost/benefit balancing framework. For instance, a particular decision may prioritize certain dimensions over others. In this work, we identify seven evaluation dimensions.

\subsubsection{Harmfulness/Social Impact}
\textit{Harmfulness} measures the extent to which the evaluation workflows and outcomes inflicts an injury on any individual or population.\jessica{are we making this up, or taking from prior definitions? I personally would prefer more careful citation in this section} The law \jessica{what law?} provides a broad interpretation of injury. The most well-known form of injuries are physical, and involve losses of ``life or limb.'' However, injuries may also be dignitary, and considered to affect an individuals' well being or reputation. Such dignitary harms include defamation or the infliction or emotional distress. Finally, injuries may be economic, as they directly deprive individuals of monetary benefits, or deprive them of the opportunity to realize monetary benefits.

Consequently, harm can manifest in evaluation workflows in a variety of ways. Engineers commonly deploy experimental models over users in order to collect actual performance data. Erroneous predictions may result in physical~\cite{siddiqui2022teslas} or economic harms \cite{linkedin} to users. Collecting annotations for certain types of tasks–like content moderation–can result in harms to human labelers~\cite{bbc2020}.

\subsubsection{Interpretability}

\textit{Interpretability} measures the extent to which the outputs of an evaluation test can be understood by the stakeholders in a particular ML application. Interpretability encompasses two principles. First, evaluation tests derive value from providing actionable information to stakeholders. Tests which enable practitioners to better diagnose the source of model errors are preferable to those that don't. Second, evaluation tests derive value as a means by which practitioners can communicate information about performance to relevant stakeholders. When tests involve proprietary data or methods, the ability for stakeholders to understand or contest model performance is thus severely limited. \jessica{prev sentence seems like a very specific example in an otherwise general paragraph}  


Certain evaluation tests involve metrics which are difficult to understand or quantify in absolute terms \cite{xu2018empirical}. Other metrics–while understandable to developers–may be too complex for downstream users to engage with~\todocite{medical imaging metrics}. \yannis{\cite{kaychi2015} shows that even commonly used metrics, such as the F-measure, come with interpretability challenges.} Others have noted that certain evaluations are more likely to induce developer confirmation bias, or that the presentation of a test may significantly impact a developer's understanding of a model~\todocite{work on fairness presentation}. \jessica{so what is the implication of that?} For some applications, model developers have refused to reveal evaluation outputs or protocols due to concerns involving trade secrets~\cite{wexler2018life}. Privacy concerns with past dataset releases~\todocite{Netflix and AOL dataset releases} mean that developers are often hesitant to release internal evaluation datasets.\jessica{how is this interpretability rather than privacy?}

\subsubsection{Privacy}
Broadly, privacy as a value measures the extent to which engineering practices or processes avoid the unnecessary collection of an individual's data or information~\todocite{privacy by design and related literature}. \jessica{isnt it also often about sharing data, not just collection?} In the context of evaluation, privacy preserving tests or workflows are ones which avoid collecting additional information about a user. \jessica{or disclosing sensitive identifying information evaluation.}

Evaluation workflows implicate privacy in different ways. Prior work has noted, for instance, that measuring model fairness or performing disaggregated evaluations often requires collecting additional, sensitive, demographic metadata~\todocite{work on collecting demographic data}. Evaluating models on data from deployment requires collecting and storing user data. This can increase the likelihood for privacy violations, either by engineers, or in data breaches.  

\subsubsection{Fairness}
\jessica{need citations; otherwise reader may wonder how much we're making this up rather than grounding in existing literature. In general this section of paper would read much stronger if we it were about distilling key concerns from the literature, rather than just listing things people care about but not being specific about how we are coming up with this}
The traditional definition of fairness encompasses the extent to which individuals belonging to different subgroups are treated equivalently by a process. In the context of evaluation, fairness measures the extent to which evaluation tests and workflows induce varying outcomes that correlate with subgroup membership. Fairness in evaluation is not about the model's performance on different subgroups, but the extent to which a workflow privileges or harms certain subgroups over others. 

Concerns regarding fairness in evaluation thus usually accompany other dimensions of evaluations. For instance, evaluation harms--through practices like live testing–-may be disproportionately inflicted on certain demographic subgroups. Alternatively, the underrepresentation of subgroups may subject them to increased data collection, resulting in greater privacy violations. For tasks like toxic content detection–where annotations can depend on annotator democraphic characteristics–internal validity concerns can arise for simple-majority vote label aggregation strategies.

\subsubsection{Cultural Sensitivity}

todo: fill in with folder given by Hari. 

\subsubsection{Environmental Impact/Sustainability}

Many AI systems aim to be environmentally friendly, regardless of whether sustainability is a primary aim of the product. Sustainability can be achieved in the energy consumption and resources required at any point during the development lifecycle. Sustainability is a major goal of governments across the world, and their encouragement, as well as consumer sentiment, has made this a goal for many private industries developing ML models as well \cite{eugoals}. \yannis{This reads more like the environmental impact/sustainability of the final model and/or other parts of the development process rather than the environmental impact/sustainability of the model evaluation itself. When I first read the section title, I was thinking more of the environmental impact of setting up the infrastructure for testing, incl. running model inference, the impact of travel for testing that involves physical participation, etc.}

\jessica{is this list supposed to be comprehensive? how was it arrived at? Missing a sense of methodological rigor}

\jessica{thinking about this section after reading more of the paper - I think we are mixing definitions of properties of methods that have instrumental value (as a means to an end) with outcomes (eg harms, monetary costs). I think it would help to split the list into something like Desirable Properties and Outcomes. Things like interpretability and privacy are desirable properties that lead to outcomes like trust, better use of the system, etc in practice. avoiding harms and reducing resource expenditure on the other hand are better thought of as outcomes rather than properties of methods. I think preceding the values section shoudl be a section laying out the fundmantal formalization we are talking about (see my comments in next section)  
}


\subsection{Cost}
\textit{cost} measures the resources required to conduct an evaluation. Machine learning developers always operate under resource constraints, which affect the time, money, and labor that may be devoted towards evaluation. For instance, monetary constraints may restrict the amount of annotations developers may procure for validation data~\todocite{work on efficiently building validation sets}. Constraints on labor availability may restrict the number of engineers capable of focusing on evaluation, requiring more automation and less manual examination of errors~\todocite{work on automatically detecting errors}. Constraints on time may restrict the ability for engineers to run longer-range evaluations.

\subsection{Related works on utility framing in software}
This is not the first body of work framing ML models as providing utility to society, and emphasizing ethical considerations, but other works restrict to discussing a single model's output and social impact. For example, in \cite{corbett2017algorithmic}, the authors provide a definition of immediate utility, which reflects the costs and benefits of a fair decision by a policymaker, notably in the setting of pre-trail bail release decisions. Similarly, in \cite{corbett2018measure}, the utility function reflects a single decision made by a model, such as whether or not to screen an individual for diabetes. In \cite{chohlas2021learning}, a utility function determines the optimal decision making, such as in the decision of providing funded transportation for court appearances. Our framework deviates from these in that we are not focused on the fair output and decisions made by an ML model. Rather, we are focused on the decisions made by a team when developing and deploying a large-scale ML system.

This is also not the first body of work to discuss ML models and utility while emphasizing evaluations. \cite{hutchinson2022evaluation} use a utility function to simplify and discuss framing of an evaluation of a single model's appropriateness for a given application. The motivating philosophy of consequentalism - that actions are good or bad depending on its consequences - also applies here. However, our framing centers on an overall system rather than one model. In broadening the discussion to a teams' model development lifecycle, we are able to incorporate teams' value decisions at all stages of a development lifecycle - including creating, testing, and deploying - rather than just consequences of a single model's use for a particular application. 

\newpage

==> old/jan_03_framework.tex <==
\section{Considering Ethics in Selecting Evaluation Frameworks}

We show how ethical values and other practical needs of practitioners are considered when selecting best evaluation practices for ML systems. In illustrating the discussion teams have, we introduce a novel utility based framework that shows the interaction and tradeoffs between ethics and information gained in performing evaluations. 
% state how we came up with this and the fact that this is novel.  

\subsection{Sketch of Utility Framing of Best Evaluation Practice} \hari{Desiderata for ethical/optimal/responsible? evaluation practice}

We step \hari{formulate?} through six illustrative properties of a team's decision\hari{unless we know this from literature, I wouldn't frame it as team's decisions, keep it at a high level, we identified.. } making when selecting an evaluation practice for ML systems, building to a single utility model that captures the advantages and disadvantages of a best evaluation practice. For each of the six properties, we discuss its necessity, the underlying assumptions, and its implications. We close by discussing how the properties interlink to create a model of the best \hari{do we have a definition of "best" in related work, or are we defining what best means?} evaluation practice. In representing the multilayered behaviors of teams in these steps, we are able to  clearly define their choices, tradeoffs, and constraints. These steps also will allow us to discuss cases in Section 4, and frame advice for mitigation strategies for the ethical AI industry in Section 5. 

\textbf{Property 1: Selecting a best evaluation out of several alternatives.}
ML development teams have several considerations and options for evaluation practices, including both online and offline testing methods.  Some questions teams might ask themselves in formulating evaluation methods include which desired properties tests should target, or what specific components of a large system need to be tested. The fundamental purpose of an evaluation is to detect differences between desired and actual model behavior, so defining what desired model behavior is is critical \cite{zhang2020machine}. Prior works describe the innumerable evaluation decisions (is d a specific evaluation method, or is it more low level and relates to decisions that needs to be made when planning evaluation?) as leading to a ``paradox of choice" for practitioners deciding how to perform an evaluation \cite{goel2021robustness}. So, the starting point for our utility model of decision making is generating options for evaluation frameworks $D$ and our goal will be:

$$\textit{choose best } d \in D$$

\textbf{Property 2: Evaluations are cost constrained.}
Across the development lifecycle, workers are often ``incentivized by metrics associated with financial gain" \cite{ali2023walking}. For ML testing specifically, one of the fundamental challenges is cost constraints, with teams often considering options for reducing costs of tests via methods such as test prioritisation, in which inputs generated for tests are limited to inputs that are most indicative of problematic behavior \cite{zhang2020machine}. Thus, our decision function is restricted by resources available. We represent this as:

$$\textit{choose best } d \in D \textit{ such that cost(d)}\leq \textit{resources}$$

\textbf{Property 3: The best evaluation method has the highest utility.}
An evaluation practice can be good or bad depending on its consequences, and the best evaluation practice can be chosen based on the utility of the evaluation practice. This is in following of the consequentialism philosophy - that actions are good or bad depending on its consequences - which is used to argue that the goal of a ML model evaluation is to understand how a model will interact with society, and establish that this ``understanding" can be represented as utility \cite{hutchinson2022evaluation}. The fair ML literature has established the representation of ML models as providing a utility, to consider decision making regarding model choice as a function of costs and benefits \cite{corbett2017algorithmic, corbett2018measure, chohlas2021learning}. Here, rather than utility maximization representing the decision of a team in selecting a model, the utility maximization problem represents the decisions made by a team in developing and deploying a large-scale ML system \hari{should this just be evaluation, a step in developing and deploying...}.

We represent the best decision of evaluation practice for the team as the decision with the highest utility. The utility function maps each decision option the team is considering to a single numeric value (with unit ``utils"), and selecting the best decision equates to selecting the decision with the highest utility. An evaluation framework $d^*$ is the optimal decision if it is the utility maximizing decision, indicated as:

$$u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$$


\textbf{Property 4: Utility is composed of gain and loss, in the form of of information and ethical harms.}
The goal of machine learning testing is to learn about system performance in order to detect differences between desired and actual model behavior \cite{zhang2020machine}. We characterize the information we learned from a test as the \emph{gain} from the evaluation process. On the other hand, concerns about ethics of machine learning systems include concerns about the ethics of evaluation practices, because operationalizing the evaluation process may lead practitioners to make sacrifices across ethical values. This will be further exemplified in a series of cases in Section 4. We break the utility function into a cost-benefit function, with the information gain representing the utility benefit, and potential ethical harm representing the utility cost. Thus, our decision of the optimal evaluation framework would solve:

$$\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{such that cost}(d) \leq \textit{resources}$$

\textbf{Property 5: Information gain and ethical harm are in expectation}. 
Thus far, we have chosen to represent the decision of the best evaluation framework as choosing an evaluation with the highest numeric value of utility, and we now need to acknowledge that in doing so, costs and benefits in the utility function need to be represented as average expected values. This expectation allows us to illustrate three things: (1) In several instances, ethical values are difficult to prove or quantify \cite{ali2023walking}, as is information gain. (2) There are several instances of models that differ in social impact across groups, notably underrepresented groups. The estimate of expected ``ethical harm" can be considered an average of harm across several individuals who experience disparate impact from the models \cite{hutchinson2022evaluation}. (3) We account for likelihood of risks over time. In following the consequentialism argument, utility corresponds with impact \cite{hutchinson2022evaluation}. Ethical harm of an evaluation may not be guaranteed but may have some likelihood of occurring (for example, an evaluation that may carry risk of potential privacy leaks at some point in the future, but is not guaranteed to today). For these reasons, we adjust our notation and use the function $\mathit{IG}(d)$ for information gain, the function $\mathit{EH}(d)$ for ethical harm of the evaluation, and now our optimal decision of evaluation framework would solve:

$$\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$$


\textbf{Property 6: Ethical harm is composed of weighted ethical values.}
Ethical values need to be accounted for independently of one another in the utility function, for two reasons. (1) It is obvious that not all ethical values are applicable in all settings -- for example, there may be applications where privacy is not a concern because only public data is used, or cultural sensitivity is not a concern because individual data is not used. (2) There is an established tradeoff between some ethical concerns themselves. For example, existing literature has established gains in fairness of a model yield loss of privacy ~\todocite{ashwin?}. By parameterizing ethical values in our utility function, we acknowledge the need for model practitioners to weigh ethical concerns against each other in selecting the best evaluation practice. With these values parameterized, we add a weighting to each value, to represent differing ethical priorities of teams, or regulatory requirements on particular ethical values.

Thus, parameterizing values by $j$, with weights $w_j$, the best evaluation practice for a team would solve:
\begin{equation}
\text{max}_{d\in \mathcal{D}}\mathbb{E}(\mathit{IG}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))
\end{equation}

\subsection{Discussion and Implications}
\hari{I would keep the two tables and fold it into the previous sub-section, I dont think we need to have discussion and implications here}
\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.45\linewidth}|p{0.35\linewidth}|p{0.2\linewidth}|}
        \hline
        \textbf{Utility Framing} & \textbf{Properties} & \textbf{Motivating questions and considerations} \\
        \hline
         $\textit{choose best } d \in D$ & Selecting the best evaluation & \emph{What is our testing goal, what options do we have for evaluation frameworks, and what would they look like?} \\
        \hline
        $\textit{choose best } d \in D \textit{ s.t. } \textit{cost} (d)\leq \textit{resources}$& Evaluations are cost constrained & \emph{What are our resource limitations for evaluating our system?} \\
        \hline
        $u(d^*) = \textit{max}_{d \in D}U(d) \textit{ such that cost(d)}\leq \textit{resources}$
& The best evaluation has the highest utility & \emph{How can I define the best evaluation framework and compare between options?}\\
        \hline
        $\textit{max}_{d \in D} (\textit{potential information gain} - \textit{potential ethical harm}) \textit{such that cost}(d) \leq \textit{resources}$
& Information gain and ethical harm & \emph{What information do I hope to gain and what ethical harms could I cause?} \\
        \hline
         $\textit{max}_{d \in D} \mathbb{E}(\textit{IG}(d)) - \mathbb{E}(\textit{EH}(d)) \textit{such that cost}(d) \leq \textit{resources}$& Expectation of information gain and ethical harm & \emph{Have I accounted for potential ethical harm or information gain in the future? Have I accounted for disparate impact by population?} \\
        \hline
        $\textit{max}_{d\in \mathcal{D}}\mathbb{E}(\mathit{IG}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))$& Ethical harm composed of ethical values & \emph{Which ethical values am I prioritizing, or what regulatory requirements for ethics do I need to satisfy?} \\
        \hline
    \end{tabular}
    \caption{Summary of properties of deciding to use an ethical evaluation that, when taken together, lead to a single utility model framing the costs, benefits, and resource constraints for a team's decision making. Although the order in which these are listed increase in detail, this is for the purpose of describing the setting, and do not need to be considered in this order. }
    \label{tab:tab1}
\end{table}


\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.2\linewidth}|p{0.35\linewidth}|p{0.45\linewidth}|}
        \hline
        \textbf{Notation} & \textbf{Definition} & \textbf{Meaning} \\
        \hline
         ${d \in D}$ & Evaluation choices & The set of possible evaluation methods is D and we are aiming to choose the d that yields maximium utility \\
        \hline
        $\mathbb{E}(\textit{IG}(d))$& Expected benefit in utility & Expected information gain from evaluation practice d. \\
        \hline
        $\mathbb{E}(\textit{EH}_j(d))$& Expected cost in utility & Expected ethical harm of decision d across value j \\
        \hline
        $j$ & Specific ethical value & Parameterizes ethical value concerns \\
        \hline
         $\textit{cost}(d) \leq \textit{resources}$& Resource constraints to testing & Limits to evaluation processes that fit budget \\
        \hline
        $w_j$ & value importance & weight of particular value concern, imposed by priority or regulation \\
        \hline

    \end{tabular}
    \caption{Notation guide to Equation 1, which serves to illustrate the components and tradeoffs of a team's decision to select an ethical evaluation practice.}
    \label{tab:tab2}
\end{table}


We have described, in the section above, the key properties of practitioners' decision making when selecting an ethical evaluation practice. Combining these properties into a single equation, Equation 1 (with notation guide in Table 2), we see that a best evaluation practice is chosen after considering the information gained from the practice, potential ethical harms, and is limited by the resources available. In Table 1, we combine these properties with suggested questions a team might ask itself in the process of formulating this decision making process.

In the next section, we will discuss cases of teams that have utilized this cost-benefit framework, and, in discussing analagous domains, we will cover the potential mitigations that strengthen ethical value considerations in machine learning. 

% Defend why this is a good model, why we care about max utility, how can we think about info gain and evaluation, why did we decide not to consider time. Walk through formulation and get them to buy in. Make sure a person who is new will be able to understand. Self contained. Come up with list of cases for section 4, flesh out the model some more. define what tradeoff is, why we need it, elaborate on formulation. Convince them it is useful. 


%\textbf{Model Implications to improve ethical ML}
% Continuing the framing described, we now discuss implications this analogy has for ways to improve the ethicality of machine learning systems. \textbf{Mitigation 1: Better tests eliminate uncertainty} IRB checks on expectation of ethical harm.  \textbf{Mitigation 2: Add constraints} Increase costs to ethical harm by creating regulation driving up weight on ethical harm.  In the next section, we will discuss ways in which these weights, if enforced by regulation, can be used to ensure ethical evaluation practices. The optimization is also subject to the cost constraints of the evaluation, as teams are bind by infeasibility of doing every possible evaluation on a system.  \textbf{Mitigation 3: Create incentives for earnings to vary with values} Information gain or resources can vary with ethical harm. 


==> old/jan_04_dimensions_in_practice.tex <==
\section{Real-World Case Analysis for Evaluation Harms}\label{sec:mlcases}

Our conceptual framework above provides a high-level ``sketch'' of the ethical harms associated with machine learning evaluation, delineating how these harms can affect the overall utility derived from the evaluation process. Here, we aim to further expand on the nature of ethical harm by considering real-world examples of evaluation harm by applying case analysis. Case-based analysis is a process that involves examining previous examples to understand the complexity of the problem or concept~\cite{kolodner1992introduction} and gain nuanced insights into patterns of harm and trade-offs in ML evaluation. This approach is particularly effective in identifying recurring themes and understanding the contextual factors that contribute to these outcomes.
\neha{

In selecting cases to highlight of evaluation practices with ethical harms, we conducted a broad search across scholarly publications and news media. We focused on identifying instances that varied in context, and ethical values associated with the ultimate harm. We also prioritized cases that provided clear insights into potential incurred harms, or direct evidence of ethical harms.

These examples together are not intended to be considered a comprehensive analysis of potentially ethical or unethical evaluation practices within machine learning systems. %Instead, we highlight these with opportunities to create systems that will help mitigate ethical harms from evaluation practices for the machine learning community to consider, in order to move the industry towards balancing compliance and effective development. 
Instead, we use these cases to expand on the nature of ethical harms. For each example, we provide a basic description of the setting, and then discuss a formulation of issues the setting generates within the framework proposed in the previous section, while pointing to specific ethical values impacted by practitioner decisions. Ultimately, we illustrate that broader themes emerge regarding what factors impact the magnitude of ethical harm of system evaluations. These lead to particular questions that we propose practitioners consider in order to better estimate the magnitude of ethical harms in their decision making regarding evaluation practices.

% We conclude by highlighting recurring factors that compose magnitude of ethical harm, and propose practitioners to consider particular questions when making decisions regarding evaluation practices. 


%Here, we discuss the cases to ultimately unpack factors influencing ethical harms as defined in our initial model (equation 1). 
}



\st{In selecting the cases, we focused on identifying instances that varied in context, scale, and ethical values associated with harm. We also prioritized cases that provided clear insights into the evaluation goals and evidence of incurred harms.  We excluded cases in which the ethical harms resulted from full-scale deployment and only included ones that pertained to some form of model or system evaluation. By conducting a broad search across scholarly publications and news media, here we discuss the following cases to unpack the factors influencing ethical harms as defined in our initial model (equation 1). For each example, we provide a basic description of the intermediary decisions a team makes and then discuss a formulation of the trade-offs within the framework proposed in the previous section, pointing to specific values implicated by practitioner decisions.}
\subsection{Case Studies}

\subsubsection{Case 1: Car Crash Incidents from Tesla Autopilot System Testing}

\textbf{Summary:} \neel{California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}, and this program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles ``test drove'' at least four million miles on public roads in California~\cite{bellan2022}. One of the autonomous vehicle systems utilizing is program is the Tesla Autopilot system, which, during training and testing on public roads with other drivers, was involved in several tragic fatal crashes \cite{siddiqui2022}.}








% general statement on live testing ML
\textbf{Ethics and Utility Framing}
We look at the decision to use live testing for evaluation of autonomous vehicles through the lens of the framework established in Section \ref{sec:framework}, discussing both the information gain and the ethical harm composing the utility of the live testing. 

Information gain in live testing has been established in prior literature. In general settings, live testing provides information when it can be used to evaluate performance such as testing performance on real-time rare events. Driving does contain many rare events, which could confuse an autonomous navigation system ~\cite{ackerman2017}. This is because real world roads contain phenomenon that are difficult to simulate in synthetic environments, such as inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. Therefore, testing on live roads allow engineers to study instances of systems returning manual control to the human driver~\cite{banerjee2018}. Studying these interventions allows teams to identify failures in perception or control systems~\cite{wang2020safety}. Additionally, they can interview passengers of the car, and learn more about the smoothness of the ride and identify instances of erratic behavior~\cite{donfro2018}. Therefore, there is information gained from live testing. 

The other part of the utility function, ethical harm, $EH(d)$, appears through the value of harmfulness. As discussed in Property 5, ethical harm is an expectation, capturing likelihood of occurrence. Given that the ethical harm did ultimately occur, it is possible the teams failed to accurately estimate the likelihood of the fatal crashes. Alternatively, it is possible the team didn't prioritize the harmfulness value, via the weighted prioritization discussed in Property 6. 

Ultimately, as the utility of the overall system is composed of both information gain and ethical harm, the tragic deaths and subsequent media backlash \cite{siddiqui2022} implicate that low utility from this evaluation, due to high ethical harms outweighing information gain. The overall utility of the evaluation would be improved with lower ethical harms, which could be achieved through proposals to improve the safety of testing autonomous vehicle systems \cite{burton2017making, li2022safety}.
\neha{todo check all citations}
% Tesla's live evaluation practice aims to yield information gain in training and testing the autonomous driving systems, but the utility of the testing is significantly diminished by the ethical harm to society of harmfulness and diminishing roadway safety, as proven by the tragic deaths that have occurred \cite{siddiqui2022}. Media and researchers have noted the harmfulness of live testing strategies, and have made calls suggesting improving the safety of testing automated driving systems \cite{burton2017making, li2022safety}. Others have suggested techniques to improve safety of systems through actionable testing steps or error detection strategies among others \cite{mohseni2022taxonomy}. %external validity vs safety

%- what are the safety-related harms and how it negatively impact utility
%- does ML have advice for safety considerations, what we know from ML in safety consideration during live testing  

% xx negatively impacting utility, positively through xx. 
% lack of decision support 

\subsubsection{Case 2: Microsoft Tay Livetesting}
\textbf{Summary}
In 2016, Microsoft launched a chatbot, Tay live online. This online live testing and release came after an offline development lifecylce, during which they conducted user studies, and stress-tested the bot under various conditions, to ensure the bot had positive interactions. They hoped to reach a larger userbase to learn and improve Tay when they released it online on Twitter \cite{leemicrosoft}. However, within 24 hours, it needed to be removed from Twitter, because a vulnerability in the model led to inappropriate words and images from the chatbot \cite{wolf2017we}. 

\textbf{Ethics and Utility Framing}
We first look at the offline testing done on Tay, then look at the live testing, drawing on aspects of the framework established in Section \ref{sec:framework}. In discussing both, we note that this illustrates how a single ML system may face decisions about evaluation ethics at multiple points during a system's lifecycle.

When the team performed offline testing on Tay, the information they gained led them to believe that it was ready for online interactions with the public. They did not gain information that included the vulnerability that was exploited to ultimately lead to toxic content \cite{leemicrosoft}. Since information gain is in expectation, per Property 5, there can be a discrepancy between information a team hoped to learn in an evaluation, and what they actually received. %\neha{We do not have information on the potential ethical harms of their offline testing, so I don't comment further on the utility as a sum of gain-loss...}

With the information gained from the offline testing, the team decided the model was ready for live testing and release on Twitter. At the time of release, the teeam did not have awareness of the vulnerability that was later exploited to cause downstream harm \cite{leemicrosoft}. Thus, their decision to evaluate with live testing was unable to accurately estimate potential ethical harms that could occur after release, which is in expectation per Property 5. The ethical harms that ultimately took place are the values of cultural sensitivity, unfairness, and harmfulness, as discussed in Property 4. Having observed these ethical harms, critics of the release say that the release of Tay is one of many instances in which the technology industry underweighed potential ethical harm \cite{wolf2017we}. It is possible that higher prioritization of certain weight parameters discussed in Property 6 would have led the team to decide the potential ethical harm was too high to yield high utility and ultimately perform live testing. Decision making that uses high weights for particular ethical values can be enforced by regulation, as we will discuss in Section \ref{sec:analogous}. 



\subsubsection{Case 3: Facebook News Feed Experiment}
\textbf{Summary}
For one week in January of 2012, Facebook ran a large scale experiment on over 600,000 users, in which it randomized unknowing participants to different News Feed ranking algorithms. The News Feed on Facebook is the primary mechanism through which individuals see their friends' content \cite{kramer2014experimental}, and relied on a machine learning algorithm optimizing on user behavior and incorporating a large number of weights \cite{meyer2015two}. The goal of the News Feed ranking experiment was to alter exposure to positive and negative content in order to study \emph{emotional contagion}, the impact on an individual's emotions based on exposure to friends' emotions \cite{kramer2014experimental}.

\textbf{Ethics and Utility Framing}
We look at the decision to perform A/B testing on Facebook users through the lens of the framework established in Section \ref{sec:framework}, discussing hypothesized information gain and ethical harm composing the utility of the experiments.

Information gain of A/B testing has been established in other literature. It is useful in allowing practitioners to observe model performance in complex interactive systems with A/B testing. By randomly assigning individuals to competing designs, the superiority of one approach over the other can be established with a high degree of statistical certainty. Participants are usually unaware in online A/B testing, in order to ensure their actions are not changed, and represent real-world interactions with the algorithm \cite{jiang2019s, bright2021}. In this case, directly observing outcomes on participants after making changes to the algorithm allowed researchers to study and concretely verify long-standing assumptions about the nature of the product and its psychological impact. This is the information gained, contributing positively to utility of the experiment.

The utility of this experiment was diminished by its ethical harm, which entered through the ethical values defined in Property 4 of social harmfulness and unfairness to participants. Property 5 lends intuition to the introduction of unfairness. It states that ethical harm is averaging by impact of the experiment across groups, and in this case, the harmfulness was greater for vulnerable individuals placed in the treatment intervention yielding less positive emotions.

The ethical harms in this experiment led to significant criticism for this experiment, including calls for federal agency investigations \cite{meyer2015two}. Critics draw parallel to regulations of A/B testing through Internal Review Boards (IRB). We discuss IRBs and other regulations of A/B testing in clinical settings further in Section \ref{sec:analogous}.

% https://www.nytimes.com/2015/06/21/opinion/sunday/please-corporations-experiment-on-us.html
% https://papers.ssrn.com/sol3/papers.cfm?abstract_id=2605132
% https://archive.nytimes.com/bits.blogs.nytimes.com/2014/03/17/searching-for-profits-in-mobile/
% https://www.nytimes.com/2014/06/30/technology/facebook-tinkers-with-users-emotions-in-news-feed-experiment-stirring-outcry.html
% https://techcrunch.com/2014/06/29/ethics-in-a-data-driven-world/
% https://www.theguardian.com/technology/2014/jul/29/okcupid-experiment-human-beings-dating
% https://www.fastcompany.com/90306916/were-all-being-manipulated-by-a-b-testing-all-the-time
% https://qz.com/181582/bad-ab-testing-is-worse-than-none-at-all
% https://www.theguardian.com/technology/2014/jun/29/facebook-users-emotions-news-feeds
% http://laboratorium.net/archive/2014/06/28/as_flies_to_wanton_boys

\subsubsection{Case 4: Watson AI for Cancer Detection}
\textbf{Summary}
In 2017, the IBM Watson supercomputer was trained on small synthetic datasets and models resulted in erroneous treatment recommendations. This was reported in media due to loud complaints from doctors with concerns regarding patient safety. A defense of the tool is that it was intended to supplement, not replace, physician judgement. Additionally, using synthetic cases allows for more diverse treatment options to be included in the set of recommendations the tool provides and does not limit to treatment recommendations from historic training data. 

 The criticisms raised further retroactive concerns, regarding the validity of published studies demonstrating the tools effectiveness. Some critics said these were likely designed to show evidence of the tool's effectiveness \cite{rossibm}.
 
\textbf{Ethics and Utility Framing}
Although we have limited information on the offline testing IBM performed on these models, we discuss testing with synthetic data broadly through the lens of the framework established in Section \ref{sec:framework}.

% Based on knowledge that the training set used synethetic data, it is possible the test set in evaluations also included simulation data. 

In general, simulation testing is often used for evaluation of machine learning systems because of the ease of testing without having to evaluate the system without having to recruit real users for testing, thus avoiding the associated monetary and time costs \cite{jung2009}. On the other hand, in correspondence with the concerns raised in this case, the simulations may not actually reflect real world, thus tending to diminish external validity. So, costs are low, but information gained is low, so the overall utility can be lower than desirable in some instances.

In this case, once physicians interacted with the model, the ethical concern of downstream harmfulness became prevalant as a concern diminishing the utility of the model's evaluation decisions as well. 

% Ultimately watson health was sold but seems unimportant to metnion idk; https://slate.com/technology/2022/01/ibm-watson-health-failure-artificial-intelligence.html, https://qz.com/2129025/where-did-ibm-go-wrong-with-watson-health

%\subsubsection{Benchmarking and/or Simulation Testing}
%\yannis{Simulation testing is often used for evaluation of interactive machine learning systems. These are interactive systems, whose output depends on the actions carried out by the users. While evaluating such systems, user simulation can be used to evaluate the system without having to recruit real users for testing, thus avoiding the associated monetary and time costs. On the other hand, the simulation may not fully reflect the behavior of the actual users, thus trading off external validity for cost. Examples of simulation testing include evaluation of dialogue systems \cite{scheffler2001corpus, jung2009, crook2017sequence, zhang2020usersimulation}, interactive systems for information extraction \cite{hanafi2022}, etc.}

\subsubsection{Case 5: AI Medical Device testing}
\textbf{Summary}
Researchers have raised concerns regarding evaluation practices and FDA approval standards of medical devices. In an analysis of 130 devices, 93 did not have multi-site assessment. This includes 54 high-risk devices, and impacts devices affecting a range of body areas (chest, breast, heart, head, other) \cite{wu2021medical}.

\textbf{Ethics and Utility Framing} We look at the decision to perform medical AI device evaluation on limited samples of the population, using `data splitting', through the lens of the framework in Section \ref{sec:framework}.

In general, when practitioners partition a population and monitor the performance of the model within a slice of data, this can be a more straightforward task, but requires careful decision making on the choice of the slice \cite{chen2019slice}. In this case, researchers criticize single-site assessment of medical AI device testing, because it is unclear that the AI device performance can be generalized to broader populations \cite{wu2021medical}. Thus, the utility to the evaluations are low because of low information gain through lack of external validity, as discussed in Property 4. 

The utility is further diminished through concerns of potential downstream ethical harm arising through the ethical value of unfairness. This is a plausible concern, based on a case study in which results of a single AI model differ by demographic group when evaluated in three different single site evaluations. The implication is that single-site tested models could yield unintended biases in performance of the device on underrepresented groups \cite{wu2021medical}. Thus, the potential future ethical harm arises through the ethical value of fairness or harmfulness.

The FDA has noted these ethical concerns and has called for improved transparency of testing, and monitoring of algorithms for bias \cite{wu2021medical}. We discuss additional options to enforce ethical decision making in Section 5. 

% This phenomenon forces practitioners to negotiate an ethical tradeoff when selecting which model to deploy. If no model maximizes performance over all subgroups, any choice of model will require sacrificing performance on some subgroup. Moreover, there is no clear principle to guide this decision. A utilitarian perspective--which would seek to maximize performance for as many people as possible--would prefer interventions which boost performance for larger subgroups at the cost of smaller subgroups. In contrast, perspectives which favor formal protections for minorities--often reflected in our social and political structures--would accept reductions to majority group performance if accompanied by improvements to minority group performance. Ultimately, this is a value question of internal and external validity, as well as domain based potential additional considerations of harmfulness or fairness.

\subsubsection{Adversarial Testing}

Although we do not highlight a specific case, we wish to also sketch a discussion of how the decision to perform adversarial testing can yield ethical tradeoffs. This is critical to discuss because of the rapid popularity gain of adversarial testing \cite{croak2023}, and executive mandate to establish guidelines and require corporate reporting of performance \cite{whitehouse2023}. 
%Google's Responsible AI team shared in 2023 that adversarial testing is one of three best practices for responsible generative AI \cite{croak2023}. The Biden Administration's executive order on AI mandates that NIST establishes red-teaming guidelines, and that companies developing foundation models are required to provide regular reports of their red-team performance \cite{whitehouse2023}.

\textbf{Summary}
In adversarial testing (also called `red-teaming'), practitioners intentionally seek out cases where models can behave in ways that would be undesirable. This can be done by individually selecting malicious inputs to provide to models, and manually observing the corresponding outputs. This direct intervention approach aims to allow engineers to uncover model failures or vulnerabilities, and identify corrective steps, either prior to release of models, or on released models, if adversarial testing is done as part of an iterated deployment process \cite{googadv, shevlane2023model}. 

\textbf{Utility Framework Analysis}
We broadly discuss sources of potential ethical harm that can diminish utility of adversarial testing, in following with the framework established in Section \ref{sec:framework}, then discuss an alternative evaluation framework that could in some cases have higher utility. 

A potential ethical harm decreasing utility of adversarial testing can enter through the value of harmfulness or cultural insensitivity. This can occur during the model output labelling step adversarial testing is model output labelling, during which, according to the Google documentation, ``necessarily involves looking at troubling and potentially harmful text or images, similar to manual content moderation" \cite{googadv}. 

An alternative to adversarial testing is model-based red-teaming. In model red-teaming, rather than manual testing, test inputs are generated using a language model, and a classifier detects harmful outputs rather than model output labelling. However, the external validity of model-based evaluation could be lower than external validity with adversarial testing \cite{perez2022red}. Therefore, the decision of whether adversarial testing is better than model red-teaming depends on the precise estimates of information gain and ethical harm for an individual setting. 

\yannis{Interesting reference for Ethical Adversarial Testing: \cite{albert2020ethical}. It also explains that adversarial testing  in some cases negatively affects external validity, because it is often conducted in the digital domain, even for use cases that involve the physical domain, thus leading to test cases that can be unrealistic.}


\subsection{Recurring Themes}
\neha{
The cases discussed here vary in ethical values, and also in additional factors, such as the population impacted by the ML system. By delibrating on the additional factors that may influence the magnitude of ethical harm, we use these cases to posit practitioners consider the following questions when selecting evaluation practices:

% additional decompositions of ethical harm, which was decomposed into the specific ethical values in Proposition 6. 

% The questions we propose teams consider when evaluating potential ethical harms include the following:

\textbf{Q1: Questions around who is impacted.}
The magnitude of ethical harm could be more significant if unknowing non-stakeholders are impacted by system failures, as opposed to individuals who choose to participate in engagement with the system. Additionally, if ethical harms exacerbate existing societal inequities based on disparate impact, this could amplify the magnitude of ethical harm. When looking to the cases above, we note a criticism arising of Facebook's experiment is that the users did not choose to participate in the experiment. 

\textbf{Q2: Questions around what could happen.} Some systems have the ability to cause greater ethical harm depending on the time duration of the ethical harm. The probability of harm and quantity of individuals harmed should also be accounted for. 

\textbf{Q3: Questions around how to mitigate}. The ethical harm caused by a model failure could be less significant if teams have mitigation options that allow them to act with speed and communicate with those impacted. The ability to mitigate with speed might depend on the nature of the feedback signals, and whether there is a clear consensus on what a system failure and mitigation requires. When looking at the cases described above, the ability of Microsoft to quickly remove the Tay chatbot from the internet was a successful mitigation strategy in reducing the potential for ethical harm. 

Overall, taking these motivating questions from the case studies into the context of the framework developed in Section \ref{sec:framework}, if a team is able to consider these groups of questions at the time when selecting the ethical evaluation $d$ that yields the highest utility, they are going to be able to better estimate the magnitude of potential ethical harm $EH(d)$. This can improve decision making by motivating teams to consider the properties of the evaluation decisions they are making.

In the next section, we expand our focus from machine learning teams to practices in other industries. This also steps away from internal team making decision processes and focuse on regulatory changes and external factors that can ensure teams are moved to make ethical decisions.}

\begin{comment}
\hari{Ethical Harm Factors from examples}

1. Context of Evaluation: 
\\- Testing Env: Controlled lab-setting vs real-world field tests 
\\- Phase of testing: preliminary testing, pilot study, full deployment for evaluation

2. Stakeholders affected
\\- Direct
\\- Indirect 
3. Type of Impact from Evaluation
\\- Immediate vs. Long-term: short-term direct effects vs. long-term societal consequences
\\ - Visibility: Easily observable vs. less noticeable effect
4. Scale??:
\\- Reach (geographic): 
\\ - Duration and Intensity: length/duration of evaluation and frequency of interaction 
5. Feedback Signals/Mechanisms: stakeholder feedback, expert analysis, performance data, 
6. Responsiveness: Speed of response, adaptability, communication 


People harmed (experiment subjects) vs. people benefited (deployment users)
Evaluation people only harmed 

Evaluation people benefited, 
\end{comment}

\begin{comment}
    In planning an evaluation, plan signals, evaluation. Planning an experiment observes these things. Whats the purpose of evaluation? At what stage does testing happen? These decisions lead to info gain and harms. 
\end{comment}


% The process of creating adversarial tests can raise privacy concerns. First, output analysis could require practitioners to directly examine data points corresponding to individual test cases. Depending on the test and type of data collected, the examining practitioner may be able to infer the identity of or sensitive information about an individual associated with the input data. Many large technology companies have already fired employees for abusing data privileges, and accessing private information about different users, ~\cite{jackson2021, cox2019,cox2021}, so teams need to take careful steps to ensure adversarial testing is done with respect to legal and social norms of protecting individual privacy.

% The guidelines provided by Google's Adversarial Testing for Generative AI documentation asks that developers find and create datasets establishing safe policy, such as definitions of toxic language phrasing, going as far as recommending ``creative" phrasing. This process is likely to be harmful or culturally insensitive for the individual creating these datasets.


%To avoid value sacrifices around harmfulness and cultural sensitivity, some authors suggest using model-based red-teaming. Here, rather than manual testing, test inputs are generated using a language model, and a classifier detects harmful outputs. This is part of the decision making a team undergoes when deciding how to structure their adversarial tests. Potential additional considerations would be cost, interpretability, or external validity \cite{perez2022red}. 


%\textbf{Formulation} Potential privacy concern, cultural sensitivity, and harmfulness concerns are the ethical harms of the evaluation practice. The information gain is how the system behaves in these adversarial settings, especially for behaviors that can't be unit tested in other ways.


\begin{comment}
    To demonstrate the need to consider utility trade-offs between information acquisition and the potential ethical harms stemming from evaluation choices, we apply a case-based analysis approach using real-world examples.  

Interpretive 

In this section, we take a case-based analysis approach, and discuss several applications of real evaluations. 

This section should not be considered a comprehensive analysis of potentially ethical or unethical evaluation practices within machine learning systems. Instead, we highlight these with opportunities to create systems that will help mitigate ethical harms from evaluation practices for the machine learning community to consider, in order to move the industry towards balancing compliance and effective development. 
\end{comment}

==> old/jan_05_evaluation.tex <==
\section{Analogous practices}\label{sec:analogous}

Here, we discuss examples of domains other than machine learning that face ethical challenges in evaluating systems, in order to present key takeaways as mitigation strategies that the ML industry can adopt to ensure ethical evaluation practices. 

These examples have been selected to illustrate tensions between competing values, or values and information gain, with cost restrictions, that exist in decision making in industries other than ML. Studying these practices using  case-based reasoning for teams developing value-driven machine learning evaluations.

%As other fields face decisions broader than a decision of what the best evaluation practice is for a machine learning system, we present a more general version of Equation 1, intended for \emph{any} ethical decision: 

%\begin{equation}
%\text{max}_{d\in \mathcal{D}}\mathbb{E}(\textit{Utility gain}(d))-\sum_jw_j\mathbb{E}(\mathit{EH}_j(d)) \textit{ s.t. resources} \leq \textit{cost}(d)
%\end{equation}
%where $d$ is a potential option between a set of decisions $D$, that, if chosen will yield some expectation of positive utility as well as various potential ethical harms, where ethical values to consider are parameterized by $j$ and weighted by $w_j$. The optimal decision $d*$ will solve this problem.

Other fields have developed ethical, regulatory and administrative frameworks that help them balance the value tradeoffs which arise in different evaluation practices. Or, they have informal best practices that guide ethical evaluation. The frameworks offer principles which are directly relevant to machine learning development. We will introduce these frameworks into the generalized Equation 2 to illustrate utility-framework based strategies to improve ethics of ML evaluations. These are summarized into proposed mitigations in Table 3. 

%Since practitioners in these disciplines have deployed actual systems at scale, they are more battle-tested and can benefit machine learning developers as the field rapidly evolves. 

As an additional note, the situations discussed below are not the only analogous domains in which these value tradeoffs appear, and we do not aim to be comprehensive in this listing. %Additionally, we highlight that there are some tradeoffs that are already particularly notable in ML, such as fairness and privacy, or social impact tradeoffs for downstream fairness ~\todocite{?}.

\subsection{Placebo Clinical Trials and Social Good}
\label{sec:clinical}
\textbf{Summary and mitigations within field}
\neel{When an A/B test is done using a placebo controlled trial, this could be argued to cause harm to some individuals. Given that other known beneficial treatments exist, denying patients access to those treatments for the sake of measuring the efficacy of the novel treatment against a placebo is considered by some to be both clinically and scientifically questionable. However, these concerns are balanced against their potential advantages. Placebo trials are widely considered to be the most rigorous test of treatment efficacy. They generally require fewer participants than active-controlled trials, thereby making them easier and cheaper to conduct ~\cite{miller2002makes}. % Even where existing treatments exist, placebo trials offer new and valuable forms of information 

Medical practitioners have come to identify several guiding principles that guide determinations as to when placebo trials may be appropriate~\cite{millum2013ethics}. First, placebo trials are permissible when no proven treatment exists for the disorder being studied (e.g., for Alzheimer's dementia). This includes the setting where a treatment may exist, but its efficacy cannot be extrapolated to the population of interest. Second, placebo trials are permissible when preventing patients from acessing a known alternative treatment would expose them to at most ``temporary discomfort or delay in relief of symptoms.'' This is common when the medical disorder being studied is ``minor,'' like common headaches or male pattern baldness~\cite{miller2002makes, millum2013ethics}. Third, placebo trials are justified when existing treatments prove to be highly variable. This is commonly the case for conditions like depression, where established drugs can sometimes fail to outperform placebos~\cite{millum2013ethics}. Finally, placebo trials are permitted when there exist compelling methodological reasons for their use, participants are not deprived of treatments they would otherwise have access to, and the benefits of the trial will be borne by the population contributing participants. 
Further protections of clinical research include federal guidelines that explicitly ensure vulnerable populations are excluded from randomization \cite{polonioli2023ethics}. Clinical research also operates under the regulation of an Internal Review Board (IRB) for research to confirm the ethics of a proposed study \cite{polonioli2023ethics, irbfaq}.}

\textbf{Implication for ML}
The medical field has established a set of standards under which selecting the option of placebo treatments is a permissible selection within the set of evaluation options $D$ \cite{millum2013ethics}. 

The role of the IRB is to evaluate the ethics of a proposed evaluation \cite{polonioli2023ethics}. In our utility framework notation, this is analagous to approving that $\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))$ meets their standards prior to the experiment proceeding.

It has been proposed that corporations launch internal IRBs or consider external IRBs \cite{polonioli2023ethics}. There have also been calls to increase transparency of A/B testing in online settings, or for platforms to offer A/B testing to provide ethics trainings to practitioners to assist their evaluation design \cite{jiang2019s}.

\subsection{US ADA Standards and Accessibility} \label{sec:ada}
\neha{Cutting this section...}

\textbf{Summary and Mitigations within field. }
In the United States, under the Americans with Disabilities Act, the Department of Justice and Department of Transportation issue standards that apply to ``places of public accomodation, commercial facilities, and state and local government facilities in new construction, alterations, and additions". These standards aim to provide accessibility for disabled adults and children. The requirements are broad, covering facilities including elevators, drinking fountains, golf facilities, and courtrooms \cite{ada}.

To assist with meeting these goals, the US Access Board - a federal agency - updates ADA standards, and engages with the public ``to inform the development of accessible design'' \cite{accessboard}. 

\textbf{Implications for ML. } The field of accessible construction has established federal guidelines that mandate a particular ethical value be enforced according to code \cite{ada}. We draw an analogy to the decision process of a construction team in selecting the best design. In our utility framework notation from Equation 2, the weight, $w_j$, corresponding to the ethics of accessibility has been established, and teams do not consider violating this when selecting the best design, due to concerns regarding fines or civil suits. 

\subsection{Testing of Childrens Toys} \label{sec:toys}

\textbf{Summary and Mitigations within field.}
Hello.
\textbf{Implications for ML.} Hello. 

\subsection{US government environmental impact standards and Environmental values} \label{sec:epa}

\textbf{Summary and mitigations within field. }The 1970 National Environmental Policy (NEPA), requires environmental effects to be considered by federal agencies about their actions. This requires federal agencies to begin an environmental review process before their final decisions are made, in which they must determine if their proposed actions have causal relations to significant environmental effects. It does not mandate the most environmentally sound alternative be chosen in any decision, but requires knowledge of the impact of decisions. Among other organizations, the Environmental Protection Agency works on overseeing NEPA \cite{citizensnepa}. 

Critics say NEPA is weak due to the lack of accurate ex-ante predictions on environmental impact, and lack of follow-up monitoring  \cite{karkkainen2002toward}. Furthermore, many categorical exclusions exist, initially introduced to acknowledge that not all governmental actions pose environmental risk, but now critics say this is abused as a loophole to bypass review \cite{foxhill}. A final criticism is that environmental reviews have become time and cost consuming, and can delay critical clean energy projects, indicating clear dysfunction \cite{meyersohncnn}. Reform efforts balance the need for action and ethical value evaluations, and recommend fewer exclusions, and adaptive mitigation strategies \cite{meyersohncnn, karkkainen2002toward, foxhill}

\textbf{Implications for ML. }The field of sustainability has established mandates that environmental analysis be considered in a decision making process. In our utility framework notation, this is analogous to mandating that the set of ethical values, $j$, include sustainability. The specific mechanics involved in ensuring that the ethical value is evaluated are critical to the success of accomplishing ethical development, as illustrated by NEPAs critics.

\subsection{Crash Test reconstruction and liability for ethical harm}

\textbf{Summary and Mitigations within field. }
\neel{Regulators and automotive engineers administer tests to evaluate the ``crashworthiness'' of different vehicles. This is motivated by decisions made by American courts in the the late 1960s, when they began to find automotive manufacturers liable for passenger injuries where elements of the car served to exacerbate the harms experienced by passengers~\cite{choi2019crashworthy}. Though these accidents were often caused by human error, courts argued that the statistically inevitable nature of car accidents meant that manufacturers carried a duty to minimize the consequences of such accidents. This caselaw--dubbed the ``crashworthy doctrine''--would by some accounts inspire a wholesale change in the way manufacturers approached safety, be responsible for technical improvements ranging from seatbelts to padded interiors, and spur a tremendous drop in traffic deaths~\cite{choi2019crashworthy}. }

\neel{Crashworthiness is evaluated through crash tests. In a crash test, researchers place a crash dummy (formally called an anthropomorphic testing device, or ``ATD'') in a vehicle, and remotely drive the vehicle into a barrier in order to simulate a crash~\cite{engber2006}. Sensor readings from the vehicle and ATD–along with camera footage of the crash–are then studied to determine the crashworthiness of the vehicle. }

\neel{Assessing the crashworthiness of a vehicle for every possible type of crash is infeasible, due to (1) the wide range of crash-specific factors, including but not limited to weather conditions \cite{saha2016adverse}, road conditions \cite{fitzpatrick2014influence}, or location of impact \cite{fitzpatrick2014influence}. And (2), individual tests can be expensive, as ATDs can cost between \$100,000 and \$1 million USD \cite{automology2021, hall2015,ferris2022, reilly2021}  and (3), Tests are labor intensive, with each taking several days to perform \cite{automology2021}.}\neha{todo: check these citations}


%A challenge in performing evaluations of crashworthiness is that no two crashes are alike. For instance, researchers have shown that the survivability of a crash is dependent on a range of crash-specific factors, including but not limited to: weather conditions~\cite{saha2016adverse}, road conditions~\cite{fitzpatrick2014influence}, the location of the impact on the vehicle (e.g. frontal impact or side impact)~\cite{keall2018relative}, the type of impacting object (e.g. concrete barrier vs deer)~\cite{iihsobjects}, the speed at which the vehicle is travelling~\cite{iihsnewtests}, the relative wear of the vehicle itself~\cite{national2013vehicle}, the individual physiologies of the passengers~\cite{ishii2020factors}, and the actions of first responders~\cite{calland2005extrication}. 

%Moreover, assessing the crashworthiness of a vehicle for every possible type of crash is infeasible. Individual tests can be extremely expensive. ATDs are sophisticated and highly engineered devices, costing between \$100,000 and \$1 million dollars, containing as many as 30,000 distinct parts, and have a limited shelf life~\cite{automology2021, hall2015, ferris2022, reilly2021}. As cars are typically destroyed after a test, each test requires a brand new vehicle. For cars earlier in the manufacturing process–or higher end cars–this can make testing extremely costly~\cite{automology2021}. Tests are also labor intensive. A single test can require several days to perform, as engineers must carefully prepare the car, calibrate sensors, execute the test, and then analyze data~\cite{automology2021}. Finally, certain types of crashes are impossible to perform in simulated environments, due to the complexity of factors (e.g. multiple cars) or difficulty in simulating conditions (e.g. extreme weather events).   

Thus, evaluating crashworthiness for vehicles requires engineers to navigate a tradeoff space between the cost of a crash test, and the information it provides. Automotive companies are motivated to invest in crash testing based on established standards. %The ways that crash responsibility is on auto companies and successfully motivates thorough testing standards, motivate the need for regulatory practices that ensure responsible, safe AI, to ensure that corporations invest in testing. 


%Today, the precise regulations governing crashworthiness are laid out in the Federal Motor Vehicle Safety Standards~\cite{fmvss}, which establish minimum safety and performance criteria for motor vehicles. These regulations are maintained by NHTSA pursuant to its authority under the National Traffic and Motor Vehicle Safety Act of 1966.  
% https://www.bloomberg.com/news/features/2018-10-25/even-the-crash-test-dummies-are-putting-on-weight
% https://jalopnik.com/how-your-car-gets-crash-tested-1829793856
% https://www.consumerreports.org/car-safety/some-cars-will-never-be-crash-tested-crash-test-ratings/

\textbf{Implications for ML. }
Automotive standards have been established that teams invest high costs into evaluating the crashworthiness of vehicles. This has been established by high penalties for failure to do so, as well as consumer preferences for safe vehicles. 
In our utility framework notation, we can denote this as teams allocating high $resources$ to their optimization problem about testing, so that the overall crashworthiness tests that can be selected from all available tests $D$, is high in cost. 

\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.45\linewidth}|p{0.35\linewidth}|p{0.2\linewidth}|}
        \hline
        \textbf{Ethical Intervention in Utility Framework Notation} & \textbf{Domain} & \textbf{Ethical Values} \\
        \hline
         Centralized agency overseeing approval of $\sum_jw_j\mathbb{E}(\mathit{EH}_j(d))$ & Placebo clinical trials require IRB approval required prior to study & Overall ethics\\
        \hline
        Federal enforcement that vulnerable populations excluded from $D$, as well as other standards established for $D$ & Clinical Trials regulated by federal mandate & Fairness, social good \\
        \hline
%%        Federal enforcement that $w_j$ enforced for some $j$ & ADA standards for construction & Accessibility \\
%        \hline
        Regulatory enforcement that $j$ required to include some values & US NEPA mandates environmental analysis for federal agencies & Sustainability \\
        \hline
         Legal and consumer motivation to ilncrease budget towards evaluation, so increase $\textit{resources}$, widening range of possible $D$ & Automotive crash testing & Cost restrictions in evaluation \\
        \hline

    \end{tabular}
    \caption{A summary of potential ways to ensure ethical values are prioritized in decision making, inspired by strategies implemented in domains other than ML. We draw an analogy between the ethical intervention and our utility framework, introducing this sketch of notation. This allows us to concisely summarize and motivate actions the ML industry can introduce in order to mitigate for ethical harm in evaluation practices. Note also, the ethical intervention suggested by the domain need not be restricted to the particular ethical value it corresponds with (ie enforcing $j$ required to include some values could apply for other values than sustainability).}
    \label{tab:tab2}
\end{table}



\hari{Analogous domains strategies trying to limit harms from evaluation, RCT.... harms are caused by evaluation, is anything being done.... content moderation.... automated harms from humans, automated technique is not as good as a human}. 

\hari{Social Policy Experiments, Psychological Research, consumer product testing: testing children's toys}

==> old/jan_06_discussion.tex <==
\section{Discussion}

\subsection{Implications for ML Teams}

\noindent
\textbf{Ethical Guidelines and Review Boards:} Similar to how the medical field uses Internal Review Boards (IRB) to evaluate the ethics of clinical research, ML evaluation can benefit from internal or external IRBs. These boards would assess the ethical aspects of evaluation designs, ensuring that they meet certain ethical standards, particularly when making trade-offs.


\noindent
\textbf{Legal and Regulatory Compliance}



\noindent
\textbf{Environmental Considerations}


\noindent
\textbf{Risk Assessment and Mitigation}


\noindent
\textbf{Balancing Benefits and Harms}


\noindent
\textbf{Public Engagement}



Strategies: 




\subsection{Broader Utility}

\textbf{Evaluating the Ethical Values of ML Systems}. More disparate than the other two relevant bodies of literature is a broad set of work that focuses on the ethicality of machine learning systems. \jessica{is it that easy to separate ethics? like isn't a choice to prioritize accuracy ethical in some sense, because you're minimizing bad outcomes as population level?} Existing work characterizes principles and values that machine learning systems should adhere to, and questions goals of deployed systems. Evaluation processes and metrics assess the performance of a model across specific \textit{values}, as values are aspects of a system which practitioners are interested in measuring. For instance, engineers may use metrics to measure achievement of values, such as fairness, robustness, or accuracy. \jessica{again im not sure there's a clear distinction between the values you mean here and the values that lead us to use more conventional metrics}

As an example to illustrate the differences between these three types of research areas, the ethics literature would ask: `Why would we use facial recognition technology in surveillance?'. In contrast, the metrics literature would ask about the best metric for evaluating the bias vs the effectiveness of the model. Meanwhile, evaluation questions would ask what an effective test of the facial recognition technology would be.\jessica{aren't these all evaluation questions?} We proceed by discussing the importance of bridging these disparate fields, and prompt teams to think about ethics in their evaluation methods, rather than exclusively considering the ethical values of their end products.

\jessica{How we chose the categories in this section is hard for me to understand. Worth considering how exactly they set up the rest of the paper. It also feels like we're talking very broadly here, and the ML evaluations subsection is particularly generic/hard to separate from ethical values.}


\subsection{Software Lifecycle}

\cite{ashmore2021assuring} surveys ways in which machine learning models are determined to be safe, referring to these as assurance methods, at various stages of the machine learning lifecycle. When they define the machine learning lifecycle, they discuss 3 initial stages: data management, model learning, and model verification, in which models are produced. The final stage they define is model deployment. Every model is spiraling through these stages over its lifecycle, as models can be updated after deployment or with new data samples gathered. The authors further describe key disederata for each of these stages of the lifecycle. For the data management stage, they are relvance, completeness, balance, and accuracy. For the model learning stage, desiderata include whether the assurance method is performant, robust, resuable, and interpretable. 

When \cite{zhang2020machine} discuss the role of testing in ML systems, they describe a circular model in which both online and offline testing happen, and the user cycles through: historical data, prototyping, offline testing, deployment, user interaction, predictions, online testing, adapted model, online data. The authors describe the testing properties as happening only in the online and offline testing phases of the cycle, and discuss questions such as \emph{why} we test models. The ethical \emph{why} question should go beyond what properties a model can be tested for, and should be posed at stages of the lifecycle beyond testing, such as the security and privacy of data management systems. 

In \cite{ashurst2022disentangling}, the authors discuss ethics in ML research. Research precedes deployment of live systems, and considerations they discuss, such as treatment of workers contributing to research that influences a deployed model, should be considered part of a deployed systems' lifecycle.




\subsection{Limitations and Future Work}




==> old/jan_07_conclusion.tex <==
\section{Conclusion}
The cases of existing machine learning evaluations described in Section \ref{sec:mlcases} has some parallels to the ethical interventions illustrated in non-machine learning domains in Section \ref{sec:analogous}, such as discussions around whether there should be centralized agencies overseeing approval of ethical considerations in live machine learning experiments, in following the precedent set by clinical trials.

Our utility framework for decision making illustrates the importance of selecting a decision that weighs gains against potential harms in both machine learning evaluations, and domains that have navigated prioritizing of ethical considerations. These mitigations offer suggestions for future research, as we do not have sufficient information to guarantee that the ethical mitigations used in other domains would be \emph{causal} of improving ethics of evaluation practices in machine learning. We hope this framework will motivate future research and suggest discussions for machine learning community as it aims to move towards ethical evaluation frameworks through regulatory means or best practices. 

%Fields other than machine learning, notably medical fields and automotive safety fields, have developed regulatory standards, and best practices for evaluation procedures over time. This was necessary in order to protect consumers, of drugs and automotives, respectively. In offering human protection in testing, these fields are better able to execute values of their fields. We discuss the necessity for values in evaluation of machine learning models, by exploring six common evaluation practices used to test machine learning systems, and discussing how values of machine learning models (such as fairness or robustness) are integral parts of the process of using these evaluation as well. 

%Thus, we have motivated the necessity of considering values in evaluation, during the model development lifecyle, whereas previous research discusses values of deployed models. We motivate further research and suggest that future works which could develop frameworks or regulatory guidelines for ethical evaluations of machine learning models.

==> old/jan_07_relatedwork.tex <==
\section{Related Work}

==> old/neha_02_relatedwork.tex <==
\neha{

\begin{itemize}
    \item In \cite{zhang2020machine}, the authors define testing `properties', as the motivation illustrating \emph{why} we test ML systems. They list properties that the ML community is most concerned about, selecting the following: correctness, overfitting, robsutness, security, privacy, efficiency, fairness, and interpretability. Based on my read, we can relabel their overfit to external validity, but their correctness seems to cover both internal and internal validity. Their definition of robustness is basically adversarially tested to not fail on wacky input. 
    \item Also in \cite{zhang2020machine}, they categorize online vs offline testing, calling A/B testing and live testing both `online'. They have a testing `workflow' defined, which is the \emph{how} of how the testing will be done. See figure 5 of the process. It includes 6 major topics: test input generation (adversarial and natural), test oracle (does a bug exist or not basically), teset adequacy (do the tests reveal bugs), test prioritization and reduction (how much testing are we doing), and debug and repair, general testing framework and tools (ehhhh -- ok at the end this paper got kinda hard to read I'm not sure these are actual decisions or parts of the workflow but just things they wanted to talk about). 
    \item In \cite{nahar2022collaboration}, the authors motivate ML challenges with several interview. Some of the ones they mention include: ``establishing model adequacy" (when a model is good enough), which often leads to another issue of lack of transparency about test resultsand test process, a third is responsibility for model quality (as individual components are tested as well as the integration), and lastly, online testing is rare and things are often not monitored online.
    \item Some literature focuses on developing types of tests for example Ribeiero et al offer three different test types for NLP models, including MFTs minimimum functionality tests (inspired by unit tests in software engineering), inv invariance tests which  perturb input expecting same output, and directional expectation which expects a certain style of change. Offers templates for test generation
    \item \cite{davis} uses 165 NLG papers using human evaluations in natural language generation to say that there needs to be a standardization in methods and terminology due to a breadth of approaches and ``lack of clairty in reports" How to define quality criterion? How to collect responses? What are participants responding to?

    \item Coverage criteria needs to be reevaluated because traditional code coverage metric from software engineering might not be helpful in ML \cite{giray}.
    \item \cite{braiek} separate white box and black box testing of models -- both of which test conceptual mistakes when writing code. black box doesnt require implementation details of the models and whie box does. I'm not sure how this generalizes to our discussion - I guess live testing and generative testing are black box. 
    \item \cite{weyuker} The definition of an oracle -- some person or mechanism which establishes correct program output, and nontestbale programs are where oracle doesn't exist.  Weyuker identified three categories of “non-testable”programs: (1) programs that produce so many outputs that it is practically impossible to verify them all; (2) program for which developers and testers have different specifications and thus a tester miscon- ception exists; (3) programs that were written to determine an an- swer (such as ML programs where developers aim to learn the ap- plication logic from data without any prior knowledge on it).
    \item \cite{felderer} follows \cite{zhang2020machine} and expands to say that there are these  challenges in developing appraoches for testing of AI: (direct quote)  Understandability and interpretability of AI models, Lack of specications and defined requirements, Need for validation data and test input generation, Dening expected outcomes as test oracles, Accuracy and correctness measures, Non-functional properties of AI-based systems, Self-adaptive and self-learning characteristics, Dynamic and frequently changing environments. They discuss each with a few citations. 
    \item \cite{kaushik2022human} (I think that citation is right) discuss issues wit croudsourcers in ML and whether and how ethics comes in there. This is a good point. If you put it in context of \cite{zhang2020machine}, they're calling out key testing properties, but realistically those apply elsewhere in ML system development too including in historical data generation/online data generation. 
    \item \cite{marijan} says bascially what other authors say too...code coverage is misleading...there's no test oracle....quality of test datasets is questionable...cost effectiveness of adversarial examples....research area of how to verify ethics is largely unaddressed because frameworks assume that system is separated from ... vague and kinda poorly written tbh....
    \item \cite{foidl} discuss the data validation process before ML systems are developed (part of ML lifecycle). Could bring this back to \cite{zhang2020machine}. They have figure 1, which illustrates the ML software system (data, cleaning, ml model) and we can argue that our novel contribution extends to the entire lifecylce because of this. 
    \item \cite{ashmore} establishes the ML lifecylce as a 4 part spiral. We can connect one of our frameworks to each of these parts I think. 
    \item \cite{martinez-fernandez} does a metastudy of 248 other studies and highlight what properties most AI-based systems study. They do find that most people tend to study a number of properties....(safety, functional correctness, robustness, reliability, security, accuracy, testability, explainability, maintainability, performance...). This paper is really long but it probably has some pretty good stuff - maybe see google docs with main highlights. 
    \item \cite{ashurst} Really good. Table 3 discusses research ethics at various parts of the process. This includes non-participants (A/B testing), ethical treatment of workers (labelling harmful data), management of assets (data privacy). Connect this to the other pieces.  
    \item \cite{jakesch2022values} lists out values that different groups prioritize (crowdsource workers vs public vs etc etc) and so we can use their list and also briefly mention differing ideals. 
    \item \cite{jobin2019global} this is highly highly cited and has a listing of key ethics. 
\end{itemize}
}

==> old/old_01_intro.tex <==
\st{Traditionally, evaluating machine learning models has been standardized across model type, domain, and application.}

\st{However, a number of real-world deployment failures have highlighted the limitations of the conventional evaluation approach. In these instances, the evaluation process failed to surface critical error modes, and model failures were only noticed \textit{after} deployment. (Take examples from Deb's paper on why machine learning doesn't work)}

\st{These failures have generated calls for a new approach to evaluation, in which practitioners take an active role in designing evaluation protocols specific to the domain and application. For instance, models should be evaluated with regards to data subgroups, and tested for reliance on spurious correlations.}

\neha{It has been established that the suitability of a machine learning model is governed by more than just it's accuracy, necessitating evaluation of models with regards to additional characteristics, such as robustness, privacy, fairness, and interpretability. Traditionally, evaluation methods for machine learning models that rely on quantified metrics have been established for a singular one of these characteristics. In measuring accuracy of a machine learning model, we may look to predictive capabilities on independent test datasets using a loss function such as squared error or absolute error. In evaluating the fairness of a model, we may look to counterfactual fairness of individual outcomes, or dataset biases mirrored in a model. In measuring the privacy of the model, we may look to differential privacy mechanisms. Some research has gone further, and have suggested quantified metrics that allow accounting for multiple of these characteristics (If citations needed, skim quickly/cite \cite{pujol2021equity} and \cite{fish2016confidence}, Elements of Statistical learning, counterfactual fairness paper?)}

Others have highlighted that evaluation requires non-technical lines of inquiry, \neha{via nonquantifiable metrics}, and that practitioners should consider the downstream harms of models, and whether performance disparities align with historic or engrained power imbalances. In assessing how and whether to deploy a model, practitioners should identify and engage with different stakeholders, and understand the extent to which they are impacted by the deployment \neha{Do we have/need citations for this?}. 

\neha{Regardless of whether an evaluation practice is via a quantified metric or using a non-quantifiable argument,} the higher level goal of both of these efforts is to make evaluation more effective by enabling practitioners to better identify model \st{failure modes}\neha{shortcomings} before deployment. 

 
\st{
However, some of these proposed practices also present a dilemma. While a particular practice may provide engineers with greater information on a model’s potential failure modes, the  process itself may create the opportunity for an ethical harm. Already, researchers have identified instances where effective and ethical evaluation are at odds
}  

\neha{However, some of the proposed practices of evaluating models, whether through quantifiable metrics or nonquantifiable evaluation practices, present additional dilemmas. While a particular evaluation procedure may provide engineers with greater information on a model's potential shortcoming, the evaluation process itself may create ethical harms. Already, researchers have identified instances where an evaluation practice may be effective at preventing downstream harm, but is unethical in itself:}
 

\begin{enumerate}
    \item \neel{Live testing with Tesla}
    \item \neel{Collecting data from vulnerable populations}
    \item \neel{Privacy fairness tradeoffs in collecting demographic data}
\end{enumerate}

\st{Unfortunately, the literature offers little guidance on how practitioners should navigate ethical dilemmas in evaluation. The machine learning evaluation literature primarily focuses on methods and toolkits for performing evaluation, and thus ignores the ethical challenges that emerge. For instance: despite the the abundance of literature describing different definitions of fairness, there is little work describing when evaluating fairness necessitates the privacy incursion of collecting sensitive demographic data. In contrast, the AI ethics literature primarily focuses on the ethical impacts of a deployed model on a population of users. There is comparatively little work documenting or discussing the ethical challenges that can arise in developing models}

\neha{Unfortunately, the literature offers little guidance on how practitioners should navigate ethical dilemmas while evaluating a model. Machine learning literature which focuses on quantifiable metrics for performing evaluation ignores ethical challenges that emerge in the evaluation process. In contrast, reporting toolkits that have become available aim to increase transparency of AI ethics by acknowledging model shortcomings across various ethical characteristics, and are often provided by teams that have built models as documentation with a deployed model. These allow teams considering using a model to accurately evaluate its ethical impacts and tradeoffs of deploying a provided model on a population of users (cite modelcards etc).}

\st{Our work seeks to bridge this gap, by developing a framework to assist practitioners in navigating the tradeoffs between ethical and effective evaluation. Our framework has two focal points. First, we identify that any evaluation practice can be assessed with regards to different \textit{dimensions}, which indicate the practice's compliance with different values (e.g. harm-avoidance, interpretability, cost, etc.). These dimensions allow us to identify and explain why certain evaluation practices create ethical tradeoffs. Second, we observe that similar tradeoffs arise in the evaluation practices of analagous domains (e.g. automotive safety). Using our dimensions, we can study these analagous domains to identify (1) how comparable practitioners balance tradeoffs, and (2) the mitigating procedures they have developed. Thus, our framework provides value as a tool for detection (i.e. identifying ethical tradeoffs), deliberation (i.e. balancing competing values), and mediation (i.e. applying mitigating protocols).}

\neha{
Our work seeks to fill the gap in documenting and discussing tradeoffs in creating ethical and effective evaluation processes for machine learning models. We identify that any evaluation practice can be assessed with regards to different \textit{goals}, which indicate the practice's compliance with different values (e.g. harm-avoidance, interpretability, cost, etc.). These values allow us to identify and explain why certain evaluation practices create ethical tradeoffs. We frame these questions as noteworthy throughout the entire model development lifecylce. In addition to the typical post-deployment documentation, these questions and values are relevant during model training, testing and pre-release.}
% Notes from hari:  1st. ID nature of tradeoffs in modeling/eval practices, what kind of tradeoffs occur in common ml practices (section 4). What values we should be caring about? One contribution could be identifying ethical values for ML modeling processes. ID tradeoffs across methods or within a method. 3rd can be recommendations based on analogous domains. How do we balance values w viabilities?

% quantitative vs qualitative not so important. 
% values of creators are different than values for users. 
% is the nd result model a good fit for what its being used for?
% in disaggregated evaluation when a model is deployed in the wild and methods we have for that -- while we care about values of deployed models -- we haven't talked about how were building/testing in ethical ways. 

%In building fair/useful/ethical ML we care about evaluation across various criteria but based on prior work/literature, when carrying these evalus out, we make tradeoffs. have methods that assess viability of xx...but in operationalizing we sacrifice....In this work we define ethical criteria for evaluation practices, and asess how certain methods force us to prioritize certain values over others. WE describe how each method leads to tradeoffs along value dimensions...This is not a new problem in ML, people make similar tradeoffs and how can we do things better? 

% Given that I'm using these evals, what are the mapping from evals to values. Not reverse. Highlight value tradeoffs in methods that exist. 

Specifically, we make the following novel contributions.\neha{
% These are repetitive.
\begin{enumerate}
    % first two are good but 3rd needs work. what are takeaways for people? Providing values based on social science and responsible AI research. How would each of these practices force us to consider/prioritize different values. Given that these tradeoffs are unavoidable what can we learn from other domains that can be applied? Be clear about values we hold as ethical practitioners and what we care about post deployment. A lot of current research is on post deployment. Examples are around meeting the distilled goal -- not doing harmful practices. 5 point intro framing the paper and then list contributions. 
    \item We define three distinct questions that teams need to answer: (1) What is the set of high level values I am building my model around? (2) How will I ensure my model meets these values -- what quantitative metrics or qualitative goals do I have? %tradeoffs
    (3) What will my model design, development, and testing lifecycle look like in order to meet these goals? 
    % guidelines
    \item While discussing these three key questions, we frame each in terms of core values or principals, which operate as both the primary aim, and constraints.
    \item This is novel in that this evaluation protocol aims primarily to be considered during the model development lifecycle and pre-deployment, although can also be discussed post-deployment, post-incident, or during regulatory compliance changes.
    % This is the methods. 

\end{enumerate}

We close by observing where similar tradeoffs arise in the evaluation practices of analagous domains. For example, A/B testing done in clinical trials requires IRB approval. We study these analagous domains such as drug development to identify (1) how comparable practitioners balance acheiving their goals subject to various constraints when building models, and (2) the mitigating procedures and institutions that have been developed in order to support their values.
}

\begin{comment}
    Intro:
(stuff from your current background)
•	Traditionally ML evaluation is standardized.
•	Flaws in the real world due to evaluation blindspots
•	Shifting/ need for ML practices to be more comprehensive (values, stakeholders, downstream harms..) 
•	Ethical vs. effective evaluation decisions and tradeoffs, real-world examples <--- our motivation to understand how to make better evaluation decisions based on understanding from analogous domains
Related Work:
•	What to evaluate in ML?
•	How to evaluate?
•	Ethical Evaluation Needs and Challenges (less focus on AI ethics but on ethical evaluation practices, longer comment in the google doc)
 
Formalizing Ethical Dimensions for ML Evaluation 
•	Seven Dimensions
 
An Analysis of ML Evaluation Decisions and Ethical Trade-Offs in Practice
•	Eight Practices
•	decisions, trade-offs, ethical dilemmas, harms?
 
A *Decision-Making* Framework for Ethical Evaluation (I am not sure we want to call it a framework but we can discuss)
Option A:
•	Lessons from Analogous Domains
•	Domain, Decision, Trade-Off
•	Implications from ML evaluation decisions
•	Not by evaluation practice but based on evaluation decision
•	Survey with practitioners
•	(current practice, feasibility of implications/ decision-making framework)
Option B (I prefer this option if one analogous domain highlights one decision trade-off ):
•	Trade-off 
•	Lesson from an analogous domain (from your outline, I am assuming each of the analogous domains highlights a specific trade-off between values)
•	Decisions and Trade-offs
•	Implications from ML evaluation decisions
•	Not by evaluation practice but based on evaluation decision
•	Survey with practitioners
•	(current practice, feasibility of implications/ decision-making framework)
 
Discussion and Conclusion

\end{comment}

==> old/old_02_background.tex <==
\textbf{Machine learning evaluation goals.} A related body of work focuses on the goals of evaluation– the different aspects of a model’s performance that practitioners may seek to quantify. For instance, beyond simply accuracy, developer's may seek to measure a model's fairness, robustness, interpretability, or capacity for misuse. In service of these goals, related work has developed and studied the tradeoffs of different metrics. Research has additionally highlighted how emerging machine learning paradigms necessitate new evaluation goals. For instance, the rapid growth in generative models has given rise to a need to quantify these models in terms of their toxicity, bias, and factual correctness. 

\textbf{Machine learning evaluation tools.} To support the pursuit of these evaluation goals, prior work has studied how to perform accurate and effective evaluation under different types of resource constraints. Researchers have focused on methodological and dataset flaws that can confound evaluations, and recommended strategies for avoiding these errors. Prior work has also developed tools and infrastructure for practitioner use. A number of toolkits focus on certain concrete goals (e.g. robustness or privacy), and enable practitioners to effectively evaluate different models with respect to these goals. Other toolkits take a more holistic view, seeking to provide practitioners with a means of balancing multiple forms of evaluation.  Practitioners have also developed institutional mechanisms to aid in evaluation, including bug bounty challenges, infrastructure to support stakeholder feedback, and documentation practices.

\textbf{Evaluating the ethicality of machine learning systems.} Finally, we draw a connection to the broader constellation of work focusing on the ethicality of machine learning systems. Prior work  has characterized the principles that ethical machine learning should adhere to, including values like privacy, fairness, misuse deterrence, transparency, and contestability. Independent auditing efforts have in turn highlighted instances where deployed systems have failed to adhere to such values [Cite to audits]. Thus, machine learning practitioners and stakeholders have begun to experiment with approaches for directly evaluating the ethicality of a machine learning system. Prominent among these include efforts to incorporate ethics feedback into grant funding processes, deployments in governmental settings, and industry ethics review processes. In addition, a range of actors–spanning research groups, governmental entities, and industry–have released frameworks for guiding such ethical deliberations [CITE to AIA work]. 



==> old/old_03_nehas_time_varying_model.tex <==
Old. Removing. 
\subsection{Model}

This is not the first body of work framing ML models as providing utility to society, and emphasizing ethical considerations, but other works restrict to discussing a single model's output and social impact. For example, in \cite{corbett2017algorithmic}, the authors provide a definition of immediate utility, which reflects the costs and benefits of a fair decision by a policymaker, notably in the setting of pre-trail bail release decisions. Similarly, in \cite{corbett2018measure}, the utility function reflects a single decision made by a model, such as whether or not to screen an individual for diabetes. In \cite{chohlas2021learning}, a utility function determines the optimal decision making, such as in the decision of providing funded transportation for court appearances. Our framework deviates from these in that we are not focused on the fair output and decisions made by an ML model. Rather, we are focused on the decisions made by a team when developing and deploying a large-scale ML system.

This is also not the first body of work to discuss ML models and utility while emphasizing evaluations. \cite{hutchinson2022evaluation} use a utility function to simplify and discuss framing of an evaluation of a single model's appropriateness for a given application. The motivating philosophy of consequentalism - that actions are good or bad depending on its consequences - also applies here. However, our framing centers on an overall system rather than one model. In broadening the discussion to a teams' model development lifecycle, we are able to incorporate teams' value decisions at all stages of a development lifecycle - including creating, testing, and deploying - rather than just consequences of a single model's use for a particular application. 

We define the model below, and then discuss six properties and four implications. Taken together, the composition of these properties illustrate the way a software teams decisions regarding values, accuracy, and costs can be made over the entire model lifecycle. The accompanying implications and mitigating strategies motivate potential options for the machine learning industry to overcome existing challenges in building ethical AI. 


Suppose a machine learning development team is rational and utility maximizing, and building a product that will exist for infinite time periods. They have some utility function, which is increasing in their consumption, $c$. Consumption can be thought of as factors such as team wages.

Each time period, the team has the ability to choose how much they will consume, or how much they will invest into either their values, $v$, or model accuracy, $a$. An investment in values can be thought of as something like green energy consumption. An investment in accuracy can be thought of as improved model performance measured by AUC. There are no other options for spending. Both accuracy and values influence the income a team is able to receive, and this income is determined by some non-deterministic function $f(v,a)$. The team is given some initial income at the start of time period 0. There are no additional income sources.

The team is thus selecting a resource allocation, in the form of the following three sequences $\{v_{t+1}\}_{t=0}^\infty$, $\{a_{t+1}\}_{t=0}^\infty$, $\{c_{t}\}_{t=0}^\infty$ which solve the following optimization problem:

$$\text{max}_{\{v_{t+1}, c_t, a_{t+1}\}}\mathbb{E}(\sum_{t=0}^\infty\beta^tU(c_t))$$
subject to the budget constraint:
$$\mathbb{E}(f(v_t,a_t))\geq c_t + v_{t+1} + a_{t+1}$$
$\beta_t$ is a constant parameter that can be considered a time discounting rate.
(Note to self; do I want a zt stochastic parameter in f? Do I want to remove the beta? Do I want to make this one period ahead security trading instead of time zero?)

\subsection{Model Properties}
Here, we discuss various features of this framework, evidence that suggests assumptions surrounding the feature are defensible, and potential issues with each feature. 

\textbf{Property 1: Agents are rational, utility maximizing decision makers}
This is a necessary typical property in the standard macroeconomic model. 

The decision to allocate resources towards consumption, investment in products, or investment in values seems accurate anecdotally. In case studies and interviews of AI ethics  workers within organizations, results showed that ``workers were incentivized by metrics associated with financial gain" \cite{ali2023walking}. It seems true anecdotally that less investment is made towards values, compared to investment accurate modelling that yields financial gain, and efforts to improve firm consumption -- rational individual firm workers would invest towards their individual consumption.   

\textbf{Property 3: Multiple time periods}
Just as an economic agent would aim to optimize utility across the lifetime of an economic model, software teams look towards the lifecylce of a machine learning model. 

\cite{ashmore2021assuring} breaks the machine learning lifecylce into four stages (data management, model learning model verification, and model deployment).  Every model is spiraling through these stages over its lifecycle, as models can be updated after deployment or with new data samples gathered. The authors further describe key disederata for each of these stages of the lifecycle. For the data management stage, they are relvance, completeness, balance, and accuracy. For the model learning stage, desiderata include whether the assurance method is performant, robust, resuable, and interpretable. Decisions are made by teams regarding monitoring and updating of systems after deployment as well. Overall, the decision of what optimal allocation of resources towards consumption, investment in values, or investment towards model accuracy, look different in each time period.

When a team makes its resource allocation decision, there are going to be \emph{time-variant} and \emph{time-invariant} tradeoffs. As an example of a time-variant tradeoff, we look to autonomous vehicle developments.Through specialized testing programs, California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}. The program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles “test drove” at least four million miles on public roads in California~\cite{bellan2022}. In the Tesla Autopilot systems, teams choose to forego ethical value investments in time period when conducting evaluations with live testing, as the systems was trained and tested on public roads with other drivers and involved in several fatal crashes, but this may prove to be effective at preventing downstream harm once development is completed.

As an example of a time invariant tradeoff, there is a well established link between loss of privacy when fairness acheives gains, and this value tradeoff does not depend on future and past tradeoffs. ~\todocite{cite} 

\textbf{Property 4: Stochastic nature of model and expectations}

This model allows the function for firm income, $f$, to be non-deterministic, and also requires that we maximize for the expected value of utility. 

The income function is deterministic because of the difficulty in quantifying values, accuracy, and their impact on firm income, as well as firm income independent of fluctuations in values and accuracy. When teams make decisions regarding their products, no choice guarantees any income. 

The expected value of utility is necessary for two reasons. First, the fact that values and consumption can be quantified is an oversimplification necessary for the sake of creating a modeling framework here. In several instances, ethical values are difficult to prove or quantify \cite{ali2023walking}. Even if they were quantified, they couldn't guarantee utility directly and there would be some uncertainty. This is due to the second arguemnt, which is that positive utility, in the consequentialism argument, would require positive value impact. There are several instances of models that differ in social impact across groups, notably underrepresented groups, and instances of accuracy failures in underrepresented groups \cite{hutchinson2022evaluation}. Thus our model taking the expectation of utility does reduce some benefit of the model, but this is something teams would be aware of when choosing resource allocation and estimating utility. 

\subsection{Model Implications to improve ethical ML}
Continuing the framing described, we now discuss implications this analogy has for ways to improve the ethicality of machine learning systems. 

\textbf{Mitigation 1: Better tests eliminate uncertainty}
If teams are able to better estimate the social impact of a model, or better able to estimate the accuracy of a model, through better testing, they have a better estimate of the expectation on $f$ and the utility function, and are thus more precisely able to choose their resource allocation.

\textbf{Mitigation 2: Add constraints}

If an additional constraint were added to the optimization function -- for example, in the form of a policy made to mandate a particular value meet some threshold -- this would require firms to adjust all aspects of their development lifecylce accordingly and would ensure the value meets the threshold.

\textbf{Mitigation 3: Create incentives for earnings to vary with values}

The $f$ function was largely undefined here, but if incentives are made with policies where firms receive benefits or penalities for social impact or harm, this would shape $f$ in a way that ensures the choices made in the development lifecylce respond accordingly. 


==> old/old_04_Jan24.tex <==
\subsection{Case 3: A/B testing with political ads}
\textbf{Summary}
Researchers have found, via mined data from the Optimizely service used to run and analyze A/B tests on websites, that several websites that are rated as having a political leaning, ran A/B tests. This includes CNN, the New York Times, and ESPN. The authors do not note any unethical experiments (ie using unethical click-bait headlines could cause political consequences, such as changes in voting behavior). However, due to the established link between internet behavior via search results and changes to voting preferences, malicious actors could use A/B testing with news outlets to cause ethical consequences 

In A/B testing, practitioners evaluate two competing designs–approach ``A'' and approach ``B''–by evaluating the impact of both approaches on two completely separate populations of users, where individuals are randomly assigned to one approach and not the other. The differing outcomes of individuals in each group are compared, with the purpose being to establish the superiority of one approach over the other with a high degree of statistical certainty. Most internet users browsing on sites using Optimizely are unaware of their membership in these A/B tests.

\cite{jiang2019s}.

\textbf{Utility Framework Analysis}
A/B testing aims to yield information gain by optimizing product design. They may aim to analyze behavior by seeing which treatment group yields more clicks. 
The potential for ethical harm is in fairness and social impact. Furthermore, when experimenting with social leaning, the collection of data on a persons political identity is a protected status by some measures, opening a further potential ethical concern. 

\subsection{Case 4: A/B testing with price discrimination}
\textbf{Summary}
\textbf{Utility Framework Analysis}
Privacy


\subsection{A/B testing}
% https://www.nytimes.com/2015/06/21/opinion/sunday/please-corporations-experiment-on-us.html
% https://papers.ssrn.com/sol3/papers.cfm?abstract_id=2605132
% https://archive.nytimes.com/bits.blogs.nytimes.com/2014/03/17/searching-for-profits-in-mobile/
% https://www.nytimes.com/2014/06/30/technology/facebook-tinkers-with-users-emotions-in-news-feed-experiment-stirring-outcry.html
% https://techcrunch.com/2014/06/29/ethics-in-a-data-driven-world/
% https://www.theguardian.com/technology/2014/jul/29/okcupid-experiment-human-beings-dating
% https://www.fastcompany.com/90306916/were-all-being-manipulated-by-a-b-testing-all-the-time
% https://qz.com/181582/bad-ab-testing-is-worse-than-none-at-all
% https://www.theguardian.com/technology/2014/jun/29/facebook-users-emotions-news-feeds
% http://laboratorium.net/archive/2014/06/28/as_flies_to_wanton_boys


\textbf{Definition} In A/B testing, practitioners evaluate two competing designs–approach ``A'' and approach ``B''–by evaluating the impact of both approaches on two completely separate populations of users, where individuals are randomly assigned to one approach and not the other. These are utilitized in a wide range of industries and research disciplines. The differing outcomes of individuals in each group are compared, with the purpose being to establish the superiority of one approach over the other with a high degree of statistical certainty. Participants in A/B tests may be oblivious to their membership in the test, to ensure minimal altering of their behavior and results. A/B tests can help practitioners compare performance of two models, and can also be used by practitioners to understand the broader effects of algorithmic changes. Teams can use this information to understand how users engage with the system, and better optimize for future experience.

A/B testing is ubiquitous and controversial. Users of most internet services are often included as part of experiments that measure the impact of minor changes to models. \jessica{why is it controversial? I don't agree. some scholars have written about how irrational the belief it is controversial is}


\textbf{Evaluation Process and Values} The evaluation process teams undergo when setting up an A/B test is similar to the setup necessary for live testing, once it has been determined that an intervention merits an A/B test. Key decisions include the populations that will be used for each arm, and the duration of the test.

A/B tests implicate similar trade-offs to live-testing. Like live testing, A/B tests offer greater external validity. 

By evaluating a model modification with actual users, practitioners can sidestep the challenges of static benchmarks. This allows the testing of additional complexity of interactive systems, and rare events to be observed. But perhaps most significantly, A/B tests enable practitioners to pursue more exploratory forms of evaluations. A/B testing in tech companies allows testing larger changes implicating numerous different models. Through these changes, practitioners were able to study and verify long-standing assumptions about the nature of the product, and the experience of users. 

Like live testing, A/B testing also raises concerns regarding harmfulness. However, the harms surrounding live testing are often dignitary in nature. A/B tests are often critiqued for failing to gather the consent of users. Individuals have noted that A/B tests–especially in the context of technology–are akin to ``social experimentation.'' \jessica{for the good of helping more people in the population than would be helped if only one option were pursued, which is why I find it difficult to argue there is fault to this. perhaps there is an argument about not being able to gaurantee that any individual wouldn't be better under the alternative treatment (or whatever the default would be with no A/B test) but I don't think we are making that argument in a convincing way} As they are conducted in industry settings, these tests usually occur without the traditional IRB approval that would regulate similar experiments in academic contexts. Additionally, A/B tests can significantly alter the experience for some subset of users–sometimes in materially negative ways. Practitioners are evaluating developmental models still under development, so users exposed to the model may be subject to an increased risk of model mispredictions. Critics have noted that LinkedIn's experiments varying social ties may have diminished job prospects for individuals in the experiment, depriving them of opportunities for upward mobility ~\todocite{??}.  


%In A/B testing, engineers deploy an experimental model on a subset of users, and collect metrics corresponding to the model's performance on those users~\cite{seldon2021, bright2021, luigi2020, amatriain2019,shankar2022}. Metrics could directly measure model performance (e.g., accuracy of a prediction), or a downstream impact of performance (e.g. the time users spend on a platform). In deciding whether to deploy a model, practitioners will compare metrics computed for the experimental model against metrics of the status-quo on a control group of users. 


\subsection{Adversarial Testing}

\textbf{Definition}

In adversarial testing, practitioners intentionally seek out cases where models can behave in ways would be undesirable. This can be done by individually selecting malicious inputs to provide to models, and manually observing the corresponding outputs. The aim of this direct intervention approach is to allow engineers to uncover model failures or vulnerabilities, and identify corrective steps. Adversarial testing is typically done prior to release of models, or is done on released models as part of an iterated deployment process \cite{googadv, shevlane2023model}. Adversarial testing is also called `red-teaming', and is done by dedicated `red-teams' in collaboration with development teams \cite{whitehouse2023}.

Adversarial testing has been used to ensure security of systems, and has gained increased popularity with the rise of public attention on safety of generative AI models. Google's Responsible AI team shared in 2023 that adversarial testing is one of three best practices for responsible generative AI \cite{croak2023}. The Biden Administration's executive order on AI mandates that NIST establishes red-teaming guidelines, and that companies developing foundation models are required to provide regular reports of their red-team performance \cite{whitehouse2023}.

\textbf{Evaluation Process and Values}
In conducting adversarial testing, teams decide what and how many adversarial test cases to use on their systems. They also decide what defines undesirable output, and what the procedure is for categorizing output as undesirable, before ultimately deciding how to correct unsafe or inaccurate behavior. There is considerable room for interpretation and subjective decisions with regards to team values. Ethical questions of fairness and harmfulness are most notably open to interpretation, and red teaming with regards to whether model output is classified as unfair or harmful is a team's decision. Beyond this, the process brings up further value issues.

The process of creating adversarial tests can raise privacy concerns. First, output analysis could require practitioners to directly examine data points corresponding to individual test cases. Depending on the test and type of data collected, the examining practitioner may be able to infer the identity of or sensitive information about an individual associated with the input data. Many large technology companies have already fired employees for abusing data privileges, and accessing private information about different users, ~\cite{jackson2021, cox2019,cox2021}, so teams need to take careful steps to ensure adversarial testing is done with respect to legal and social norms of protecting individual privacy.

The process of creating tests and labelling output can raise ethical questions around harmfulness and cultural sensitivity. 
The guidelines provided by Google's Adversarial Testing for Generative AI documentation asks that developers find and create datasets establishing safe policy, such as definitions of toxic language phrasing, going as far as recommending ``creative" phrasing. This process is likely to be harmful or culturally insensitive for the individual creating these datasets. The next step, model output labelling, according to the Google documentation, ``necessarily involves looking at troubling and potentially harmful text or images, similar to manual content moderation" \cite{googadv}.  Content moderation is established to raise value concerns of harmfulness and cultural sensitivity. 

To avoid value sacrifices around harmfulness and cultural sensitivity, some authors suggest using model-based red-teaming. Here, rather than manual testing, test inputs are generated using a language model, and a classifier detects harmful outputs. This is part of the decision making a team undergoes when deciding how to structure their adversarial tests. Potential additional considerations would be cost, interpretability, or external validity \cite{perez2022red}. 

\yannis{Interesting reference for Ethical Adversarial Testing: \cite{albert2020ethical}. It also explains that adversarial testing  in some cases negatively affects external validity, because it is often conducted in the digital domain, even for use cases that involve the physical domain, thus leading to test cases that can be unrealistic.}


\subsection{Ethical hacking}
\neha{Technically, this name might be misleading. In the security world, it seems ethical hacking can include red teaming which we define as adversarial testing....https://www.ibm.com/blog/red-teaming-101-what-is-red-teaming/}

\textbf{Definition}
In ``ethical hacking", practitioners want to predict a sensitive variable not present in the dataset using features in the dataset. For example, they may use zip code information to see whether race can be accurately predicted. This can be quite effective, as prior work on deidentification has illustrated that individuals in supposedly ``anonymized'' datasets can be easily identified using only a few features~\cite{narayanan2006break, anderson2009, de2013unique}. There are many plausible motivations for this: (1) In a form of adversarial testing, ethical hackers want to evaluate an adversary’s ability to learn the label from the data (for potentially harmful purposes), (2) Teams of practitioners wanting to learn more about the performance of their model across dimensions not recorded in their data. We detail both motivations below.

To detail motivation of ethical hacking for the purpose of learning about an adversary's abilities, we consider downstream risks of datasets. When a dataset enables accurate prediction of a sensitive characteristic, public releases of those datasets should be limited. 

To detail motivation of teams to learn about their model performance over hidden features, we look to research over the last several years in which researchers have established ways machine learning models may produce good overall error, while significantly underperforming on certain subgroups of samples~\cite{buolamwini2018gender,chen2019slice, oakden2020hidden}. The presence of these performance differentials have raised significant concerns with regards to fairness, and significant attention has been devoted to identifying and rectifying such differences. However, in practice, identifying such subgroup disparities requires subgroup identification information (e.g., gender, race, or nationality) for individuals in evaluation data~\cite{andrus2021we}. This information might not be collected because doing so would raise privacy concerns, or violate government and industry data use policies~\cite{andrus2022demographic, xiang2022being}. 

%For instance, subgroup identification is often the source of discrimination-–individuals may fear that this information may be used in other, more insidious ways. While ostensibly to prevent disparate effects, the collection of racial identification data may thus be seen as a precursor to enabling discrimination~\cite{andrus2022demographic, cabanas2020does}.

%It allows practitioners to understand properties of their datasets. Given the opacity of modern machine learning systems-–and the difficulty in specifying which types of correlations should be learned from data-–understanding the correlations that exist can be an important indicator of the risk of bias. For instance, if practitioners observe that a feature facially unrelated to gender (e.g., an applicant’s college major) actually encodes strong information about the applicant, then they may elect to remove that feature from their dataset. 

However, prior work akin to ethical hacking has also inspired controversy. Recent studies have attempted to predict a range of attributes (e.g. sexual orientation, criminality, etc) from photos of faces~\cite{paullada2021data}. These studies have been critiqued for presupposing that such predictions are possible, or reflective of underlying casual mechanisms. Other researchers have pointed out that much of the performance can be explained by correlated proxies present in the data~\cite{aguera2018}. 

\textbf{Evaluation Process and Values}
Key decisions in ethical hacking is the model and dataset to be used in predicting unknown variables, as well as how to store these predictions.

Ethical hacking allows for privacy by not directly collecting or storing a users data or information. Some researchers suggest private data collection can ensure that algorithmic fairness methods are more likely to be successful in mitigating treatment disparities, but others say collecting private data is often a precursor to actively enabling discrimination \cite{andrus2022demographic}. \neha{Add more references to this paper, it's good.}

When ethical hacking is done because private data is not provided, regardless of practitioner decisions, the prediction is guaranteed to lack external validity. It is impossible to evaluate the accuracy of the predicted variable with statistical certainty. Furthermore, the model used to predict unknown variables can be interpretable or uninterpretable based on team decisions. 

%subgroup identification is often the source of discrimination-–individuals may fear that this information may be used in other, more insidious ways. While ostensibly to prevent disparate effects, the collection of racial identification data may thus be seen as a precursor to enabling discrimination~\cite{andrus2022demographic, cabanas2020does}.

Ethical hacking should only be done if the goal is positive social impact rather than harmfulness. One popular example is in the work done by \citep{elzayn2023measuring} in which they use the Bayesian Improved First Name and Surname Geocoding (BIFSG) method to impute race on tax return data provided by the US Treasury, based on full name and geographic location.  The authors conclude that Black taxpayers are audited at much higher rates than non-Black taxpayers, and gained commitment from government officials towards addressing biases in audit selection algorithms.

% It is important that if ethical hacking is done, prediction is done using interpretable algorithms. BISFG is one of many popular methods in a growing field of algorithms aiming to improve the accuracy and interpretability of race prediction, also including \cite{jain2022importance}. Race prediction has been applied by health and social science researchers in a number of contexts beyond this one, such as in measuring disparities in COVID-19 outcomes, or traffic safety outcomes \cite{sartin2021facilitating}.


\subsection{Benchmarking and/or Simulation Testing}
todo: need more references if any available. 

\yannis{Simulation testing is often used for evaluation of interactive machine learning systems. These are interactive systems, whose output depends on the actions carried out by the users. While evaluating such systems, user simulation can be used to evaluate the system without having to recruit real users for testing, thus avoiding the associated monetary and time costs. On the other hand, the simulation may not fully reflect the behavior of the actual users, thus trading off external validity for cost. Examples of simulation testing include evaluation of dialogue systems \cite{scheffler2001corpus, jung2009, crook2017sequence, zhang2020usersimulation}, interactive systems for information extraction \cite{hanafi2022}, etc.}

\subsection{Data Splitting}

\textbf{Definition}

Practitioners partition the population into different slices of data, and monitor the performance of the model within a slice. A slice consists of a strata of data points characterized by common attributes, oftentimes divided by demographic characteristics. Slice performance is critical as it drives evaluation, with the ability to halt wider model deployment if slice performance is low.

 This is similar to A/B testing, in that performance is evaluated on a subset of the population, but performance does not need to be compared across multiple subsets, and rather than a randomization of individuals across treated and control subsets, there is a deliberate placement of individuals into the slice receiving treatment.

 After results of models are measured on slices, the models may be modified as needed prior to release.

 \textbf{Evaluation Process and Values}

 Developers must determine which slices are most relevant for evaluating models on, as well as an appropriate size of a slice. This  likely requires collecting relevant demographic details of the individuals in the slice, which could lead to privacy considerations.
 
 Determining slices might not be a straightforward task and may involve discussions of fairness values. Laws and regulations may, a priori, classify certain subgroups as ``protected'' and create legal penalties for failing to equalize performance across these subgroups. Other tasks may contain data which naturally divide into simpler groups that are amenable to measuring. For instance, in multi-class tasks--where a model must map each sample to one of $k$ classes--each class forms a natural slice.
 
 Practitioners also decide the testing evaluation criteria within the slice. Overall, their aim is to guarantee deployment outside of the slice is likely to succeed based on performance within the slice.

Thus, a core challenge is accuracy of external and internal validity. An example of slice identification where this is a concern is in medical device testing. Pre-deployment evaluation studies may be performed on patients in one site, leading to criticism in the medical community. The use of data in a single slice of the population does not permit validation in heterogeneous populations. In \cite{wu2021medical}, the author review 130 FDA-approved medical devices and note that pre-deployment evaluation studies for 93 of these devices were not performed on patients in more than one site. They highlight the importance of multi-site assessment in clinical trials, because a small number of sites can indicate limited geographic or demographic diversity in the patients a device is tested on. 

Furthermore, algorithmic or dataset modifications following results from data splitting, might improve metrics for minority subgroups while reducing performance for majority subgroups. Many possible explanations exist for this phenomenon. For instance, models have limited representational capacity. When different subgroups implicate different features, learning better representations for one subgroup may require sacrificing the model's ability to capture meaningful representations for other subgroups~\cite{chen2019slice}. 

This phenomenon forces practitioners to negotiate an ethical tradeoff when selecting which model to deploy. If no model maximizes performance over all subgroups, any choice of model will require sacrificing performance on some subgroup. Moreover, there is no clear principle to guide this decision. A utilitarian perspective--which would seek to maximize performance for as many people as possible--would prefer interventions which boost performance for larger subgroups at the cost of smaller subgroups. In contrast, perspectives which favor formal protections for minorities--often reflected in our social and political structures--would accept reductions to majority group performance if accompanied by improvements to minority group performance. Ultimately, this is a value question of internal and external validity, as well as domain based potential additional considerations of harmfulness or fairness.








\jessica{Overall, while I think some good points are made, it reads as pretty anecdotal. It would be nice if there was some deeper structure in how these trade-offs are discussed. I'm not sure the current draft rises to the level of articulating something generalizable. }


\begin{itemize}
    \item The case of Tesla's automated driving live testing has parallels to many of the non-machine learning ethical interventions. This includes automotive crash testing, in which there are incentives to invest in simulation testing prior to release.
    \item The case of Microsoft's chatbot live testing followed intermediate testing that was unable to expose vulnerabilities prior to the live test. Federal enforcement that ethical harms of accessibility are required in construction 
    \item The case of Facebook's A/B testing regarding NewsFeed happiness has drawn criticism of A/B testing not following precedents of clinical trials, in which there is informed consent, and a centralized agency overseeing approval of potential ethical concerns.
    \item The case of Watson's AI for Cancer model illustrates the importance of careful use of synthetic data in testing. This could benefit from many of the ethical interventions, such as widening the testing done prior to release. 
    \item Research on AI Medical device testing illustrates the importance of potential testing frameworks $D$ having wide ranges of population. This is similar to the enforcement of ...
    \item Research on Adversarial testing shows concerns regarding the use of human subjects in model output labelling. This has similarities to xx
\end{itemize}


Through specialized testing programs, California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}. The program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles “test drove” at least four million miles on public roads in California~\cite{bellan2022}. In the Tesla Autopilot systems, the systems was trained and tested on public roads with other drivers and involved in several tragic fatal crashes \cite{siddiqui2022}.

% general statement on live testing ML
Live testing provides valuable information for evaluating performance such as testing performance on real-time rare events. Driving is a long tailed distribution, containing many rare events which could confuse an autonomous navigation system~\cite{ackerman2017}. Real world roads contain phenomenon that are difficult to simulate in synthetic environments: inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. By testing on live roads–in a variety of diverse environments–engineers can study when systems return manual control to the human driver~\cite{banerjee2018}. Studying these interventions allows them to identify failures in perception or control systems~\cite{wang2020safety}. They can also interview passengers of the car, allowing them to learn more about the smoothness of the ride and identify instances of erratic behavior~\cite{donfro2018}. Thus, there is information gained from live testing. \neha{todo check citations}

\textbf{Utility Framework Analysis}
Tesla's live evaluation practice aims to yield information gain in training and testing the autonomous driving systems, but the utility of the testing is significantly diminished by the ethical harm to society of harmfulness and diminishing roadway safety, as proven by the tragic deaths that have occurred \cite{siddiqui2022}. Media and researchers have noted the harmfulness of live testing strategies, and have made calls suggesting improving the safety of testing automated driving systems \cite{burton2017making, li2022safety}. Others have suggested techniques to improve safety of systems through actionable testing steps or error detection strategies among others \cite{mohseni2022taxonomy}. 



==> old/old_04_evaluation_practices.tex <==

\subsection{Live testing}

\textbf{Definition}

A common evaluation workflow is to deploy a developmental model on a subset of the user population, in order to collect statistics regarding its performance. We refer to this practice as \textit{live testing}. By allowing the model to operate in real world-settings, practitioners are able to understand and study its performance.
\jessica{It would be nice if there was a more precise way to talk about this. I think a formalization would be helpful to set up earlier. E.g., evaluation is about getting information about performance, which can be used to serve certain values. When getting that information leads to threats to other values, ethical concerns can enter. (though I'm not sure what our definition of ethical is). We could formalize things more in terms of an underlying cost-benefit question that is often overlooked: is the utility I expect to get from the additional information the eval brings greater than the utility I expect to lose from harms induced by the evaluation process. Our argument can be that this is often happening implicitly and this can lead to lost utility (worse outcomes) overall. It would be nice if our values included the kinds of values people care about when they go to collect more eval data (see my comments above about dividing values into properties and outcomes. Predictive power could be added as a property we want to achieve (which is why ppl usually collect more eval data), subsuming internal and external validity }

The most notable use case is in the evaluation of autonomous vehicles. Through specialized testing programs, California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}. The program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles “test drove” nearly five million miles on public roads in California~\cite{bellan2022}. However, live testing–especially in the context of autonomous vehicles–is not without controversy. 

 
\textbf{Evaluation Process and Values} Teams must decide when a live test is appropriate for a model and when to begin, as models are usually evaluated on static validation sets before being live tested, and the amount of evaluation necessary before executing a live test is subjective. 
Teams must also decide the population for the test, and the manner in which the test is executed. Often, which users receive the experimental model can be controlled. Hence, they can construct the test to capture (or ignore) certain populations or settings. Finally, teams control the duration of the test.

Live testing benefits external validity. Using real-time data to evaluate avoids problems with unrepresentative validation sets~\todocite{OOD/distribution shift/long tails}. It also allows developers to capture metrics that may be challenging to measure in offline validation, because they pertain to user behavior. Live testing with autonomous vehicles exemplifies these advantages. Autonomous driving has a long tail–cars are expected to navigate incredibly diverse conditions impacted by weather, road construction, obstacles, and traffic. Developing simulations or validation datasets to capture all of these settings is prohibitive. Moreover, live testing allows developers to measure how a particular model changes driver behavior–developers often quantify performance in terms of the number of times a human driver ``retakes control'' of the vehicle. This requires an actual human in the loop, and is difficult to simulate offline. 


However, live testing can increase the harmfulness of an evaluation. Developmental models carry more uncertainty, and have only been partially validated. Hence, the risk of model misclassifications is higher. In low risk settings, the dangers of mispredictions are minimal, and may only result in harms of convenience~\todocite{Deb paper on models not working}. But in high risk settings, model mispredictions can result in significant physical or emotional harm. Autonomous vehicles, for instance, have already been involved in a number of crashes that have harmed drivers and bystanders. Errors with developmental content moderation models, could expose users to harmful content, potentially leading to significant distress. 
\yannis{Another potentially harmful aspect of live testing is that software undergoing live testing often exhibits security vulnerabilities, thus opening up developers and users to potential security and privacy risks. The reason for this is that software security is often addressed only in later stages of the software development cycle \cite{karim2016}.}

%One prominent illustration of ``live user testing'' occurs with self-driving vehicles. Through specialized testing programs, California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}. The program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles “test drove” nearly five million miles on public roads in California~\cite{bellan2022}. Live testing of autonomous vehicles provides valuable information for evaluating performance. Driving is a long tailed distribution, containing many rare events which could confuse an autonomous navigation system~\cite{ackerman2017}. Real world roads contain phenomenon that are difficult to simulate in synthetic environments: inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. By testing on live roads–in a variety of diverse environments–engineers can study when systems return manual control to the human driver~\cite{banerjee2018}. Studying these interventions allows them to identify failures in perception or control systems~\cite{wang2020safety}. They can also interview passengers of the car, allowing them to learn more about the smoothness of the ride and identify instances of erratic behavior~\cite{donfro2018}. None of this could be measured in a laboratory. 
 

%Additionally, individuals in a live test may be deprived of access to a superior experience. Suppose engineers are seeking to evaluate a model which they belive more accurately performs a task for users. By choosing a subset of users to operate in the control group, the engineers are deliberately depriving them of the opportunity to recieve what they believe is a superior experience. 

%Thus, the decision to live test a model forces engineers to tradeoff between the correctness of an evaluation and the harm it may inflict. If engineers valued the correctness of an evaluation, then the ancilliary harms to users though live testing would be an acceptable cost. Similarily, choosing not to perform a live test would indicate that engineers valued the minimization of harm over the accumulation of additional evaluation information.



==> old/old_04_neha.tex <==
\subsection{Sensitive data collection for error analysis}

% Cite to: https://www.consumerreports.org/privacy/teslas-in-car-cameras-raise-privacy-concerns-a9884415005/

\textbf{Practice}. In order to understand model mispredictions, engineers will sometimes collect or leverage additional metadata about samples for which the model mispredicts. The type of metadata collected and the information it provides can be wide ranging. Demographic data about individuals (e.g., race, gender, etc.) can enable practitioners to quantify a model's fairness~\todocite{fairness work}, or the demographic representativeness of a dataset. In medical contexts, information about patient history can help developers notice spurious correlations, or patients for whom model performance may be poorer. Sometimes, developers will need to collect the model inputs so engineers can inspect model inputs. Inspecting samples from deployment can help developers understand the deployment distribution, and the source of model errors. This is especially valuable in unstructured domains like image or speech processing, where boolean operations to process data are unavailable~\todocite{domino work}. 

\textbf{Evaluation decisions}. Collecting metadata for error analysis requires a range of evaluation decisions. Developers must first decide what information to leverage in analysis (e.g. gender or race). When such information isn't already available, developers must design protocols for collecting it. For demographic data in particular, developers must decide on the grouping scheme to be used (e.g. how granularly is race represented?). Developers must also decide \textit{who} to collect information from. While randomly selecting individuals may yield a uniform sample, developers may be particularly interested in minority groups, which requires more targeted sampling techniques. Even after collecting data, developers will need to make decisions regarding data use and storage policies. For instance, will collected data be saved in perpetuity, or is it subject to auto-deletion after a period of time? Developers must also decide which engineers will be permitted to access sensitive data, and the manner in which information will be presented to them. For instance, will the engineer's view of the information be restricted to only that which is deemed to be technically necessary, or will they have access to all information associated with a prediction?   

\textbf{Dimensions and tradeoffs}. Evaluation decisions which expand the scope of error analysis–allowing for more information to be collected-generally improve the interpretability of evaluation. Prior work illustrates that additional metadata enables uniquely valuable forms of evaluation. Properties like fairness are impossible to measure without accurate subgroup information. Though efforts to impute sensitive attributes do exist, they're often inaccurate, or require practitioners to make significant simplifying assumptions. Manual error analysis also enables practitioners to identify and group distinct families of errors~\cite{shankar2022}. In practice, these can inspire the development of new tests. 

However, such decisions also diminish the evaluation's adherence to privacy. Collecting more information about individuals raises questions about awareness (do individuals know their personal information is being used in this way?), consent (do they permit such use?), and accuracy (is the information being collected actually correct?). These concerns are heightened for demographic information, which is often regarded as especially sensitive~\todocite{Alice Xiang and Andrus work}. Greater data collection also increases the risk of harm stemming from developer misbehavior or negligence~\todocite{articles on illicit access of data by engineers/crowdworkers}. 

\hari{I think this version has a lot of the information we need to describe the ethical trade-off and highlight decision points. But the current organization makes it a bit repetitive and lacks coherence. How about something like this:}

To evaluate model fairness, engineers must analyze performance disparities across different population sub-groups. This requires collection and access to additional metadata to improve the interpretability of model performance. For example, in the medical domain, information about patient history can help data scientists notice spurious correlations, or patients for whom model performance is poor. Or in a loan-granting scenario, demographic information can help assess model performance for marginalized subgroups. However, in such analysis, there is a \textbf{trade-off between fair evaluation and adherence to data privacy}, which current practices are not equipped to handle. To ethically evaluate for model fairness, practitioners assess privacy trade-offs in making the following decisions:

\hari{In each of the following paragraphs, we can talk in more detail about approaches and corresponding trade-offs, and unanswered questions.}

\textit{What information to collect:} Developers must first decide what information to leverage in analysis (e.g. gender or race). Collecting more information about individuals raises questions about awareness (do individuals know their personal information is being used in this way?), consent (do they permit such use?), and accuracy (is the information being collected actually correct?). These concerns are heightened for demographic information, which is often regarded as especially sensitive~\todocite{Alice Xiang and Andrus work}. \hari{What does prior literature tell us about how practitioners identify what metadata to collect? Whether/how do they assess trade-offs? What are open questions.... these paragraphs can generate questions for our survey with practitioners}


\textit{How to collect information:} When such information isn't already available, developers must design protocols for collecting it. For demographic data in particular, developers must decide on the grouping scheme to be used (e.g. how granularly is race represented?). Developers must also decide \textit{who} to collect information from. While randomly selecting individuals may yield a uniform sample, developers may be particularly interested in minority groups, which requires more targeted sampling techniques. Even after collecting data, developers will need to make decisions regarding data use and storage policies. For instance, will collected data be saved in perpetuity, or is it subject to auto-deletion after a period of time?


\textit{Who has access to information:} Developers must also decide which engineers will be permitted to access sensitive data, and the manner in which information will be presented to them. For instance, will the engineer's view of the information be restricted to only that which is deemed to be technically necessary, or will they have access to all information associated with a prediction? Greater data collection also increases the risk of harm stemming from developer misbehavior or negligence~\todocite{articles on illicit access of data by engineers/crowdworkers}. 

\subsection{Annotating for content moderation}

\textbf{Practice} Reliance on crowdworkers for data annotation is ubiquitous in machine learning development. Though techniques for automating data labeling are being developed, manual annotation is still the gold standard. Annotation is especially ubiquitous for tasks like content moderation, where humans are required to make subjective determinations regarding the toxicity, profanity, or explicitness of different types of online content. Many platforms manage thousands of human workers, who annotate and filter hundreds of thousands of posts and messages every day for compliance with platform rules. \neel{Still in progress} 

\textbf{Decisions}

\textbf{Dimensions/tradeoffs}



A/B testing presents the following advantages: 
\begin{itemize}
    \item Because practitioners can run a development model on live data, concerns associated with static datasets (e.g. distribution shift, rare events/long tails, out-of-distribution data) are less salient (\textbf{external validity}). 
    \item Because practitioners can observe how users respond to model outputs, A/B testing allows practitioners to evaluate models deployed in complex, interactive systems (\textbf{external validity}). In an application like autonomous driving, practitioners can measure the number of times a user grabs the steering wheel, or performs a similar corrective action. Performing such evaluations without the aide of A/B testing may require building complex simulations (\textbf{cost}), which themselves would make simplifying (and sometimes incorrect) assumptions (\textbf{external validity}).
    \item Because the longer-term effects of models can be observed in system behavior, practitioners can actually measure the metric of interest (\textbf{interpretability}). For instance, in a task like content moderation (where labels can often be subject to disagreement), practitioners can actually measure whether certain models are correlated with less or more time on the platform, which itself may measure user satisfaction. 
\end{itemize}
However, A/B testing presents the following concerns:
\begin{itemize}
    \item As practitioners are evaluating developmental models still under development, users exposed to the model may be subject to an increased risk of model mispredictions. Depending on the application, this can expose users to various types of physical \textbf{harm}. Autonomous vehicles operating in testing programs have crashed during testing, resulting in tragic injuries and loss of life to other road occupants~\cite{associatedpress2022, kao2022}. These sorts of failures have produced significant controversy, leading some to call for more stringent regulation regarding the ability for autonomous vehicle companies to test on public roads. 
    \item When practitioners have strong reason to believe that a particular model is superior (as was the case in LinkedIn's tests~\cite{}), the denial of the superior model to users in the control group deprives them of a benefit, thereby inflicting \textbf{harm} on them. \jessica{is there lit on the philosophy behind why this is wrong, ie why should we assume that as engineers we owe the best experience we know to everyone?}
    \item Users often lack the ability to consent to participation in an A/B test. As policymakers increasingly recognize a ``right'' for users to know whether they are interacting with algorithms, A/B testing with machine learning models may also inflict dignatory \textbf{harm}~\cite{engler2020}.
    \item Finally, A/B tests may disproportionately result in harm to certain vulnerable populations, especially when that population holds valuable data~\cite{fussell2019google}. In these instances, A/B tests may diminish \textbf{fairness}.
\end{itemize}

\subsubsection{Slice identification}

Machine learning researchers have found that in many settings, a model may provide high overall performance (i.e. \textit{global}) on a test set, but significantly struggle on certain subgroups of data (often termed as \textit{slices})~\cite{blodgett2016demographic, chen2019slice,oakden2020hidden, hashimoto2018fairness}. The discrepency between high global performance and low subgroup performance has been observed in a variety of domains. In facial recognition for instances, practitioners have noticed that models significantly underperform on racial minorities and women~\cite{buolamwini2018gender}. In healthcare settings, practitioners have observed that chest x-ray models underperform on patients with certain surgical implants~\cite{oakden2020hidden}. 

As a result, a common evaluation practice is to identify, define, and engineer slices into evaluation frameworks~\cite{goel2021robustness, re2019overton, eyuboglu2022domino}. Here, practitioners will independently evaluate the model on test samples representing a certain slice. In addition to analyzing aggregate performance over the entire test set, practitioners will look to slice performance to determine model quality. As an example: practitioners building a recognition system for an autonomous vehicle may define a slice consisting of images that contain cyclists at night~\cite{chen2019slice}. In practice, an evaluation system can contain numerous slices~\cite{re2019overton}.

Measuring performance on a slice serves a variety of functions. First, practitioners may use slice performance to guide the model development process. If a model is underperforming on a particular slice, practitioners will take steps to improve performance on that slice. This could include: adding more training data from the distribution captured by the slice, adding more features, or modifying the architecture of the model. Second, practitioners use slice performance to determine when to deploy a model. If performance on a slice is too low, practitioners delay deployment until the problem can be alleviated.

However, determining \textit{which} slices are worth measuring can be a challenging endeavor. In defining a slice over a subset of samples, practitioners are explicitly prioritizing the performance of the model on those samples over performance on other samples. Hence, slice selection requires value judgements on the part of practitioners. 

In some settings, determining slices may be a straightforward task. 

In many cases however, the choice of which slices to measure is less clear. Practitioners may have access to rich demographic descriptions of individuals in a dataset. Different demographic attributes could be combined to capture the intersection of different identities. Consider, for example, a healthcare company developing a chest x-ray model to deploy at different hospitals. The company can construct slices using a plethora of information: patient age, race, gender, locale, or previous medical history. Slice descriptions could become arbitrarily complex (e.g., ``male patients with high cholestroal between the ages of 25 and 35 in the Pittsburgh area'').

Adding slices can come at a cost. Practitioners must ensure that slices contain sufficient samples to yield statistically powered measurements. For slices corresponding to rare subgroups, gathering sufficient data can thus be expensive or difficult. As practitioners add slices moreover, the significance of existing slices are diluted. 

Thus, the process of formalizing slices presents practitioners with an ethical tradeoff. On the one hand, creating a slice enables practitioners to better understand the performance of the model, and detect when a particular subgroup experiences lower-than-average performance. Yet, the choice to define some slices–-and not others--places different subgroups on different footings, implicitly valuing certain populations over others.  
\jessica{how does this relate to framework?}

\subsubsection{Slice prioritization}

A challenge that follows from slice identification is \textit{slice prioritization}. When performance on a slice is low, practitioners may pursue a range of strategies to improve metrics. This can include collecting additional data~\cite{vokinger2021mitigating} or altering training strategies~\cite{sagawa2019distributionally, liu2021just}. By applying such interventions, practitioners can often improve performance for minority subgroups present in the data. 

Unfortunately, researchers have observed that such interventions often \textit{decrease} performance for other subgroups~\cite{liu2021just, zhang2022correct, sohoni2020no}. In practice, algorithmic or dataset modifications which improve metrics for minority subgroups reduce performance for majority subgroups. Many possible explanations exist for this phenomenon. For instance, models have limited representational capacity. When different subgroups implicate different features, learning better representations for one subgroup may require sacrificing the model's ability to capture meaningful representations for other subgroups~\cite{chen2019slice}. 

This phenomenon forces practitioners to negotiate an ethical tradeoff when selecting which model to deploy. As no model maximizes performance over all subgroups, any choice of model will require sacrificing performance on some subgroup. Moreover, there is no clear principle to guide this decision. A utilitarian perspective--which would seek to maximize performance for as many people as possible--would prefer interventions which boost performance for larger subgroups at the cost of smaller subgroups. In contrast, perspectives which favor formal protections for minorities--often reflected in our social and political structures--would accept reductions to majority group performance if accompanied by improvements to minority group performance.

\subsubsection{Slice identification}

\textbf{Practice}
%Practitioners monitor performance for different slices. A slice consists of a strata of data points characterized by common attributes. 

%Examples of slices could include: 
%Individuals with a particular set of demographic characteristics (e.g. women, individuals from China, etc.)
%Samples which contain a particular features (e.g. chest X-rays with chest drains)

%As slices are considered to be critical, slice performance can drive evaluation. Practitioners need to ensure that a slice is sufficiently well represented in test data, which may involve specifically collecting data corresponding to a slice. A model’s deployment may be halted if slice performance is too low, and engineers will investigate remedies for improving performance. 

%A site will be accompanied by limited geographic or demographic diversity, which raises concerns regarding the overgeneralizability of research findings due to heterogeneity in health needs across genetically and sociologically disparate populations.}

\textbf{Decisions} \neha{}

\textbf{Dimensions/tradeoffs}
\neha{
Slice identification lacks external validity. T
% My personal casual interpretation of this problem is as follows: The testing of these devices in limited sites would indicate the assumption that given health outcome $H$ and class membership $B$, the clinical trials operate under the belief that believe that $\mathbb{E}(H|B=1)=\mathbb{E}(H|B=0)$. Although the clinical trials do not directly predict class membership $B$, or do any ``ethical hacking", they have created an assumption on that variable.

In \cite{national2022improving}, the authors highlight seven threats to healthcare if there is a lack of representation in clinical research, including overgeneralizability of research findings due to heterogeneity in health needs for genetic and socioeconomic reasons, downstream lack of access to effective interventions due to limitations in obtaining approval of treatments for all populations, potential compounding effects of health disparities, and increased costs. 

In \cite{clark2019increasing}, the authors identify critical barriers to inclusive clinical trials, and solutions that might allow dismantling these barriers. Some of the recommendations they offer include language that will emphasize available support and appreciate involvement. Additionally, they recommend making trials more patient centric and offering transportation. The FDA has offered recommendations for a standardized approach to collecting race and ethnicity data in clinical trials [cite], so that studies have knowledge of what slices have been studied.

Generalizing these recommendations outside of clinical trials or medical device evaluation; More broadly, developers can mitigate the tradeoff to the external validity by making slice participation more easy and having a wider representative slice. 

Slice identification also raises concerns of harmfulness or fairness, although the degree of this would be unique to the problem and whether there is in actuality a difference in outcomes for the population that was not part of testing compared to the population that was used. A likely advantage of slice identification is that it may be cost effective to avoid needing to test models on a wide range of individuals. [Didn't comment on internal validity/interpretability...]}



==> old/old_04_tradeoffs.tex <==
\section{Existing ethical dimensions}
In this section, we identify evaluation practices which balance different values. 

\subsection{Knowledge vs Harmfulness}

A variety of evaluation practices tradeoff between harmfulness, knowledge, and fairness. These are evaluation practices which increase the likelihood of--or actually inflict-–some type of harm on certain populations of individuals. Moreover, the harm inflicted is rarely uniform–certain subgroups are often at greater risk of harm.  

However, these practices often provide practitioners with detailed knowledge about the performance of their system. The risk of harm and the informational value of these practices are often coupled, and hence, best understood as a natural tradeoff. Many practices exemplify this tradeoff.

\subsubsection{Existing practices}

\underline{Live testing}: Practitioners sometimes partially deploy models–allowing them to operate in certain real world settings–in order to better understand and study performance. For instance, a variety of autonomous vehicle manufacturers “test” autonomous driving systems on California roads through a specialized testing program~\cite{dmvpermitholders}. Between December 2020 and November 2021, autonomous vehicles “test drove” nearly five million miles on public roads in California~\cite{bellan2022}.

Live testing of autonomous vehicles provides valuable information for evaluating performance. Driving is a long tailed distribution, containing many rare events which could confuse an autonomous navigation system. Real world roads contain phenomenon that are difficult to simulate in synthetic environments: inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. By testing on live roads–in a variety of diverse environments–engineers can study when systems return manual control to the human driver~\cite{banerjee2018}. Studying these control switches allows them to identify failures in perception or control systems~\cite{}. They can also interview passengers of the car, allowing them to learn more about the smoothness of the ride and identify instances of erratic behavior. None of this could be measured in a laboratory. 

However, live testing–-particularly with autonomous vehicles–-can manifest in many harms. Some of these harms are “dignitary,” relating to violations of consent or inflictions of emotional distress. While the driver of an autonomous vehicle consents to being transported by an autonomous system, other individuals on the road have little say. Indeed, most drivers believe–-and drive under the reasonable assumption–that other vehicles are controlled by individuals who have been subject to stringent training and testing. Knowing that an autonomous vehicle–-controlled by untested systems-–is proximate to them, or present in their communities-–can be a source of great distress. Beyond these dignitary harms, live testing failures can result in physical harms. Autonomous vehicles have crashed during testing, resulting in tragic injuries and loss of life to other road occupants. These sorts of failures have produced significant controversy, leading some to call for more stringent regulation regarding the ability for autonomous vehicle companies to test on public roads. 

\underline{Harms to crowdworkers}: Sometimes, the construction of evaluation datasets–critical for assessing the performance of models–-can also result in harms to individuals. Consider the example of machine learning for detecting explicit content. Machine learning models are deployed by a range of platforms for content moderation purposes. Here, the goal of the model is to identify content containing explicit, illegal, irrelevant, or obscene materials, for the purpose of removing that content from the platform.

Ensuring that machine learning systems for content moderation perform well requires constructing test sets which are capable of accurately evaluating those models. Test set construction is especially important in this context. As a task, content moderation is subject to frequent distribution shifts. Adverse actors frequently experiment with a range of tactics to bypass models, and new forms of explicit and illegal content are being generated every day. Hence, evaluation test sets must be continually updated to reflect evolving trends. Failures of content moderation systems are often public and derided, placing increased pressure on engineers. 

However, the creation of these test sets requires crowdworkers to observe and annotate actually harmful content. The content that moderators see is often considered to be highly distressing, depicting graphic forms of violence and other disturbing acts. Various studies have shown how individuals responsible for annotating these materials often suffer longer term traumatic stress disorders and experience burnout. 

Moreover, annotators are often drawn from non-Western countries, where they often work in borderline exploitative conditions for little pay. This has given rise to concerns that-–for harmful tasks like content moderation–-certain demographic groups disproportionately suffer the longer term harms.

\underline{Privacy}: Error analysis–-the process of examining model misclassifications to better understand the source and origin of the errors–-is considered to be an integral part of the evaluation pipeline. By actually examining where the model goes wrong, practitioners can attribute errors to failures in the design and  construction of models, enabling them to take better remedial decisions. In the past several years, a wealth of literature has offered tools for helping practitioners with this endeavor.

Yet, the process of error analysis raises a variety of privacy concerns. First, error analysis requires practitioners to directly examine data points corresponding to individuals. Depending on the task and type of data collected, the examining practitioner may be able to infer the identity of or sensitive information about the individual associated with the data point. 

Second, error analysis may require collecting additional sensitive information about the individual. Over the last several years, practitioners have improved their understanding of how machine learning models may produce good overall error, while significantly underperforming on certain subgroups of samples. The presence of these performance differentials have raised significant concerns with regards to fairness, and significant attention has been devoted to identifying and rectifying such differences. In practice, identifying such subgroup disparities requires subgroup identification information (e.g., gender, race, or nationality) for individuals in evaluation data. Collection of this information raises significant privacy concerns. Subgroup identification is often the source of discrimination-–individuals may fear that this information may be used in other, more insidious ways. While ostensibly to prevent disparate effects, the collection of racial identification data may thus be seen as a precursor to enabling discrimination.  

\underline{Ethical hacking}: Sometimes, researchers attempt to evaluate the properties of a dataset, by training a model to predict a secondary task from the data. A frequent illustration of this is found in work on dataset bias, where researchers evaluate the extent to which certain features encode information about race or gender by having a model learn to predict race/gender from those features. We refer to this practice as “ethical hacking.”

Ethical hacking has important benefits. First, it allows practitioners to understand properties of their datasets. Given the opacity of modern machine learning systems-–and the difficulty in specifying which types of correlations should be learned from data-–understanding the correlations that exist can be an important indicator of the risk of bias. For instance, if practitioners observe that a feature facially unrelated to gender (e.g., an applicant’s college major) actually encodes strong information about the applicant, then they may elect to remove that feature from their dataset. Second, ethical hacking allows researchers and practitioners to understand the downstream risks of a particular dataset. When a dataset enables accurate prediction of a sensitive characteristic, public releases of those datasets should be limited. In the context of privacy, such forms of ethical hacking can better inform when model releases should be accompanied by datasets. 

However, ethical hacking has also inspired controversy. Projects engaging in ethical hacking–-like [], which infamously attempted to train models to predict sexual orientation from social media profile pictures-–have been critiqued for leveraging task framings which perpetuate harmful stereotypes, ground in unsound science, and misinterpret results. Similarly critiqued tasks include studies of generating facial images from audio recordings, and predicting criminality from photos. 

Additionally, ethical hacking raises questions about the proliferation of harmful machine learning methodologies. Studies have shown, for instance, that protein folding models–-originally designed to guide drug exploration-–can be engineered to design toxic compounds and bioweapons. The proliferation of computational power and data means that the barrier for entry for developing such models is alarmingly low. Though the publication of such research is intended to raise awareness, it could inadvertently empower malicious actors to develop these tools. 


\subsubsection{Analogous discipline: clinical trials}

We find that the tradeoffs present here–-balancing the risk of user harm against the benefits of more accurate evaluation–-mirror those that arise in medical clinical trials. In clinical trials, medical practitioners evaluate experimental treatments or drugs on human patients, in order to better study the efficacy and safety of the interventions. As these treatments are experimental, participants in trials endure a non-trivial amount of risk. We begin by reviewing the ethical considerations of clinical trials, before suggesting several guiding principles that machine learning engineers can borrow. 


Medical practitioners employ many different types of clinical trials, depending on the treatment being tested and the stage of development. These trials pose different ethical considerations. 

For instance, placebo controlled trials--in which a subset of patients are given a ``placebo treatment'' that will not improve their condition--raises concerns around intentionally depriving a group of treatment. First, placebo controlled trials would appear to violate the professional obligations of doctors to provide the optimal medical care to patients~\cite{miller2002makes}. Second, when other known beneficial treatments exist--denying patients access to those treatments for the sake of measuring the efficacy of the novel treatment against a placebo is both clinically and scientifically questionable~\cite{miller2002makes}.

However, the ethical concerns emerging from placebo controlled trials should be balanced against their prospective advantages. Placebo trials are widely considered to be the most rigorous test of treatment efficacy~\cite{miller2002makes}. They generally require fewer participants that active-controlled trials, thereby making them easier and cheaper to conduct~\cite{miller2002makes}. Even where existing treatments exist, placebo trials offer new and valuable forms of information~\cite{miller2002makes}. 

Thus, medical practitioners have come to identify several principles that guide determinations as to when placebo trials may be appropriate~\cite{millum2013ethics}. First, placebo trials are permissible when no proven treatment exists for the disorder being studied (e.g., for Alzheimer's dementia). This includes the setting where a treatment may exist, but its efficacy cannot be extrapolated to the population of interest. Here, the absence of a proven treatment means that placebo participants are therefore no worse off than if they weren't participating in the trial. 

Second, placebo trials are permissible when preventing patients from acessing a known alternative treatment would expose them to at most ``temporary discomfort or delay in relief of symptoms.'' This is common when the medical disorder being studied is ``minor,'' like common headaches or male pattern baldness~\cite{miller2002makes, millum2013ethics}. In these settings, placebo trials are considered ethical as the harms are often minute enough to justify the investigative value of these trials. 

Third, placebo trials are justified when existing treatments prove to be highly variable. This is commonly the case for conditions like depression, where established drugs can sometimes fail to outperform placebos~\cite{millum2013ethics}. Here, comparing a new drug to an existing drug can diminish the internal validity of a study~\cite{miller2002makes}. If both the efficacy of both drugs are indistinguishable, then it could be the case that either both drugs are effective, or neither are. Here, placebo trials are ethical as the lack of medical confidence in superiority of existing treatments over a placebo diminish the harm inflicted on placebo participants.

Finally, placebo trials are permitted when there existing compelling methodological reasons for their use, participants are not deprived of treatments they would otherwise have acess to, and the benefits of the trial will be borne by the population contributing participants. The confluence of these conditions often arises for trials conducted in developing countries~\cite{millum2013ethics}. Here, trial participants may lack access to conventional treatments, either for administerability or economic reasons. Hence, placebo participants would be no better off. As the drug being tested is usually designed to be more accessible, questions as to its efficacy exist, thereby justifying the need for a RCT. Finally, ensuring that the drug will eventually be used by the population responsible for contributing participants ensures that harms and benefits are equally distributed~\cite{resnik2008randomized}. 


Ethical concerns also arise in phase one trials for pharmaceuticals. These trials are the first conducted on human beings, and assess the safety of a drug. In the course of these trials, doctors will repeatedly escalate the dosage of a drug to determine the maximum tolerable dosage--the point at which the drug produces toxicity or intolerable symptoms~\cite{shamoo2006strategies}. Though phase one trials are usually involve patients suffering from terminal diseases, they are sometimes conducted on healthy volunteers. 

The classical lens through which individual participation in trials is analyzed--weighing the harm to an individual against the benefits that individual might recieve from participation--are not applicable for phase one trials involving healthy adults. As healthy phase one trial volunteers are unlikely to accrue significant benefits from participation, medical ethical experts have noted the importance of ensuring that risks are reasonably minimized~\cite{shamoo2006strategies}. 

To ensure this, \cite{shamoo2006strategies} proposes six recommendations that they argue will promote the welfare of participants. First, additional data should be collected on the short-term and long-term risks of participation for study participants. Second, strict inclusion/exclusion criteria should be developed for determining which participants are eligible to volunteer in phase one trials, so as to avoid reliance on vulnerable subjects. Third, structural precautions should be taken so as to avoid repeated participation from a single pool of volunteers, which would dramatically increase the risk of harm borne by this population. Fourth, researchers should develop mechanisms to track phase one participants over time. Fifth, participants should be gauranteed compensation for their involvement in the trials. Sixth–-and finally--participants should be allowed to engage in collective bargaining arrangements with trial sponsors. 


Though these principles offer guidance, they do leave significant room for interpretation. For instance, there is no universal consensus on when a placebo trial is methodologically justified. Neither is there a clear understanding of what harms could be considered as ``minor.'' Despite the lack of clarity here, we believe that the principles articulated can still be cogently extrapolated to the machine learning setting. We articulate these now.

\subsubsection{Intelligible principles for machine learning}. Extrapolating from the learnings of medical ethicists, we identify the following principles that can guide machine learning evaluation in settings where the harmfulness of an evaluation is balanced against its empirical value.

\underline{Harms and benefits should reciprocate}. First, the population at risk of suffering harm from the evaluation should also recover the benefits of the computational system being evaluated. This accords with an analagous principle in clinical trials, that the population from which a trial is drawn should also benefit from the development of the drug.  

In the context of the evaluation practices discused above, adherence to this principle would have several implications. Autonous vehicle practitioners should be mindful of the communities in vehicles are being evaluated in. As these types of vehicles are often expensive, evaluating such systems in lower-income communities--who are unlikely to afford them--would appear to raise the concerns discussed above. In the context of content moderation systems, practitioners should take steps to ensure that the countries from which those crowdworkers are drawn also benefit from similar moderation systems. Prior work has illustrated that this unfortunately isn't the case, and content moderation systems for underresourced languages are often extremely poor~\cite{culliford2021}.

\underline{Balancing against the status quo}. Second, harms inflicted through evaluation may be more permissible when the alternative process an individual would interact with is known to perform poorly or highly variably. This is analaogous to instances in clinical trials where no known treatment exists, or known treatments have highly variable performance. This inquiry is based on a counterfactual---if the evaluation practice wasn't conducted, would individuals have actually suffered less harm?

Suppose, for instance, that practitioners whish to deploy a computational system to replace a human decision making process, and that human decision makers have a high error rate in performing the task. This setting is quite common, and found in applications spanning law~\cite{}, content moderation~\cite{}, and medicine~\cite{}. Here, an individual would suffer no greater harm by being subject to a computational system than the baseline performance. Hence, the harm arising from live testing should be no worse than those ordinarily endured by users. 

Returning to our examples above, this principle suggests that when considering the ethicality of live testing with autonomous vehicles, the appropriate inquiry is whether autonomous vehicles--during testing--do not increase the danger to bystanders above and beyond what ordinary cars would. This is a highly context specific question–-autonomous vehicles may be more or less dangerous in different neighborhoods, depending on features of that neighborhood. 

Interestingly, this principle also elucidates a perspective on ``ethical hacking.'' Here, we analyze harms with respect to a larger population that may be harmed as a result of the practice. For instance, with regards to \cite{} (predicting sexual orientation from profile pictures), the vulnerable population would be LGBTQ individuals. The inquiry then, is whether the action of training such a model would increase the harm felt by this community. Again, this analysis will be highly specific to the context, and depend on the extent to which the work actually enables malevolent parties to weaponize such tools. 

\underline{Minimal or short-term harms are acceptable}. Finally, inflicting harm on users through evaluation may be permissible when that harm is short-lived or temporary, and individuals are not repeatedly subject to the harm. Here, we draw inspiration from the permissibility of placebo trials for less severe health conditions, and the recommendations on tracking phase one trial participants. The rationale is that when harms are minimal, they are outweighed by the benefits accrued from evaluation. 

This principle is most pertinent for privacy harms arising out of model debugging, as it suggests that privacy violations in the course of evaluation may be permissible where remediatory measures are taken to minimize the extent of the harm. There are a range of practices that engineers can deploy to achieve this. Numerous institutions--across education, healthcare and government--have developed specialized practices for handling sensitive data, and require involved practitioners to undergo specific trainings. Engineers can also ensure that datasets used for manual analysis are frequently refreshed, so that different individuals are studied each time (thereby avoiding the case where the privacy of a small subset of individuals is repeatedly jeopardized). Finally, practitioners can ensure that only the information necessary to evaluate the model is actually surfaced. 


\subsection{Slice identification and prioritization}
\textbf{What is the practice?} Machine learning researchers have found that in many settings, a model may provide high overall performance (i.e. \textit{global}) on a test set, but significantly struggle on certain subgroups of data (often termed as \textit{slices}~\cite{chen2019slice}). The discrepency between high global performance and low subgroup performance has been observed in a variety of domains. In facial recognition for instances, practitioners have noticed that models significantly underperform on racial minorities and women~\cite{buolamwini2018gender}. In healthcare settings, practitioners have observed that chest x-ray models underperform on patients with certain surgical implants~\cite{oakden2020hidden}. 

As a result, a common evaluation practice is to identify, define, and engineer slices into evaluation frameworks~\cite{goel2021robustness, re2019overton, eyuboglu2022domino}. Here, practitioners will independently evaluate the model on test samples representing a certain slice. In addition to analyzing aggregate performance over the entire test set, practitioners will look to slice performance to determine model quality. As an example: practitioners building a recognition system for an autonomous vehicle may define a slice consisting of images that contain cyclists at night~\cite{chen2019slice}. In practice, an evaluation system can contain numerous slices~\cite{}.

Measuring performance on a slice serves a variety of functions. First, practitioners may use slice performance to guide the model development process. If a model is underperforming on a particular slice, practitioners will take steps to improve performance on that slice. This could include: adding more training data from the distribution captured by the slice, adding more features, or modifying the architecture of the model. Second, practitioners use slice performance to determine when to deploy a model. If performance on a slice is too low, practitioners delay deployment until the problem can be alleviated.

\textbf{What are the ethical concerns raised by this practice?} The process of identifying slices and prioritizing performance on slices can raise several ethical challenges for practitioners. 

First, practitioners must determine \textit{which} slices are worth measuring. In defining a slice over a subset of samples, practitioners are explicitly prioritizing the performance of the model on those samples over performance on other samples. Hence, slice selection requires value judgements on the part of practitioners. 

In some settings, determining slices may be a straightforward task. Laws and regulations may, a priori, classify certain subgroups as ``protected'' and create legal penalties for failing to equalize performance across these subgroups. Other tasks may contain data which naturally divide into simpler groups that are amenable to measuring. For instance, in multi-class tasks--where a model must map each sample to one of $k$ classess--each class forms a natural slice.

In many cases however, the choice of which slices to measure is less clear. Practitioners may have access to rich demographic descriptions of individuals in a dataset. Different demographic attributes could be combined to capture the intersection of different identities. Consider, for example, a healthcare company developing a chest x-ray model to deploy at different hospitals. The company can construct slices using a plethora of information: patient age, race, gender, locale, or previous medical history. Slice descriptions could become arbitrarily complex (e.g., ``male patients with high cholestroal between the ages of 25 and 35 in the Pittsburgh area'').

Unfortunately, adding slices creates a tradeoff. While more slices provide practitioners with a better picture of performance--and avoid inequities where certain individuals are represented in a slice while others are not--slices can be source of expense. When a particular slice is insufficiently represented in test data, practitioners may be required to collect additional data. Given that slices often correspond to rarer types of samples, this can be expensive. In other cases, procuring data for slices can raise the privacy concerns discussed above~\cite{xiang2022being}.  

Second, precisely defining the inclusion/exclusion criteria for a slice can also raise challenges. Defining these criteria often requires building a rigid ontology over amorphous and evolving concepts like race and gender. Researchers in other disciplines have shown how such ontologies are prone to perpetuating harmful stereotypes, missing vulnerable populations, and providing inaccurate empirical assessments~\cite{}. Moreover, as defining slices in this manner may sometimes require access to unavailable attributes (e.g. race), practitioners may be forced to impute them, which raises its own set of concerns~\cite{}. 

Finally, practitioners must determine how to proceed when methodological interventions favor one slice over another. A significant body of work in machine learning has shown how it is often difficult to improve performance over all slices. Most methods either improve performance for the majority samples (at the cost of the minority samples), or vice-versa~\cite{}. Hence, practitioners are often forced to choose between different models, each of which tradeoff between slices in different ways.  

\textbf{Analagous domain: crash testing.}
Here, machine learning practitioners can take inspiration from the practices that automotive safety engineers use when evaluating the crashworthiness of vehicles. In car safety, the principle of crashworthiness dictates that a car's design should seek to minimize the injuries experienced by passengers during a crash. Crashworthiness arose in the latter half of the twenty-first centruy, in response to findings by researchers that many vehicle related fatalities could be attributed not to the initial impact between a vehicle and a foreign object, but to to a ``secondary impact'' between the vehicle's occupants and objects inside the vehicle. Today, the principle of crashworthiness extends beyond automobiles, and is present in many forms of transportation safety~\cite{}.

A key way in which engineers assess crashworthiness in automobiles is through \textit{crash tests}. The purpose of a crash test is to observe how a vehicle behaves during a crash. In the test, a vehicle is attached to a harness, which is capable of moving the vehicle in a particular direction at a particular speed. Engineers place an anthropomorphic test device (ATD)--colloquially known as a ``crash test dummy''--in a vehicle. ATDs are highly specialized devices containing an array of sensors capable of measuring the forces exerted upon the dummy. They are subject to extensive development, and can cost hundreds of thousands of dollars. After placing the ATD in the vehicle, engineers simulate a crash by moving the vehicle into a precisely placed obstacle at a fixed speed. The force sensors on the crash test dummy enable the engineers to measure the force that a human being--in the same crash as the test--would have experienced. From these measurements, engineers are able to assess safety, and hypothesize the extent of injuries that a human would have suffered. 

We find that several aspects of the crash test ecosystem are relevant for machine learning engineers. 

\begin{enumerate}
    \item Engineers determine, ex ante, test environments to evaluate vehicles in. The choice to restrict attention to these setups allows them to balance the cost of crash tests against the comprehensiveness of evaluations. 
    \item Engineers follow rigorous documentation procedures for ensuring that tests follow standardized setups. 
    \item Regulations specifying test performance orient engineers towards minimum performance thresholds for different groups.
    \item Crashworthiness continues to be assessed after deployment. In theory, this allows engineers to identify new tests to add. 
\end{enumerate}

We discuss these in more detail below. 

\underline{Ex Ante Tests}. A key challenge facing engineers is that the survivability of a crash is incredibly dependent on factors specific to that crash. Crashes can vary in terms of the location of the impact on the vehicle (e.g. frontal impact or side impact), the type of impacting object (e.g. concrete barrier vs deer), the speed at which the vehicle is travelling, and the relative wear and age of the vehicle itself. A person's chance of surviving a crash also depends on individual qualities: their physiology (e.g. height, weight, muscle mass, age), position in the vehicle, and prior health conditions. Even factors like their reaction time--which govern their ability to brace--can affect their likelihood of survival. In short: no two crashes are ever alike. 

Car safety experts have approached the challenge of crash variability by (1) identifying the most important factors affecting a crash, and (2) focusing on fixed settings for these factors. First, engineers restrict their attention to only certain types of crashes. Each type of crash is captured by a specific test (e.g. ``moderate overlap frontal test''), in which the direction of the car, it's speed, the impacting object, and the position of the impact are all fixed. There are only a fixed set of crash tests, and regulators/engineers rarely vary from these crash types during a vehicle evaluation. Though these tests are incomplete--there are certain real world crashes which occur but aren't accurately captured in these setups--these tests have been judged to capture the most common or critical crashes. Hence, they offer a cost-effective way to assess safety. Second, engineers restrict their attention to certain types of passenger physiologies. To do so, they design crash test dummies to mimic certain types of physiologies. As the distribution across human weights and heights is quite broad, they focus on several ``representative'' points for adults and children (e.g. median adult male) ~\cite{}. Crash test dummies are design to match the heights and weights of individuals at these distribution points. Tests are run with different sets of dummies.

Of course, this approach is not without its drawbacks. As researchers have noted in the context of automotive safety, much depends on whether the attributes and values chosen \textit{actually} reflect different aspects of the data population. Crash test dummies for instance, have been critiqued for failing to accurately capture female anatomy.


\underline{Rigorous Standardization of Tests}. Both crash tests and crash test dummies follow fixed specifications which are replicated across most vehicle tests. Though a wide array of different parties conduct tests~\cite{}, there is a strict adherence to common standards. Testers disclose both the dummy model that is used, and the exact parameters of the test. This includes details as specific as vehicle speed, the position of the barrier, the composition of the barrier, the configuration of the car battery, and others~\cite{ihsfrontaloverlap}.

This has several benefits. First, it enables external stakeholders to exactly reproduce the crash tests that automotive manufacturers or regulators perform. This can be helpful for auditing or enforcement purposes. Second, it enables stakeholders to better compare performance. If tests or dummies were continually changing, then drawing comparisons between different makes or models of cars would be empirically challenging, and confounded by the differences in test setups. 


\underline{Minimum performance thresholds}.


\textbf{Lessons for machine learning}


This setting bears several important similarities to the machine learning challenges with slices described above. First, both car engineers and machine learning practitioners face a ``long tail'' problem--because there are many rare events that impact performance, even reasonably large samples will fail to capture certain types of failure modes. Second, testing for these rare events can be costly. In the machine learning setting, practitioners must curate high quality datasets capturing rare subgroups. For automotive safety, crash tests are both time consuming and expensive. Hence, there is a limit to the extent to which testing for rare events can be performed. 




A similar approach could be applied in machine learning settings. Here, practitioners would identify, a priori, the most critical data attributes which they believe affect model performance. Then, they would fix a set of values a particular sample could take along these attributes, and use these attribute-value pairs to define potential slices. 



\underline{Slices definitions must be clear and capable of standardization}. 

In the context of machine learning, practitioners can apply this principle by developing rigorous inclusion/exclusion criteria for slices, and validating that samples belonging to a slice actually  



2. The criteria should be minimum performance. 
3. Slice definitions should be capable of clear definition. 
4. Slices should be updated. 

\subsection{Slice identification}

\textbf{Practice}
%Practitioners monitor performance for different slices. A slice consists of a strata of data points characterized by common attributes. 

%Examples of slices could include: 
%Individuals with a particular set of demographic characteristics (e.g. women, individuals from China, etc.)
%Samples which contain a particular features (e.g. chest X-rays with chest drains)

%As slices are considered to be critical, slice performance can drive evaluation. Practitioners need to ensure that a slice is sufficiently well represented in test data, which may involve specifically collecting data corresponding to a slice. A model’s deployment may be halted if slice performance is too low, and engineers will investigate remedies for improving performance. 

\neha{In slice identification, practitioners partition the population into different slices, and monitor the performance of the model within a slice. A slice consists of a strata of data points characterized by common attributes, oftentimes divided by demographic characteristics. Slices are considered to be critical, and slice performance drives evaluation, with the ability to halt wider model deployment if slice performance is low. An example of slice identification is medical device testing, in which pre-deployment evaluation studies will be performed on patients in one site, and this opens criticism in the medical community.

 This is similar to A/B testing, in that performance is evaluated on a subset of the population, but performance does not need to be compared across multiple subsets, and rather than a randomization of individuals across treated and control subsets, there is a deliberate placement of individuals into the slice receiving treatment.}

%A site will be accompanied by limited geographic or demographic diversity, which raises concerns regarding the overgeneralizability of research findings due to heterogeneity in health needs across genetically and sociologically disparate populations.}

\textbf{Decisions} \neha{Developers must determine which slices are most relevant for evaluating models on, as well as an appropriate size of a slice. This  likely requires collecting relevant demographic details of the individuals in the slice. They also decide the testing evaluation criteria within the slice. Overall, their aim is to guarantee deployment outside of the slice is likely to succeed based on performance within the slice.}

\textbf{Dimensions/tradeoffs}
\neha{
Slice identification lacks external validity. The use of data in a single slice of the population does not permit validation in heterogeneous populations. Slice identification in clinical trials is criticized for these problems. In \cite{wu2021medical}, the author review 130 FDA-approved medical devices and note that pre-deployment evaluation studies for 93 of these devices were not performed on patients in more than one site. They highlight the importance of multi-site assessment in clinical trials, because a small number of sites can indicate limited geographic or demographic diversity in the patients a device is tested on. 

% My personal casual interpretation of this problem is as follows: The testing of these devices in limited sites would indicate the assumption that given health outcome $H$ and class membership $B$, the clinical trials operate under the belief that believe that $\mathbb{E}(H|B=1)=\mathbb{E}(H|B=0)$. Although the clinical trials do not directly predict class membership $B$, or do any ``ethical hacking", they have created an assumption on that variable.

In \cite{national2022improving}, the authors highlight seven threats to healthcare if there is a lack of representation in clinical research, including overgeneralizability of research findings due to heterogeneity in health needs for genetic and socioeconomic reasons, downstream lack of access to effective interventions due to limitations in obtaining approval of treatments for all populations, potential compounding effects of health disparities, and increased costs. 

In \cite{clark2019increasing}, the authors identify critical barriers to inclusive clinical trials, and solutions that might allow dismantling these barriers. Some of the recommendations they offer include language that will emphasize available support and appreciate involvement. Additionally, they recommend making trials more patient centric and offering transportation. The FDA has offered recommendations for a standardized approach to collecting race and ethnicity data in clinical trials [cite], so that studies have knowledge of what slices have been studied.

Generalizing these recommendations outside of clinical trials or medical device evaluation; More broadly, developers can mitigate the tradeoff to the external validity by making slice participation more easy and having a wider representative slice. 

Slice identification also raises concerns of harmfulness or fairness, although the degree of this would be unique to the problem and whether there is in actuality a difference in outcomes for the population that was not part of testing compared to the population that was used. A likely advantage of slice identification is that it may be cost effective to avoid needing to test models on a wide range of individuals. [Didn't comment on internal validity/interpretability...]}

\subsection{Metric-outcome discordance}

\textbf{Practice}
Practitioners care about a particular outcome. However, that outcome is difficult to capture with the metrics available to practitioners in an evaluation setting. \neha{So, practitioners choose an alternative outcome of interest as a substitute and focus on using this as a metric for evaluation.

\paragraph{Case Study: Mullainathan and Obermeyer's Metric-Outcome Discordance Framework} In \cite{mullainathan2021inequity}, the authors illustrate the following scenario. Suppose researchers are interested in some risk score $S$, for each patient $i$, based on health $H$, in which $H_1$ is the health outcome if treated and $H_0$ is the health outcome if untreated, and the known variables are pre-treatemnt covariates $X$. Thus, the ideal risk score would be $S_i^*=\mathbb{E}(H_{1i}-H_{0i}|X_i)$ Due to obvious limitations, we instead focus on $S_i=\mathbb{E}(Y_{0i}|X_i)$, or the untreated health needs, and assume that those with the greatest untreated health needs have the greatest benefit of treatment. Since health needs are not easily quantifiable, we use costs, so $S=\mathbb{E}(C|X)$. However, costs is not random with respect to indicator $B$, of protected class, and $\mathbb{E}(C|H,B=1) < \mathbb{E}(C|H,B=0)$. This generalizes to the following issue: We are in general aiming to predict $Y$, can measure $Y^*$, but $Y=Y^*+\Delta$ where $\Delta$, an error, may be biased with respect to protected classes.
}

\textbf{Decisions}
\neha{Engineers must decide whether an alternative metric is necessary, due to hurdles in using the preferred metric. They then must decide which of a number of alternative metrics is most likely to meet their needs. The final decision is in how to create an evaluation model using the preferred alternative metric.
}

\textbf{Dimensions/tradeoffs}
\neha{
External validity is not possible because the preferred metric is not available in the population. 

Much like slice identification, interpretability, privacy, fairness, and harmfulness depend on the particular setting.
}


\subsection{Dataset releases}

\textbf{Practice}

\textbf{Decisions}

\textbf{Dimensions/tradeoffs}

\subsection{Error analysis and privacy}
Error analysis–-the process of examining model misclassifications to better understand the source and origin of the errors–-is considered to be an integral part of the evaluation pipeline~\cite{nushi2018towards}. By actually examining where the model goes wrong, practitioners can attribute errors to failures in the design and  construction of models, enabling them to take better remedial decisions. In the past several years, a wealth of literature has offered tools for helping practitioners with this endeavor~\cite{eyuboglu2022domino, d2022spotlight, zhu2022gsclip}.

Yet, the process of error analysis raises a variety of privacy concerns. First, error analysis requires practitioners to directly examine data points corresponding to individuals. Depending on the task and type of data collected, the examining practitioner may be able to infer the identity of or sensitive information about the individual associated with the data point. Prior work on deidentification has illustrated that individuals in supposedly ``anonymized'' datasets can be easily identified using only a few features~\cite{narayanan2006break, anderson2009, de2013unique}. Moreover, large technology companies have already fired employees for abusing data privileges, and accessing private information about different users~\cite{jackson2021, cox2019,cox2021}.   

Second, error analysis may require collecting additional sensitive information about the individual. 
Thus, error analysis can present practitioners with a value tradeoff. On the one hand, pursuing more detailed forms of error analysis could enable engineers to uncover model failures, or identify corrective steps. However, error analysis could also jeopardize the privacy of individuals being studied. The choice to pursue different types of error analysis--including what additional data to collect--therefore reflects a value balancing on the part of engineers.


==> old/old_05.tex <==
\subsubsection{Phase one trials}
Phase one clinical trials are the first evaluative experiments conducted on human beings, in the process of testing drugs meant for humans, and play a key role in helping researchers assess the safety of a drug. In the course of these trials, doctors will repeatedly escalate the dosage of a drug to determine the maximum tolerable dosage--the point at which the drug produces toxicity or intolerable symptoms~\cite{shamoo2006strategies}. Though phase one trials are usually involve patients suffering from terminal diseases, they are sometimes conducted on healthy volunteers. 

The classical lens through which individual participation in trials is analyzed--weighing the harm to an individual against the benefits that individual might recieve from participation--are not applicable for phase one trials involving healthy adults. As healthy phase one trial volunteers are unlikely to accrue significant benefits from participation, medical ethical experts have noted the importance of ensuring that risks are reasonably minimized~\cite{shamoo2006strategies}. 

To ensure this, \cite{shamoo2006strategies} proposes six recommendations that they argue will promote the welfare of participants. First, additional data should be collected on the short-term and long-term risks of participation for study participants. Second, strict inclusion/exclusion criteria should be developed for determining which participants are eligible to volunteer in phase one trials, so as to avoid reliance on vulnerable subjects. Third, structural precautions should be taken so as to avoid repeated participation from a single pool of volunteers, which would dramatically increase the risk of harm borne by this population. Fourth, researchers should develop mechanisms to track phase one participants over time. Fifth, participants should be gauranteed compensation for their involvement in the trials. Sixth–-and finally--participants should be allowed to engage in collective bargaining arrangements with trial sponsors.
TODO: Discuss the IRB more here?


\section{OLD WRITING–DISREGARD EVERYTHING BELOW}

Live testing of autonomous vehicles provides valuable information for evaluating performance. Driving is a long tailed distribution, containing many rare events which could confuse an autonomous navigation system~\cite{ackerman2017}. Real world roads contain phenomenon that are difficult to simulate in synthetic environments: inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. By testing on live roads–in a variety of diverse environments–engineers can study when systems return manual control to the human driver~\cite{banerjee2018}. Studying these interventions allows them to identify failures in perception or control systems~\cite{wang2020safety}. They can also interview passengers of the car, allowing them to learn more about the smoothness of the ride and identify instances of erratic behavior~\cite{donfro2018}. None of this could be measured in a laboratory. 

\subsection{A/B testing}
% Split out live testing -- you have something you think is good, but you need to put it out in the world in order to get better feedback  
% Split out A/B testing -- are we doing control?


In A/B testing, engineers deploy an experimental model on a subset of users, and collect metrics corresponding to the model's performance on those users~\cite{seldon2021, bright2021, luigi2020, amatriain2019,shankar2022}. Metrics could directly measure model performance (e.g., accuracy of a prediction), or a downstream impact of performance (e.g. the time users spend on a platform). In deciding whether to deploy a model, practitioners will compare metrics computed for the experimental model against metrics of the status-quo on a control group of users. 

A/B testing is ubiquitous and controversial. Users of most internet services are often included as part of experiments that measure the impact of minor changes to models. A significant portion of evaluation for self-driving vehicles is achieved through A/B testing with actual vehicles on public roads. In some cases, companies have even published the results of A/B tests, revealing how system modifications can drive patterns in user behavior.

A/B testing presents the following advantages: 
\begin{itemize}
    \item Because practitioners can run a development model on live data, concerns associated with static datasets (e.g. distribution shift, rare events/long tails, out-of-distribution data) are less salient (\textbf{external validity}). 
    \item Because practitioners can observe how users respond to model outputs, A/B testing allows practitioners to evaluate models deployed in complex, interactive systems (\textbf{external validity}). In an application like autonomous driving, practitioners can measure the number of times a user grabs the steering wheel, or performs a similar corrective action. Performing such evaluations without the aide of A/B testing may require building complex simulations (\textbf{cost}), which themselves would make simplifying (and sometimes incorrect) assumptions (\textbf{external validity}).
    \item Because the longer-term effects of models can be observed in system behavior, practitioners can actually measure the metric of interest (\textbf{interpretability}). For instance, in a task like content moderation (where labels can often be subject to disagreement), practitioners can actually measure whether certain models are correlated with less or more time on the platform, which itself may measure user satisfaction. 
\end{itemize}
However, A/B testing presents the following concerns:
\begin{itemize}
    \item As practitioners are evaluating developmental models still under development, users exposed to the model may be subject to an increased risk of model mispredictions. Depending on the application, this can expose users to various types of physical \textbf{harm}. Autonomous vehicles operating in testing programs have crashed during testing, resulting in tragic injuries and loss of life to other road occupants~\cite{associatedpress2022, kao2022}. These sorts of failures have produced significant controversy, leading some to call for more stringent regulation regarding the ability for autonomous vehicle companies to test on public roads. 
    \item When practitioners have strong reason to believe that a particular model is superior (as was the case in LinkedIn's tests~\cite{}), the denial of the superior model to users in the control group deprives them of a benefit, thereby inflicting \textbf{harm} on them. \jessica{is there lit on the philosophy behind why this is wrong, ie why should we assume that as engineers we owe the best experience we know to everyone?}
    \item Users often lack the ability to consent to participation in an A/B test. As policymakers increasingly recognize a ``right'' for users to know whether they are interacting with algorithms, A/B testing with machine learning models may also inflict dignatory \textbf{harm}~\cite{engler2020}.
    \item Finally, A/B tests may disproportionately result in harm to certain vulnerable populations, especially when that population holds valuable data~\cite{fussell2019google}. In these instances, A/B tests may diminish \textbf{fairness}.
\end{itemize}



%One prominent illustration of ``live user testing'' occurs with self-driving vehicles. Through specialized testing programs, California permits autonomous vehicle manufacturers to evaluate autonomous driving systems on public roads~\cite{dmvpermitholders}. The program is widely used. For instance, between December 2020 and November 2021, autonomous vehicles “test drove” nearly five million miles on public roads in California~\cite{bellan2022}. Live testing of autonomous vehicles provides valuable information for evaluating performance. Driving is a long tailed distribution, containing many rare events which could confuse an autonomous navigation system~\cite{ackerman2017}. Real world roads contain phenomenon that are difficult to simulate in synthetic environments: inclement weather, variable road conditions, aggressive or erratic behavior from other cars, and foreign objects~\cite{kalra2016}. By testing on live roads–in a variety of diverse environments–engineers can study when systems return manual control to the human driver~\cite{banerjee2018}. Studying these interventions allows them to identify failures in perception or control systems~\cite{wang2020safety}. They can also interview passengers of the car, allowing them to learn more about the smoothness of the ride and identify instances of erratic behavior~\cite{donfro2018}. None of this could be measured in a laboratory. 





%\jessica{make clearer - live testing is a way of getting back validity, but where you're now introducing potential harm} 
 

%Additionally, individuals in a live test may be deprived of access to a superior experience. Suppose engineers are seeking to evaluate a model which they belive more accurately performs a task for users. By choosing a subset of users to operate in the control group, the engineers are deliberately depriving them of the opportunity to recieve what they believe is a superior experience. 

%Thus, the decision to live test a model forces engineers to tradeoff between the correctness of an evaluation and the harm it may inflict. If engineers valued the correctness of an evaluation, then the ancilliary harms to users though live testing would be an acceptable cost. Similarily, choosing not to perform a live test would indicate that engineers valued the minimization of harm over the accumulation of additional evaluation information.

\subsection{Manual annotation for content moderation}

Machine learning is often employed in content moderation pipelines, where models to classify content that violates a platform's terms of service or community guidelines. Moderated content can vary significantly, but often corresponds to profane and explicit content, depicting sexual activities, violence, or bigoted ideas~\cite{chen2014}. The volume of social media content means that responsive moderation on platforms can often only occur through the use of automated tools~\cite{darbinyan2022}. Evaluating these models requires building sizeable and high quality evaluation datasets, for which human annotators must manually review and label harmful content. We discuss this practice along our aforementioned dimensions. 

Extensive reliance on human labeling for content moderation evaluation datasets presents the following advantages: 
\begin{itemize}
    \item Larger test sets offer increased statistical power, enabling more certainty in comparisons or evaluations (\textbf{internal validity}.~\cite{card2020little}. Measured differences in metrics between models are more likely to reflect actual quality differences.
    \item Larger test sets also improve the extent to which measured evaluations estimate deployment performance (\textbf{external validity}), and they are more likely to capture different subparts of the data distribution~\cite{harrison2021, roy2022does}. 
    \item For tasks like content moderation--where researchers have observed existing models often disproportionately flag content associated with minority identities~\cite{sapetal2019risk}--larger test sets enable practitioners to better detect evidence of disparate performance (\textbf{fairness}). Large test sets enable engineers to conduct disaggregated evaluations~\cite{barocas2021designing}, while still ensuring that each sub-evaluation is statistically powered.
    \item Researchers have shown that human annotations for content moderation are often subject to extensive disagreement based on annotator background~\cite{gordon2021disagreement}. Hence, acquiring more annotations per sample enables practitioners to better avoid label errors (\textbf{internal validity}). Ensuring annotations are provided by individuals from diverse backgrounds additional prevents biases from seeping into dataset-wide annotations (\textbf{fairness}).
\end{itemize}

However, extensive reliance on human annotations presents the following disadvantages:
\begin{itemize}
    \item Annotating online content can be traumatic, putting annotators at risk of physical and pyschological illness (\textbf{harmfulness}). The content that moderators see is often considered to be highly distressing, depicting graphic forms of violence and other disturbing acts~\cite{chen2014,hatmaker2022,bbc2020, newton2019}. Various studies have shown how individuals responsible for annotating these materials often suffer longer term traumatic stress disorders and experience burnout~\cite{steiger2021psychological}.
    \item Annotators are often drawn from non-Western countries, where they often work in borderline exploitative conditions for little pay~\cite{hao2022venezuela}. Prior work has noted the structural harms arising out of data labeling employment practices, including poor wages and working conditions~\cite{hao2022venezuela, hao2019}. This has given rise to concerns that–for harmful tasks like content moderation-certain demographic groups disproportionately suffer the longer term harms (\textbf{fairness}). 
\end{itemize}



%Constructing large evaluation test sets requires significant manual labor to curate and annotate data. Annotation is a delicate process, and mistakes can contaminate test sets and lead to incorrect metrics~\cite{paullada2021data}. For instance, researchers have identified mislabelled samples in popular benchmarks~\cite{northcutt2021pervasive} and underspecified label schema~\cite{tsipras2020imagenet}. As a result, machine learning practitioners spend extraordinary resources in dataset development, with a suite of technology companies specializing in offering data labelling services~\cite{kahn2020}. 


%\jessica{so, here we've prioritized validity over cost, but we've introduced harms. The image I get of all this is that we have these pairs of values, where we put the point closer to one end than the other (we prioritize validity over cost) but then because these values tend to be interrelated, everytime we adjust balance between some pair of values we may introduce imbalance with some other value (eg by moving toward validity and away from cost, we've also moved away toward prioritizing lack of harmfulness. }

%However, the reliance on human laborers to construct label content for moderation has raised significant concerns.  Moreover, 

%The choice to have human crowdworkers label evaluation datasets for tasks like content moderation requires balancing different values. On the one hand, constructing larger evaluation datasets, by hand, will provide a more accurate assessment of model performance. On the other hand, the process of constructing these datasets can significantly harm the workers employed in the task. These considerations go beyond merely the choice to construct an evaluation dataset, and implicate other questions. For instance, larger datasets--or datasets with multiple annotations per sample--improve the correctness of an evaluation, but also increase the net harm inflicted.

%\jessica{so, how do we solve this? it seems like the answer has to be more explicit cost benefit analysis. So is part of our argument that currently people are not doing these analyses, and its because they are not thinking about how the dimensions relate? I think we need to be explicit about this kind of motivation}

\subsection{Error analysis and privacy}
\jessica{should privacy be its on bullet? would be nice to have a good motivation for why fairness is separate and privacy is grouped with harms - is it because harms refers to all individual stuff and fairness can only be defined in aggregate?}
Error analysis–-the process of examining model misclassifications to better understand the source and origin of the errors–-is considered to be an integral part of the evaluation pipeline~\cite{nushi2018towards}. By actually examining where the model goes wrong, practitioners can attribute errors to failures in the design and  construction of models, enabling them to take better remedial decisions. In the past several years, a wealth of literature has offered tools for helping practitioners with this endeavor~\cite{eyuboglu2022domino, d2022spotlight, zhu2022gsclip}.

Yet, the process of error analysis raises a variety of privacy concerns. First, error analysis requires practitioners to directly examine data points corresponding to individuals. Depending on the task and type of data collected, the examining practitioner may be able to infer the identity of or sensitive information about the individual associated with the data point. Prior work on deidentification has illustrated that individuals in supposedly ``anonymized'' datasets can be easily identified using only a few features~\cite{narayanan2006break, anderson2009, de2013unique}. Moreover, large technology companies have already fired employees for abusing data privileges, and accessing private information about different users~\cite{jackson2021, cox2019,cox2021}.   

Second, error analysis may require collecting additional sensitive information about the individual. Over the last several years, practitioners have improved their understanding of how machine learning models may produce good overall error, while significantly underperforming on certain subgroups of samples~\cite{buolamwini2018gender,chen2019slice, oakden2020hidden}. The presence of these performance differentials have raised significant concerns with regards to fairness, and significant attention has been devoted to identifying and rectifying such differences. In practice, identifying such subgroup disparities requires subgroup identification information (e.g., gender, race, or nationality) for individuals in evaluation data~\cite{andrus2021we}. Collection of this information raises significant privacy concerns, and in many cases, violate government and industry data use policies~\cite{andrus2022demographic, xiang2022being}. For instance, subgroup identification is often the source of discrimination-–individuals may fear that this information may be used in other, more insidious ways. While ostensibly to prevent disparate effects, the collection of racial identification data may thus be seen as a precursor to enabling discrimination~\cite{andrus2022demographic, cabanas2020does}.

Thus, error analysis can present practitioners with a value tradeoff. On the one hand, pursuing more detailed forms of error analysis could enable engineers to uncover model failures, or identify corrective steps. However, error analysis could also jeopardize the privacy of individuals being studied. The choice to pursue different types of error analysis--including what additional data to collect--therefore reflects a value balancing on the part of engineers.

\subsection{Task hacking}
Sometimes, researchers attempt to evaluate the properties of a dataset, by training a model to predict a secondary task from the data. A frequent illustration of this is found in work on dataset bias, where researchers evaluate the extent to which certain features encode information about race or gender by having a model learn to predict race/gender from those features~\cite{gichoya2022ai}. We refer to this practice as ``task hacking.''

Task hacking has important benefits. First, it allows practitioners to understand properties of their datasets. Given the opacity of modern machine learning systems-–and the difficulty in specifying which types of correlations should be learned from data-–understanding the correlations that exist can be an important indicator of the risk of bias. For instance, if practitioners observe that a feature facially unrelated to gender (e.g., an applicant’s college major) actually encodes strong information about the applicant, then they may elect to remove that feature from their dataset. Second, task hacking allows researchers and practitioners to understand the downstream risks of a particular dataset. When a dataset enables accurate prediction of a sensitive characteristic, public releases of those datasets should be limited. In the context of privacy, such forms of ethical hacking can better inform when model releases should be accompanied by datasets. 

However, prior work akin to task hacking has also inspired controversy. Recent studies have attempted to predict a range of attributes (e.g. sexual orientation, criminality, etc) from photos of faces~\cite{paullada2021data}. These studies have been critiqued for presupposing that such predictions are possible, or reflective of underlying casual mechanisms. Other researchers have pointed out that much of the performance can be explained by correlated proxies present in the data~\cite{aguera2018}.

Additionally, task hacking raises questions about the proliferation of harmful machine learning methodologies. Studies have shown, for instance, that protein folding models–-originally designed to guide drug exploration-–can be engineered to design toxic compounds and bioweapons~\cite{urbina2022dual}. The proliferation of computational power and data means that the barrier for entry for developing such models is alarmingly low. Though the publication of such research is intended to raise awareness, it could inadvertently empower malicious actors to develop these tools. 

Thus, task hacking also implicates a value balancing question. On the one hand, task hacking makes practitioners more attuned to the dangers that a particular dataset may carry, both with regards to the information that features encode, and the types of predictions it may enable. On the other hand, the act of training models to perform these tasks threatens to legitimize them, or more easily enable malicious parties to weaponize them. 
\jessica{how does this relate to framework?}

\subsection{Slice identification}

Machine learning researchers have found that in many settings, a model may provide high overall performance (i.e. \textit{global}) on a test set, but significantly struggle on certain subgroups of data (often termed as \textit{slices})~\cite{blodgett2016demographic, chen2019slice,oakden2020hidden, hashimoto2018fairness}. The discrepency between high global performance and low subgroup performance has been observed in a variety of domains. In facial recognition for instances, practitioners have noticed that models significantly underperform on racial minorities and women~\cite{buolamwini2018gender}. In healthcare settings, practitioners have observed that chest x-ray models underperform on patients with certain surgical implants~\cite{oakden2020hidden}. 

As a result, a common evaluation practice is to identify, define, and engineer slices into evaluation frameworks~\cite{goel2021robustness, re2019overton, eyuboglu2022domino}. Here, practitioners will independently evaluate the model on test samples representing a certain slice. In addition to analyzing aggregate performance over the entire test set, practitioners will look to slice performance to determine model quality. As an example: practitioners building a recognition system for an autonomous vehicle may define a slice consisting of images that contain cyclists at night~\cite{chen2019slice}. In practice, an evaluation system can contain numerous slices~\cite{re2019overton}.

Measuring performance on a slice serves a variety of functions. First, practitioners may use slice performance to guide the model development process. If a model is underperforming on a particular slice, practitioners will take steps to improve performance on that slice. This could include: adding more training data from the distribution captured by the slice, adding more features, or modifying the architecture of the model. Second, practitioners use slice performance to determine when to deploy a model. If performance on a slice is too low, practitioners delay deployment until the problem can be alleviated.

However, determining \textit{which} slices are worth measuring can be a challenging endeavor. In defining a slice over a subset of samples, practitioners are explicitly prioritizing the performance of the model on those samples over performance on other samples. Hence, slice selection requires value judgements on the part of practitioners. 

In some settings, determining slices may be a straightforward task. Laws and regulations may, a priori, classify certain subgroups as ``protected'' and create legal penalties for failing to equalize performance across these subgroups. Other tasks may contain data which naturally divide into simpler groups that are amenable to measuring. For instance, in multi-class tasks--where a model must map each sample to one of $k$ classess--each class forms a natural slice.

In many cases however, the choice of which slices to measure is less clear. Practitioners may have access to rich demographic descriptions of individuals in a dataset. Different demographic attributes could be combined to capture the intersection of different identities. Consider, for example, a healthcare company developing a chest x-ray model to deploy at different hospitals. The company can construct slices using a plethora of information: patient age, race, gender, locale, or previous medical history. Slice descriptions could become arbitrarily complex (e.g., ``male patients with high cholestroal between the ages of 25 and 35 in the Pittsburgh area'').

Adding slices can come at a cost. Practitioners must ensure that slices contain sufficient samples to yield statistically powered measurements. For slices corresponding to rare subgroups, gathering sufficient data can thus be expensive or difficult. As practitioners add slices moreover, the significance of existing slices are diluted. 

Thus, the process of formalizing slices presents practitioners with an ethical tradeoff. On the one hand, creating a slice enables practitioners to better understand the performance of the model, and detect when a particular subgroup experiences lower-than-average performance. Yet, the choice to define some slices–-and not others--places different subgroups on different footings, implicitly valuing certain populations over others.  
\jessica{how does this relate to framework?}

\subsection{Slice prioritization}

A challenge that follows from slice identification is \textit{slice prioritization}. When performance on a slice is low, practitioners may pursue a range of strategies to improve metrics. This can include collecting additional data~\cite{vokinger2021mitigating} or altering training strategies~\cite{sagawa2019distributionally, liu2021just}. By applying such interventions, practitioners can often improve performance for minority subgroups present in the data. 

Unfortunately, researchers have observed that such interventions often \textit{decrease} performance for other subgroups~\cite{liu2021just, zhang2022correct, sohoni2020no}. In practice, algorithmic or dataset modifications which improve metrics for minority subgroups reduce performance for majority subgroups. Many possible explanations exist for this phenomenon. For instance, models have limited representational capacity. When different subgroups implicate different features, learning better representations for one subgroup may require sacrificing the model's ability to capture meaningful representations for other subgroups~\cite{chen2019slice}. 

This phenomenon forces practitioners to negotiate an ethical tradeoff when selecting which model to deploy. As no model maximizes performance over all subgroups, any choice of model will require sacrificing performance on some subgroup. Moreover, there is no clear principle to guide this decision. A utilitarian perspective--which would seek to maximize performance for as many people as possible--would prefer interventions which boost performance for larger subgroups at the cost of smaller subgroups. In contrast, perspectives which favor formal protections for minorities--often reflected in our social and political structures--would accept reductions to majority group performance if accompanied by improvements to minority group performance.


\subsection{Label disagreements}

Machine learning models are sometimes deployed for tasks where ``ground-truth'' can be highly subjective. Evaluation in these settings can be challenging, as the labels associated with a test dataset may be subject to disagreements~\cite{paullada2021data}. For example: 

\begin{itemize}
    \item For content moderation, researchers have observed that there is significant disagreement between different individuals as to whether a piece of content contains harmful or toxic messages~\cite{van2018challenges}. Unsuprisingly, disagreements often reflect demographic differences, as individuals from different communities frequently express different reactions to certain types of speech~\cite{haimson2021disproportionate}. 
    \item In medical settings, doctors sometimes disagree on diagnoses, or how to classify a particular condition~\cite{schaekermann2019understanding, nadis2022}.
    \item In e-discovery--where law firms use machine learning to identify documents pertaining to the issues litigated in a particular lawsuit--lawyers often disagree as to which documents are actually relevant~\cite{guha2022vulnerabilities}.
\end{itemize}

Evaluation under label uncertainty forces practitioners to tradeoff between different values. For instance, practitioners may elect to acquire multiple annotations per sample, and use the most common annotation as ground truth~\cite{gordon2021disagreement}. Here, practitioners sacrifice breadth for depth, as ensuring each sample has multiple annotations means that fewer samples can be annotated under a fixed budget~\cite{chen2022clean}. Additionally, prior work has highlighted how majority voting over annotations disregards minority voices, who may be more impacted by the predictions of the model~\cite{gordon2021disagreement}. In content mdoeration for instance, racial and ethnic minorities are more likely to be the target of toxic content online. Hence, disregarding their voices under a majority vote scheme may be yield suboptimal model performance. Alternatively, practitioners may elect to disregard samples where annotator disagreement meets a certain threshold. This however, alters the distribution of the test set. When disagreements indicate the complexity of a sample, evaluation sets become easier, thereby inflating metrics. 
 

\subsection{Metric-outcome discordance}

% TODO

\section{Analagous practices}
\jessica{how does this section relate to paper contributions? Need to spell it out. E.g., we use analogous evaluation practices from outside ML in order to identify guidelines that ML researchers can adopt to solve address ethical dimensions of evaluation}

The ethical tradeoffs implicated in the practices above are not unique to machine learning pipelines. The tensions they present--between competing values like harm avoidance and accuracy--pervade evaluation practices that are common in other highly technical fields. Studying similar practices in other fields can offer several benefits to machine learning engineers. 

First, these fields have developed ethical, regulatory and administrative frameworks that help them balance the value tradeoffs which arise in different evaluation practices. Many of these frameworks offer principles which are directly applicable to machine learning development. 

Second, practitioners in these disciplines have deployed actual systems at scale. Hence, they are more battle-tested. 

Third, ML can learn from their failures. 

\subsection{Phase one trials}
Phase one clinical trials are the first evaluative experiments conducted on human beings \jessica{in the process of testing drugs meant for humans}, and play a key role in helping researchers assess the safety of a drug. In the course of these trials, doctors will repeatedly escalate the dosage of a drug to determine the maximum tolerable dosage--the point at which the drug produces toxicity or intolerable symptoms~\cite{shamoo2006strategies}. Though phase one trials are usually involve patients suffering from terminal diseases, they are sometimes conducted on healthy volunteers. 

The classical lens through which individual participation in trials is analyzed--weighing the harm to an individual against the benefits that individual might recieve from participation--are not applicable for phase one trials involving healthy adults. As healthy phase one trial volunteers are unlikely to accrue significant benefits from participation, medical ethical experts have noted the importance of ensuring that risks are reasonably minimized~\cite{shamoo2006strategies}. 

To ensure this, \cite{shamoo2006strategies} proposes six recommendations that they argue will promote the welfare of participants. First, additional data should be collected on the short-term and long-term risks of participation for study participants. Second, strict inclusion/exclusion criteria should be developed for determining which participants are eligible to volunteer in phase one trials, so as to avoid reliance on vulnerable subjects. Third, structural precautions should be taken so as to avoid repeated participation from a single pool of volunteers, which would dramatically increase the risk of harm borne by this population. Fourth, researchers should develop mechanisms to track phase one participants over time. Fifth, participants should be gauranteed compensation for their involvement in the trials. Sixth–-and finally--participants should be allowed to engage in collective bargaining arrangements with trial sponsors.

\subsection{Placebo clinical trials}
In addition, we can draw a comparison to placebo control trials, which implicate similar concerns. First, placebo controlled trials would appear to violate the professional obligations of doctors to provide the optimal medical care to patients~\cite{miller2002makes}. Second, when other known beneficial treatments exist--denying patients access to those treatments for the sake of measuring the efficacy of the novel treatment against a placebo is both clinically and scientifically questionable~\cite{miller2002makes}.

However, the ethical concerns emerging from placebo controlled trials should be balanced against their prospective advantages. Placebo trials are widely considered to be the most rigorous test of treatment efficacy~\cite{miller2002makes}. They generally require fewer participants that active-controlled trials, thereby making them easier and cheaper to conduct~\cite{miller2002makes}. Even where existing treatments exist, placebo trials offer new and valuable forms of information~\cite{miller2002makes}. 

Thus, medical practitioners have come to identify several principles that guide determinations as to when placebo trials may be appropriate~\cite{millum2013ethics}. First, placebo trials are permissible when no proven treatment exists for the disorder being studied (e.g., for Alzheimer's dementia). This includes the setting where a treatment may exist, but its efficacy cannot be extrapolated to the population of interest. Here, the absence of a proven treatment means that placebo participants are therefore no worse off than if they weren't participating in the trial. 

Second, placebo trials are permissible when preventing patients from acessing a known alternative treatment would expose them to at most ``temporary discomfort or delay in relief of symptoms.'' This is common when the medical disorder being studied is ``minor,'' like common headaches or male pattern baldness~\cite{miller2002makes, millum2013ethics}. In these settings, placebo trials are considered ethical as the harms are often minute enough to justify the investigative value of these trials. 

Third, placebo trials are justified when existing treatments prove to be highly variable. This is commonly the case for conditions like depression, where established drugs can sometimes fail to outperform placebos~\cite{millum2013ethics}. Here, comparing a new drug to an existing drug can diminish the internal validity of a study~\cite{miller2002makes}. If both the efficacy of both drugs are indistinguishable, then it could be the case that either both drugs are effective, or neither are. Here, placebo trials are ethical as the lack of medical confidence in superiority of existing treatments over a placebo diminish the harm inflicted on placebo participants.

Finally, placebo trials are permitted when there existing compelling methodological reasons for their use, participants are not deprived of treatments they would otherwise have acess to, and the benefits of the trial will be borne by the population contributing participants. The confluence of these conditions often arises for trials conducted in developing countries~\cite{millum2013ethics}. Here, trial participants may lack access to conventional treatments, either for administerability or economic reasons. Hence, placebo participants would be no better off. As the drug being tested is usually designed to be more accessible, questions as to its efficacy exist, thereby justifying the need for a RCT. Finally, ensuring that the drug will eventually be used by the population responsible for contributing participants ensures that harms and benefits are equally distributed~\cite{resnik2008randomized}. 

\subsection{NASS}

% TODO: talk about ways in which CDS has been used: https://crashstats.nhtsa.dot.gov/Api/Public/ViewPublication/812128 (page 13)
Here, we draw a comparison to the National Automotive Sampling System (NASS) that is operated by the National Highway Traffic Safety Administration (NHTSA)~\cite{nassbrochure}. NASS was established in 1979 as part of an effort to reduce crashes, injuries, and fatalities involving motor vehicles. The data collected as part of NASS enables NHTSA to identify existing and potential problems in highway safety, assess the performance of vehicle safety systems, learn more about the nature of crash injuries, and assess the influence of social factors on vehicle safety~\cite{nassbrochure}. NASS consists of two subsystems: the Crashworthiness Data System (CDS) and the General Estimates System (GES). We focus on CDS.

CDS contains detailed data on a representative random sample of thousands of minor, serious, and fatal crashes~\cite{cdsoverview}. CDS is supported by 24 field research teams, referred to as Primary Sampling Units (PSU's). Collectively, PSU's study approximately five thousand crashes every year (spanning passenger cars, pickup trucks, and vans)~\cite{nassbrochure}. As performing investigations on all crashes would be prohibitively expensive (and logistically impossible), CDS investigations only occur for a sample of crashes. Special care is taken in the design of the sampling process~\cite{cdsmanual}. Only crashes which meet certain minimum criteria (e.g. involves a harmful event) are eligible, and the sampling probabilities are skewed to favor more recent vehicle models and more serious injuries. 

Trained crash researchers will visit crash sites, collecting information regarding the crash. This can encompass: photographs of damaged vechiles, skid marks, fluid spills, broken glass, bent guardrails, and other evidence of crash damages. Investigators will also observe the interior of vehicles, in order to document locations struck by occupants. When possible, investigators will follow up with crash victims and additionally collect medical records. Critically, CDS interviews are conducted with ``discretion and confidentiality''~\cite{cdsoverview}. Personal information pertaining to the crash--names, addresses, license and registration numbers, and even sometimes locations--are not included in publicly released NASS data.

Data is collected in adherence to strict standards. NHTSA rules specifically dictate what information investigators must collect, and the precise way in which different types of information must be coded~\cite{cdsmanual}. For instance, investigators will classify the collision as one of 6 types. This helps ensure standardization across different PSUs, and enables more sound post-hoc analysis of crashes. Additionally, investigations undergo a quality control process. Each PSU works in conjunction with one of two NASS Zone Centers. Each Zone Center is staffed with the most experienced crash researchers, and are responsible for coordinating and supervising the activities of different PSU's. Prior to a crash investigation being deemed complete, the Zone Center must review the PSU's findings for quality control standards. In practice, this can result in several back-and-forths until the report has met standards.  


\subsection{Crash test construction}

Here, we draw a parallel to the tests that regulators and automotive engineers use to evaluate the ``crashworthiness'' of different vehicles. In the late 1960s, American courts began to find automotive manufacturers liable for passenger injuries where elements of the car served to exacerbate the harms experienced by passengers~\cite{choi2019crashworthy}. Though these accidents were often caused by human error, courts argued that the statistically inevitable nature of car accidents meant that manufacturers carried a duty to minimize the consequences of such accidents. This caselaw--dubbed the ``crashworthy doctrine''--would be some accounts inspire a wholesale change in the way manufacturers approached safety, be responsible for technical improvements ranging from seatbelts to padded interiors, and spur a tremendous drop in traffic deaths~\cite{choi2019crashworthy}. 

Crashworthiness is evaluated through crash tests. In a crash test, researchers place a crash dummy (formally called an anthropomorphic testing device, or ``ATD'') is placed in a vehicle, and remotely drive the vehicle into a barrier in order to simulate a crash~\cite{engber2006}. Sensor readings from the vehicle and ATD–along with camera footage of the crash–are then studied to determine the crashworthiness of the vehicle. 

A challenge in performing evaluations of crashworthiness is that no two crashes are alike. For instance, researchers have shown that the survivability of a crash is dependent on a range of crash specific factors, including but not limited to: weather conditions~\cite{saha2016adverse}, road conditions~\cite{fitzpatrick2014influence}, the location of the impact on the vehicle (e.g. frontal impact or side impact)~\cite{keall2018relative}, the type of impacting object (e.g. concrete barrier vs deer)~\cite{iihsobjects}, the speed at which the vehicle is travelling~\cite{iihsnewtests}, the relative wear of the vehicle itself~\cite{national2013vehicle}, the individual physiologies of the passengers~\cite{ishii2020factors}, and the actions of first responders~\cite{calland2005extrication}. 

Moreover, assessing the crashworthiness of a vehicle for every possible type of crash is infeasible. Individual tests can be extremely expensive. ATDs are sophisticated and highly engineered devices, costing between \$100,000 and \$1 million dollars, containing as many as 30,000 distinct parts, and have a limited shelf life~\cite{automology2021, hall2015, ferris2022, reilly2021}. As cars are typically destroyed after a test, each test requires a brand new vehicle. For cars earlier in the manufacturing process–or higher end cars–this can make testing extremely costly~\cite{automology2021}. Tests are also labor intensive. A single test can require several days to perform, as engineers must carefully prepare the car, calibrate sensors, execute the test, and then analyze data~\cite{automology2021}. Finally, certain types of crashes are impossible to perform in simulated environments, due to the complexity of factors (e.g. multiple cars) or difficulty in simulating conditions (e.g. extreme weather events).   

Thus, evaluating crashworthiness for vehicles requires engineers to navigate a tradeoff space between the cost of a crash test, and the information it provides. As resources are limited–and testing all possible crashes is thus infeasible–engineers must therefore choose to intentionally forgo testing in certain contexts. 



%Today, the precise regulations governing crashworthiness are laid out in the Federal Motor Vehicle Safety Standards~\cite{fmvss}, which establish minimum safety and performance criteria for motor vehicles. These regulations are maintained by NHTSA pursuant to its authority under the National Traffic and Motor Vehicle Safety Act of 1966.  
% https://www.bloomberg.com/news/features/2018-10-25/even-the-crash-test-dummies-are-putting-on-weight
% https://jalopnik.com/how-your-car-gets-crash-tested-1829793856
% https://www.consumerreports.org/car-safety/some-cars-will-never-be-crash-tested-crash-test-ratings/

\subsubsection{Crash test performance thresholds}

\subsubsection{Crash testing metrics}

\subsection{}

\jessica{it could be interesting if this Analogous Practices  could provide more motivation for why the above guidelines were determined the right ones. Are there legal aspects to some of this? How do we convince the reader that these fields have figured this stuff out? Clearly the stakes are more clearly defined and higher in some of the above situations, but we should spell it out why these guidelines are good and ML practitioners should use them}

\section{Principles}

\subsection{}


\jessica{Is this list of bullets the main contribution? Where is the checklist?}



\begin{enumerate}
    \item Practitioners should ensure that the harms of live testing are dispersed widely throughout the population, and develop procedures for tracking how frequently a particular user is subject to a test. Engineers should establish upper limits on the number of tests an individual is allowed to be a part of for a fixed duration of time. In the context of AV testing for instance, such limits could manifest in terms of the number of autonomous test miles that may be driven in a particular neighborhood over a specified time period. This type of measure helps ensure that a community isn't repeatedly exposed to untested models, and mitigates the cumulative risk they face. 
    \item Engineers should develop inclusion/exclusion criteria governing which users may or may not be included in a test. The exact criteria will depend on the nature of the task, and the types of users a model is exposed to. In the context of AV testing, such criteria could be a function of neighborhood qualities. For instance, practitioners could mandate that AVs are not driven in areas with a high density of children, or during periods of the day when roads are likely to be filled with crowds. 
    \item Engineers should develop mechanisms for compensating subjects that are exposed to test models. The exact compensation model would depend on the nature of the risk and available monetary mechanisms for the engineers. For instance, AV vehicle manufacturers could provide residents of neighborhoods where AV miles are driven with transportation vouchers. 
    \item The population at risk of suffering harm from the evaluation should also recover the benefits of the computational system being evaluated. This accords with an analagous principle in clinical trials, that the population from which a trial is drawn should also benefit from the development of the drug. In the context of the evaluation practices discused above, adherence to this principle would have several implications. Autonous vehicle practitioners should be mindful of the communities in vehicles are being evaluated in. As these types of vehicles are often expensive, evaluating such systems in lower-income communities--who are unlikely to afford them--would appear to raise the concerns discussed above. In the context of content moderation systems, practitioners should take steps to ensure that the countries from which those crowdworkers are drawn also benefit from similar moderation systems. Prior work has illustrated that this unfortunately isn't the case, and content moderation systems for underresourced languages are often extremely poor~\cite{culliford2021}.
    \item Harms inflicted through evaluation may be more permissible when the alternative process an individual would interact with is known to perform poorly or highly variably. This is analaogous to instances in clinical trials where no known treatment exists, or known treatments have highly variable performance. This inquiry is based on a counterfactual---if the evaluation practice wasn't conducted, would individuals have actually suffered less harm? Suppose, for instance, that practitioners whish to deploy a computational system to replace a human decision making process, and that human decision makers have a high error rate in performing the task. This setting is quite common, and found in applications spanning law~\cite{}, content moderation~\cite{}, and medicine~\cite{}. Here, an individual would suffer no greater harm by being subject to a computational system than the baseline performance. Hence, the harm arising from live testing should be no worse than those ordinarily endured by users. Returning to our examples above, this principle suggests that when considering the ethicality of live testing with autonomous vehicles, the appropriate inquiry is whether autonomous vehicles--during testing--do not increase the danger to bystanders above and beyond what ordinary cars would. This is a highly context specific question–-autonomous vehicles may be more or less dangerous in different neighborhoods, depending on features of that neighborhood. 
    \item Finally, inflicting harm on users through evaluation may be permissible when that harm is short-lived or temporary, and individuals are not repeatedly subject to the harm. Here, we draw inspiration from the permissibility of placebo trials for less severe health conditions, and the recommendations on tracking phase one trial participants. The rationale is that when harms are minimal, they are outweighed by the benefits accrued from evaluation. 
\end{enumerate}



\subsection{Manual annotation for content moderation}

Machine learning is often employed in content moderation pipelines, where models to classify content that violates a platform's terms of service or community guidelines. Moderated content can vary significantly, but often corresponds to profane and explicit content, depicting sexual activities, violence, or bigoted ideas~\cite{chen2014}. The volume of social media content means that responsive moderation on platforms can often only occur through the use of automated tools~\cite{darbinyan2022}. Evaluating these models requires building sizeable and high quality evaluation datasets, for which human annotators must manually review and label harmful content. We discuss this practice along our aforementioned dimensions. 

Extensive reliance on human labeling for content moderation evaluation datasets presents the following advantages: 
\begin{itemize}
    \item Larger test sets offer increased statistical power, enabling more certainty in comparisons or evaluations (\textbf{internal validity}.~\cite{card2020little}. Measured differences in metrics between models are more likely to reflect actual quality differences.
    \item Larger test sets also improve the extent to which measured evaluations estimate deployment performance (\textbf{external validity}), and they are more likely to capture different subparts of the data distribution~\cite{harrison2021, roy2022does}. 
    \item For tasks like content moderation--where researchers have observed existing models often disproportionately flag content associated with minority identities~\cite{sapetal2019risk}--larger test sets enable practitioners to better detect evidence of disparate performance (\textbf{fairness}). Large test sets enable engineers to conduct disaggregated evaluations~\cite{barocas2021designing}, while still ensuring that each sub-evaluation is statistically powered.
    \item Researchers have shown that human annotations for content moderation are often subject to extensive disagreement based on annotator background~\cite{gordon2021disagreement}. Hence, acquiring more annotations per sample enables practitioners to better avoid label errors (\textbf{internal validity}). Ensuring annotations are provided by individuals from diverse backgrounds additional prevents biases from seeping into dataset-wide annotations (\textbf{fairness}).
\end{itemize}

However, extensive reliance on human annotations presents the following disadvantages:
\begin{itemize}
    \item Annotating online content can be traumatic, putting annotators at risk of physical and pyschological illness (\textbf{harmfulness}). The content that moderators see is often considered to be highly distressing, depicting graphic forms of violence and other disturbing acts~\cite{chen2014,hatmaker2022,bbc2020, newton2019}. Various studies have shown how individuals responsible for annotating these materials often suffer longer term traumatic stress disorders and experience burnout~\cite{steiger2021psychological}.
    \item Annotators are often drawn from non-Western countries, where they often work in borderline exploitative conditions for little pay~\cite{hao2022venezuela}. Prior work has noted the structural harms arising out of data labeling employment practices, including poor wages and working conditions~\cite{hao2022venezuela, hao2019}. This has given rise to concerns that–for harmful tasks like content moderation-certain demographic groups disproportionately suffer the longer term harms (\textbf{fairness}). 
\end{itemize}



%Constructing large evaluation test sets requires significant manual labor to curate and annotate data. Annotation is a delicate process, and mistakes can contaminate test sets and lead to incorrect metrics~\cite{paullada2021data}. For instance, researchers have identified mislabelled samples in popular benchmarks~\cite{northcutt2021pervasive} and underspecified label schema~\cite{tsipras2020imagenet}. As a result, machine learning practitioners spend extraordinary resources in dataset development, with a suite of technology companies specializing in offering data labelling services~\cite{kahn2020}. 


%\jessica{so, here we've prioritized validity over cost, but we've introduced harms. The image I get of all this is that we have these pairs of values, where we put the point closer to one end than the other (we prioritize validity over cost) but then because these values tend to be interrelated, everytime we adjust balance between some pair of values we may introduce imbalance with some other value (eg by moving toward validity and away from cost, we've also moved away toward prioritizing lack of harmfulness. }

%However, the reliance on human laborers to construct label content for moderation has raised significant concerns.  Moreover, 

%The choice to have human crowdworkers label evaluation datasets for tasks like content moderation requires balancing different values. On the one hand, constructing larger evaluation datasets, by hand, will provide a more accurate assessment of model performance. On the other hand, the process of constructing these datasets can significantly harm the workers employed in the task. These considerations go beyond merely the choice to construct an evaluation dataset, and implicate other questions. For instance, larger datasets--or datasets with multiple annotations per sample--improve the correctness of an evaluation, but also increase the net harm inflicted.

%\jessica{so, how do we solve this? it seems like the answer has to be more explicit cost benefit analysis. So is part of our argument that currently people are not doing these analyses, and its because they are not thinking about how the dimensions relate? I think we need to be explicit about this kind of motivation}

\subsection{Label disagreements}

Machine learning models are sometimes deployed for tasks where ``ground-truth'' can be highly subjective. Evaluation in these settings can be challenging, as the labels associated with a test dataset may be subject to disagreements~\cite{paullada2021data}. For example: 

\begin{itemize}
    \item For content moderation, researchers have observed that there is significant disagreement between different individuals as to whether a piece of content contains harmful or toxic messages~\cite{van2018challenges}. Unsuprisingly, disagreements often reflect demographic differences, as individuals from different communities frequently express different reactions to certain types of speech~\cite{haimson2021disproportionate}. 
    \item In medical settings, doctors sometimes disagree on diagnoses, or how to classify a particular condition~\cite{schaekermann2019understanding, nadis2022}.
    \item In e-discovery--where law firms use machine learning to identify documents pertaining to the issues litigated in a particular lawsuit--lawyers often disagree as to which documents are actually relevant~\cite{guha2022vulnerabilities}.
\end{itemize}

Evaluation under label uncertainty forces practitioners to tradeoff between different values. For instance, practitioners may elect to acquire multiple annotations per sample, and use the most common annotation as ground truth~\cite{gordon2021disagreement}. Here, practitioners sacrifice breadth for depth, as ensuring each sample has multiple annotations means that fewer samples can be annotated under a fixed budget~\cite{chen2022clean}. Additionally, prior work has highlighted how majority voting over annotations disregards minority voices, who may be more impacted by the predictions of the model~\cite{gordon2021disagreement}. In content mdoeration for instance, racial and ethnic minorities are more likely to be the target of toxic content online. Hence, disregarding their voices under a majority vote scheme may be yield suboptimal model performance. Alternatively, practitioners may elect to disregard samples where annotator disagreement meets a certain threshold. This however, alters the distribution of the test set. When disagreements indicate the complexity of a sample, evaluation sets become easier, thereby inflating metrics. 
 

\section{Principles}

\subsection{}


\jessica{Is this list of bullets the main contribution? Where is the checklist?}



\begin{enumerate}
    \item Practitioners should ensure that the harms of live testing are dispersed widely throughout the population, and develop procedures for tracking how frequently a particular user is subject to a test. Engineers should establish upper limits on the number of tests an individual is allowed to be a part of for a fixed duration of time. In the context of AV testing for instance, such limits could manifest in terms of the number of autonomous test miles that may be driven in a particular neighborhood over a specified time period. This type of measure helps ensure that a community isn't repeatedly exposed to untested models, and mitigates the cumulative risk they face. 
    \item Engineers should develop inclusion/exclusion criteria governing which users may or may not be included in a test. The exact criteria will depend on the nature of the task, and the types of users a model is exposed to. In the context of AV testing, such criteria could be a function of neighborhood qualities. For instance, practitioners could mandate that AVs are not driven in areas with a high density of children, or during periods of the day when roads are likely to be filled with crowds. 
    \item Engineers should develop mechanisms for compensating subjects that are exposed to test models. The exact compensation model would depend on the nature of the risk and available monetary mechanisms for the engineers. For instance, AV vehicle manufacturers could provide residents of neighborhoods where AV miles are driven with transportation vouchers. 
    \item The population at risk of suffering harm from the evaluation should also recover the benefits of the computational system being evaluated. This accords with an analagous principle in clinical trials, that the population from which a trial is drawn should also benefit from the development of the drug. In the context of the evaluation practices discused above, adherence to this principle would have several implications. Autonous vehicle practitioners should be mindful of the communities in vehicles are being evaluated in. As these types of vehicles are often expensive, evaluating such systems in lower-income communities--who are unlikely to afford them--would appear to raise the concerns discussed above. In the context of content moderation systems, practitioners should take steps to ensure that the countries from which those crowdworkers are drawn also benefit from similar moderation systems. Prior work has illustrated that this unfortunately isn't the case, and content moderation systems for underresourced languages are often extremely poor~\cite{culliford2021}.
    \item Harms inflicted through evaluation may be more permissible when the alternative process an individual would interact with is known to perform poorly or highly variably. This is analaogous to instances in clinical trials where no known treatment exists, or known treatments have highly variable performance. This inquiry is based on a counterfactual---if the evaluation practice wasn't conducted, would individuals have actually suffered less harm? Suppose, for instance, that practitioners whish to deploy a computational system to replace a human decision making process, and that human decision makers have a high error rate in performing the task. This setting is quite common, and found in applications spanning law~\cite{}, content moderation~\cite{}, and medicine~\cite{}. Here, an individual would suffer no greater harm by being subject to a computational system than the baseline performance. Hence, the harm arising from live testing should be no worse than those ordinarily endured by users. Returning to our examples above, this principle suggests that when considering the ethicality of live testing with autonomous vehicles, the appropriate inquiry is whether autonomous vehicles--during testing--do not increase the danger to bystanders above and beyond what ordinary cars would. This is a highly context specific question–-autonomous vehicles may be more or less dangerous in different neighborhoods, depending on features of that neighborhood. 
    \item Finally, inflicting harm on users through evaluation may be permissible when that harm is short-lived or temporary, and individuals are not repeatedly subject to the harm. Here, we draw inspiration from the permissibility of placebo trials for less severe health conditions, and the recommendations on tracking phase one trial participants. The rationale is that when harms are minimal, they are outweighed by the benefits accrued from evaluation. 
\end{enumerate}


==> old/old_05_neha.tex <==

\subsection{OLD SECTION 5 BELOW.}

% possibly add citation to Meira Levinson

\begin{table}[ht]
    \centering
    \begin{tabular}{|p{0.4\linewidth}|p{0.6\linewidth}|}
        \hline
        \multicolumn{2}{|c|}{\textbf{Best practies in analagous domains}} \\
        \hline
        \textbf{Tradeoff} & \textbf{Analogous Domain} \\
        \hline
        \multirow{2}{*}{Internal and External validity (\& social impact?) } & Treatment effects in economics - Section \ref{sec:socsci} \\
        \cline{2-2}
        & Representation in Clinical Trials - Section \ref{sec:clinical} \\
        \hline
        Cost prohibits information gain & Crash Test construction - Section \ref{sec:auto} \\
        \hline
        Information gain may yield negative social impact & Use of placebo drugs in clinical trials  - Section \ref{sec:clinical} \\
        \hline
        Privacy gained for Interpretability & NASS data collection for highway safety - Section \ref{sec:auto} \\
        \hline
        Privacy lost due to reduced Cost & FERPA and student privacy in academia - Section \ref{sec:educ} \\
        \hline
        Fairness enforced regardless of Cost & ADA Standards for public and government buildings - Section \ref{sec:ada} \\
        \hline
        Sustainability required to be discussed (but not necessarily optimized), regardless of Cost & National Environmental Policy Act and environmental impact assessments - Section \ref{sec:epa} 
        \\
        \hline
        \multirow{2}{*}{Privacy and Social Impact } & SNAP benefit execution - Section \ref{sec:snap} \\
        \cline{2-2}
        & Worker safety and whistleblower protection - Section \ref{sec:whistle} \\
        \\
        \hline
    \end{tabular}
    \vspace{1em} % Add vertical space between the two sections
    \begin{tabular}{|p{0.4\linewidth}|p{0.6\linewidth}|}
        \hline
        \multicolumn{2}{|c|}{\textbf{Tradeoffs Notable in ML}} \\
        \hline
        \textbf{Tradeoff} & \textbf{Situation} \\
        \hline
        Fairness and Privacy & Established tradeoff in ML literature
        \\
        \hline
        Social Impact and Fairness & Harmful content labelling prior to developing fair models?
        \\
        \hline
    \end{tabular}
    \caption{Ethical Value Debates}
    \label{tab:example}
\end{table}



The ethical tradeoffs implicated in the practices above are not unique to machine learning pipelines. The tensions they present--between competing values like harm avoidance and accuracy--pervade evaluation practices that are common in other highly technical fields. Studying these practices can be valuable to teams developing value-driven machine learning evaluations. 

These fields have developed ethical, regulatory and administrative frameworks that help them balance the value tradeoffs which arise in different evaluation practices. Or, they have informal best practices that guide ethical evaluation. The frameworks offer principles which are directly relevant to machine learning development. Since practitioners in these disciplines have deployed actual systems at scale, they are more battle-tested and can benefit machine learning developers as the field rapidly evolves. 

\jessica{I think this would be more convincing if we just presented the key takeaways. It feels like the writing style is a little slow to get to the point, and its not stated precisely enough to seem like a clear generalizable contribution. Ie as a reader I feel like I need to do the work to pull out common themes from the description of a bunch of specific cases. See my earlier comments with suggestions about distinguishing Desirable Properties and Outcomes and framing this as overall a utility maximization problem. It would be nice if there was some underlying formalism to refer to throughout these discussions. Otherwise it starts to feel like we haven't done enough synthesis for this to rise to the level of a research contribution - it reads more like the start of a discussion than something concrete we are providing for community.}

These are not the only analogous domains in which these value tradeoffs appear, and we do not aim to be comprehensive in this listing. Additionally, we highlight that there are some tradeoffs that are already particularly notable in ML, such as fairness and privacy, or social impact tradeoffs for downstream fairness ~\todocite{?}. \neha{I don't think it makes sense to expand on these two in a whole paragraph (for which I couldn't find an analagous domain but which are relevant to ML) but let me know if you disagree.}

\subsection{Social Science Research and Treatment Effect Estimation}\label{sec:socsci}

A common issue in social sciences research is external validity, when evidence from multiple sources may not yield consensus on results or policy implications. One emerging recommendation in the field is the usage of metastudies, or methods that jointly estimate treatment effects across various studies.

In one example, the field of labor economics has, since approximately the 1970s, studied the gender wage gap extensively, with hundreds of studies looking at different countries, time periods, and ranges of data sources. Some researchers argue the best method of aggregating these studies is via meta-analysis, which aggregate these studies. Some aggregations use sophisticated techniques, such as weighting studies by quality of data, and separating those that include factors such as experience in the labor force \cite{weichselbaumer2005meta}.

In another example, results from multiple randomized evaluations providing microcredit loans to impoverished households do not yield a clear consensus. This raises concerns that future policy recommendations can not be made. The studies being compared have differered in specifics of the microcredit policy intervention (ie the country of the study, whether individuals were in rural or urban settings, or whether women were specifically targeted).  Thus, the measured impact of these economic interventions are unable to be the same. One author proposes a statistical method that jointly estimates average effects across various studies in order to establish external validity across seven studies (each of which had already established internal validity) \cite{meager2019understanding}.

The presence of the internal and external validity debate in economics, and the growth of techniques to aggregate results across various studies, should motivate machine learning practitioners to also pay close attention to testing in which small sample results may not generalize to all populations. 

\subsection{US disability standards for public and government buildings} \label{sec:ada}

In the United States, the Department of Justice and Department of Transportation issue standards under the Americans with Disabilities Act. These standards apply to ``places of public accomodation, commercial facilities, and state and local government facilities in new construction, alterations, and additions", in order to provide accessibility for disabled adults and children. The requirements are broad, covering facilities including elevators, drinking fountains, golf facilities, and courtrooms \cite{ada}.

To assist with meeting these goals, the US Access Board - a federal agency - updates ADA standards, and engages with the public ``to inform the development of accessible design'' \cite{accessboard}. The existence of central federally funded bodies enforcing and creating fair standards could be a motivation for machine learning fairness standards.

\subsection{US government environmental impact standards} \label{sec:epa}

The 1970 National Environmental Policy (NEPA), requires environmental effects to be considered by federal agencies about their actions. This requires that  environmental analysis begin final decisions are made. It does not mandate the most environmentally sound alternative be chosen in any decision, but requires knowledge of the impact of decisions. Among other organizations, the Environmental Protection Agency works on overseeing NEPA. 

The machine learning community could similarly consider following guidelines for early considerations of environmental impacts throughout decision making, especially when weighing it against costs \cite{citizensnepa}. \neha{Not sure what is currently going on though -- theres already some regulation on bigtech footprints hence carbon credit buying...?}

\subsection{Issues with receiving public benefits} \label{sec:snap}
\neha{@hari, This one feels hard to make connect to ML, kinda want to remove}

The United States governemnt provides a federally funded program called the Supplemental Nutrition Assistance Program (SNAP) - name changed from previously being called Food Stamp Program \cite{nprsnap}. The public health benefits by receipients also come with stress in using it, originating from stigmatization by grocery clerks when paying for groceries, or ``attitude" from caseworkers in county assistance offices. Scholars offer recommendations to improve these programs such as increasing benefit durations in order to require less paperwork, and improving caseworker professionalism \cite{gaines2019recommendations}. 

The lesson that investment in employee training would increase social impact of programs is a lesson for the machine learning fairness community as well.


\subsection{Whistleblower protection}\label{sec:whistle}

As part of the US Department of Labor, the Occupational Safety and Helath Administration (OSHA), ensures ``safe and healthful working conditions for workers by setting and enforcing standards and by providing training, outreach, education and assistance". 

The US government offers privacy guarantees by permitting employees to submit confidential reports of safe workplace violations \cite{osha}. This privacy guarantee protects workers from conerns of retaliation, and thus offers increased likelihood of positive social impact in prventing unsafe working conditions. 

The existance of a federal anonymous complaint procedure with worker education on reporting, could be a beneficial blueprint as concerns regarding unsafe AI practices increase. 


\subsection{Clinical Trials and Value Evaluations} \label{sec:clinical}

A/B tests are applied in clinical settings, which implicate several value tradeoffs, including harmfulness, external validity, and internal validity.

When an A/B test is done using a placebo controlled trial, this could be argued to violate the professional obligations of doctors to provide the optimal medical care to patients. When other known beneficial treatments exist, denying patients access to those treatments for the sake of measuring the efficacy of the novel treatment against a placebo is considered by some to be both clinically and scientifically questionable. However, concerns are balanced against their prospective advantages. Placebo trials are widely considered to be the most rigorous test of treatment efficacy. They generally require fewer participants than active-controlled trials, thereby making them easier and cheaper to conduct. Even where existing treatments exist, placebo trials offer new and valuable forms of information~\cite{miller2002makes}. 

Thus, medical practitioners have come to identify several principles that guide determinations as to when placebo trials may be appropriate~\cite{millum2013ethics}. First, placebo trials are permissible when no proven treatment exists for the disorder being studied (e.g., for Alzheimer's dementia). This includes the setting where a treatment may exist, but its efficacy cannot be extrapolated to the population of interest. Second, placebo trials are permissible when preventing patients from acessing a known alternative treatment would expose them to at most ``temporary discomfort or delay in relief of symptoms.'' This is common when the medical disorder being studied is ``minor,'' like common headaches or male pattern baldness~\cite{miller2002makes, millum2013ethics}. Third, placebo trials are justified when existing treatments prove to be highly variable. This is commonly the case for conditions like depression, where established drugs can sometimes fail to outperform placebos~\cite{millum2013ethics}. Finally, placebo trials are permitted when there exist compelling methodological reasons for their use, participants are not deprived of treatments they would otherwise have access to, and the benefits of the trial will be borne by the population contributing participants. 

In these ways, the field has standardized ways to balance values of social impact and internal or external validity in evaluating drug efficacy. The field also operates under the regulation of the Internal Review Board which confirms the ethics of a proposed placebo study. 

Further proposed refinements of values within clinical trials include the push to broaden demographic representation in clinical trials. This proposal would benefit external validity of drug efficacy, as only internal validity is proven if clinical trials are done on homogenous populations. This is important in order to prevent potentially harmful outcomes \cite{bibbins2022improving}. 

This motivates questions around ways in which consumer facing online A/B testing can be subject to similar central reviews in order to balance internal and external validity, as well as social impact.

\subsection{Education Policies and Value Evaluations} \label{sec:educ}

The United States protects student privacy with the Family Educational Rights and Privacy Act of 1974 (FERPA), and Ontario, Canada with the Freedom of Information and Protection of Privacy Act (FIPPA), established in 2006. Information about the requirements of these laws is oftentimes not widespread on college campuses, particularly with new technical challenges. Some scholars note that FERPA rights such as consent to disclose records, or faculty discussing student grades without a legitimate need, are frequently commonly violated on university campuses, with one of the most cited reasons being lack of knowledge and communication. Some recommendations to alleviate these issues is to create better administrative and faculty training, as well as inform students of privacy rights \cite{gilley2006ferpa}.

FIPPA created confusion on campuses due to its complexity and forced administrations to revise outdated policies. Some recommendations say that this policy change, if accompanied with education about its necessity, would advance its effectiveness \cite{dowding2011interpreting}.

Overall, the general recommendation that privacy and social impact would be enhanced on college campuses if accompanied by investment in education - rather than minimizing costs to learning about privacy policies - is a practice that machine learning can also follow.   


\subsection{Automotive Regulations and Value Evaluations} \label{sec:auto}
\subsubsection{NASS}

Standards that ensure safety in vehicluar transportation include highway safety determinations, and vehicle crash testing. The value tradeoffs these establish can include cost, external validity, and privacy.

% TODO: talk about ways in which CDS has been used: https://crashstats.nhtsa.dot.gov/Api/Public/ViewPublication/812128 (page 13)
The National Automotive Sampling System (NASS) that is operated by the National Highway Traffic Safety Administration (NHTSA)~\cite{nassbrochure}. NASS was established in 1979 as part of an effort to reduce crashes, injuries, and fatalities involving motor vehicles. The data collected as part of NASS includes the Crashworthiness Data System (CDS), enabling NHTSA to identify existing and potential problems in highway safety, assess the performance of vehicle safety systems, learn more about the nature of crash injuries, and assess the influence of social factors on vehicle safety~\cite{nassbrochure}.

CDS contains detailed data on a representative random sample of thousands of minor, serious, and fatal crashes~\cite{cdsoverview}, studying five thousand crashes every year (spanning passenger cars, pickup trucks, and vans)~\cite{nassbrochure}. As performing investigations on all crashes would be prohibitively expensive (and logistically impossible), CDS investigations only occur for a sample of crashes. Special care is taken in the design of the sampling process~\cite{cdsmanual}. Only crashes which meet certain minimum criteria (e.g. involves a harmful event) are eligible, and the sampling probabilities are skewed to favor more recent vehicle models and more serious injuries. 

Trained crash researchers will visit crash sites, collecting information regarding the crash. This can encompass: photographs of damaged vechiles, skid marks, fluid spills, broken glass, bent guardrails, and other evidence of crash damages. Investigators will also observe the interior of vehicles, in order to document locations struck by occupants. When possible, investigators will follow up with crash victims and additionally collect medical records. Critically, CDS interviews are conducted with ``discretion and confidentiality''~\cite{cdsoverview}. Personal information pertaining to the crash--names, addresses, license and registration numbers, and even sometimes locations--are not included in publicly released NASS data.

Data is collected in adherence to strict standard established by NHTSA rules, which specifically dictate what information investigators must collect, and the precise way in which different types of information must be coded~\cite{cdsmanual}. For instance, investigators will classify the collision as one of 6 types. This helps ensure standardization across different PSUs, and enables more sound post-hoc analysis of crashes. Additionally, investigations undergo a quality control process. Each PSU works in conjunction with one of two NASS Zone Centers. Each Zone Center is staffed with the most experienced crash researchers, and is responsible for coordinating and supervising the activities of different PSUs. Prior to a crash investigation being deemed complete, the Zone Center must review the PSU's findings for quality control standards. In practice, this can result in several back-and-forths until the report has met the standards.  

The standardization of ways that agencies collect data ensures interpretability, and that the privacy is respected. This motivates the ML field to standardize data collection and establish frameworks for post-mortem analysis, while protecting privacy. 

\subsubsection{Crash test construction}

Regulators and automotive engineers administer tests to evaluate the ``crashworthiness'' of different vehicles. This is motivated by decisions made by American courts in the the late 1960s, when they began to find automotive manufacturers liable for passenger injuries where elements of the car served to exacerbate the harms experienced by passengers~\cite{choi2019crashworthy}. Though these accidents were often caused by human error, courts argued that the statistically inevitable nature of car accidents meant that manufacturers carried a duty to minimize the consequences of such accidents. This caselaw--dubbed the ``crashworthy doctrine''--would by some accounts inspire a wholesale change in the way manufacturers approached safety, be responsible for technical improvements ranging from seatbelts to padded interiors, and spur a tremendous drop in traffic deaths~\cite{choi2019crashworthy}. 

Crashworthiness is evaluated through crash tests. In a crash test, researchers place a crash dummy (formally called an anthropomorphic testing device, or ``ATD'') in a vehicle, and remotely drive the vehicle into a barrier in order to simulate a crash~\cite{engber2006}. Sensor readings from the vehicle and ATD–along with camera footage of the crash–are then studied to determine the crashworthiness of the vehicle. 

A challenge in performing evaluations of crashworthiness is that no two crashes are alike. For instance, researchers have shown that the survivability of a crash is dependent on a range of crash-specific factors, including but not limited to: weather conditions~\cite{saha2016adverse}, road conditions~\cite{fitzpatrick2014influence}, the location of the impact on the vehicle (e.g. frontal impact or side impact)~\cite{keall2018relative}, the type of impacting object (e.g. concrete barrier vs deer)~\cite{iihsobjects}, the speed at which the vehicle is travelling~\cite{iihsnewtests}, the relative wear of the vehicle itself~\cite{national2013vehicle}, the individual physiologies of the passengers~\cite{ishii2020factors}, and the actions of first responders~\cite{calland2005extrication}. 

Moreover, assessing the crashworthiness of a vehicle for every possible type of crash is infeasible. Individual tests can be extremely expensive. ATDs are sophisticated and highly engineered devices, costing between \$100,000 and \$1 million dollars, containing as many as 30,000 distinct parts, and have a limited shelf life~\cite{automology2021, hall2015, ferris2022, reilly2021}. As cars are typically destroyed after a test, each test requires a brand new vehicle. For cars earlier in the manufacturing process–or higher end cars–this can make testing extremely costly~\cite{automology2021}. Tests are also labor intensive. A single test can require several days to perform, as engineers must carefully prepare the car, calibrate sensors, execute the test, and then analyze data~\cite{automology2021}. Finally, certain types of crashes are impossible to perform in simulated environments, due to the complexity of factors (e.g. multiple cars) or difficulty in simulating conditions (e.g. extreme weather events).   

Thus, evaluating crashworthiness for vehicles requires engineers to navigate a tradeoff space between the cost of a crash test, and the information it provides. The ways that crash responsibility is on auto companies and successfully motivates thorough testing standards, motivate the need for regulatory practices that ensure responsible, safe AI, to ensure that corporations invest in testing. 


%Today, the precise regulations governing crashworthiness are laid out in the Federal Motor Vehicle Safety Standards~\cite{fmvss}, which establish minimum safety and performance criteria for motor vehicles. These regulations are maintained by NHTSA pursuant to its authority under the National Traffic and Motor Vehicle Safety Act of 1966.  
% https://www.bloomberg.com/news/features/2018-10-25/even-the-crash-test-dummies-are-putting-on-weight
% https://jalopnik.com/how-your-car-gets-crash-tested-1829793856
% https://www.consumerreports.org/car-safety/some-cars-will-never-be-crash-tested-crash-test-ratings/

%\jessica{it could be interesting if this Analogous Practices  could provide more motivation for why the above guidelines were determined the right ones. Are there legal aspects to some of this? How do we convince the reader that these fields have figured this stuff out? Clearly the stakes are more clearly defined and higher in some of the above situations, but we should spell it out why these guidelines are good and ML practitioners should use them}



